"I Try to Represent Myself as I Am": Self-Presentation Preferences of People with Invisible Disabilities through Embodied Social VR Avatars

With the increasing adoption of social virtual reality (VR), it is critical to design inclusive avatars. While researchers have investigated how and why blind and d/Deaf people wish to disclose their disabilities in VR, little is known about the preferences of many others with invisible disabilities (e.g., ADHD, dyslexia, chronic conditions). We filled this gap by interviewing 15 participants, each with one to three invisible disabilities, who represented 22 different invisible disabilities in total. We found that invisibly disabled people approached avatar-based disclosure through contextualized considerations informed by their prior experiences. For example, some wished to use VR's embodied affordances, such as facial expressions and body language, to dynamically represent their energy level or willingness to engage with others, while others preferred not to disclose their disability identity in any context. We define a binary framework for embodied invisible disability expression (public and private) and discuss three disclosure patterns (Activists, Non-Disclosers, and Situational Disclosers) to inform the design of future inclusive VR experiences.

==> sections/0-abstract-diff.tex <==
As social virtual reality (VR) grows in popularity, \DIFdelbegin \DIFdel{avatar design must be inclusive }\DIFdelend \DIFaddbegin \DIFadd{it is critical to design inclusive avatars}\DIFaddend . While researchers have investigated preferences of blind and d/Deaf people, \DIFdelbegin \DIFdel{less }\DIFdelend \DIFaddbegin \DIFadd{little }\DIFaddend is known about the preferences of \DIFdelbegin \DIFdel{people }\DIFdelend \DIFaddbegin \DIFadd{many others }\DIFaddend with invisible disabilities (e.g., \DIFdelbegin \DIFdel{ADHD}\DIFdelend \DIFaddbegin \DIFadd{autism}\DIFaddend , depression, rheumatoid arthritis)\DIFdelbegin \DIFdel{, especially in the embodied context of VR}\DIFdelend . We fill this gap through semi-structured interviews with \DIFdelbegin \DIFdel{12 participantswho represent 19 invisible disabilities . Participants }\DIFdelend \DIFaddbegin \DIFadd{14 participants, each with one to three invisible disabilities, who represent 22 invisible disabilities in total. We found that invisibly disabled people }\DIFaddend approached avatar-based disclosure through \DIFaddbegin \DIFadd{contextualized }\DIFaddend considerations informed by \DIFaddbegin \DIFadd{their in }\DIFaddend non-virtual and virtual experiences. \DIFdelbegin \DIFdel{Many used (or wanted to use) }\DIFdelend \DIFaddbegin \DIFadd{For example, some used }\DIFaddend VR’s multimodal affordances \DIFdelbegin \DIFdel{to represent their disabilities }\DIFdelend (e.g., facial \DIFdelbegin \DIFdel{expressions}\DIFdelend \DIFaddbegin \DIFadd{expression}\DIFaddend , body language) \DIFaddbegin \DIFadd{to represent their disabilities, while others preferred not to disclose their disability identity in any contexts, virtual or non-virtual}\DIFaddend . Participants proposed \DIFdelbegin \DIFdel{new features , }\DIFdelend \DIFaddbegin \DIFadd{features }\DIFaddend like a floating energy bar to indicate social battery \DIFdelbegin \DIFdel{, along with }\DIFdelend \DIFaddbegin \DIFadd{and suggested }\DIFaddend ways to make \DIFdelbegin \DIFdel{customization }\DIFdelend \DIFaddbegin \DIFadd{the customization process more }\DIFaddend accessible. We \DIFdelbegin \DIFdel{discovered a }\DIFdelend \DIFaddbegin \DIFadd{discuss the }\DIFaddend distinction between public (explicit) and private (implicit) representations of disability, which \DIFdelbegin \DIFdel{is our proposed binary for embodied disability expression. We discuss how these findings can facilitate }\DIFdelend \DIFaddbegin \DIFadd{we pose as a binary framework for embodied invisible disability expression to inform }\DIFaddend the design of inclusive VR experiences. 

==> sections/0-abstract.tex <==
As social virtual reality (VR) grows in popularity, avatar design must be inclusive. While researchers have investigated preferences of blind and d/Deaf people, less is known about the preferences of people with invisible disabilities (e.g., ADHD, depression, rheumatoid arthritis), especially in the embodied context of VR. We fill this gap through semi-structured interviews with 12 participants who represent 19 invisible disabilities. Participants approached avatar-based disclosure through considerations informed by non-virtual and virtual experiences. Many used (or wanted to use) VR’s multimodal affordances to represent their disabilities (e.g., facial expressions, body language). Participants proposed new features, like a floating energy bar to indicate social battery, along with ways to make customization accessible. We discovered a distinction between public (explicit) and private (implicit) representations of disability, which is our proposed binary for embodied disability expression. We discuss how these findings can facilitate the design of inclusive VR experiences.

==> sections/1-introduction.tex <==
\section{Introduction}
Like anyone else, people with disabilities want to represent their unique identities through their avatars when interacting with others in social VR spaces. Among other functions, avatars are vessels for self-expression in VR \cite{freeman_maloney_perception_of_self}, and their characteristics provide cues that mediate interpersonal interactions. Social VR platforms can offer users a strong sense of embodiment and freedom from some forms of physical constraint, and as more people turn to social VR for social connection, the importance of diverse mechanisms for self-expression grows \cite{falling_asleep, yalon_leisure}. However, more work needs to be done to understand what kinds of avatar representations can highlight disability identities accurately despite stigma, given the varying needs of potential users of social virtual reality spaces. 

Zhang et al. \cite{zhang_partofme} found users with visible disabilities wanted to use their avatars to disclose their disabilities, highlight their needs, and raise awareness through their VR interactions. Some desired to incorporate components like signing ASL through their avatars and adding realistic and customizable assistive technology (e.g., hearing aids) to better align their avatar representations with their non-virtual self-presentations. All participants in this study had \textit{visible} disabilities they wanted to represent through personal objects that disclosed their disability to others in the physical world. 

Many people do not appear or behave in ways that make their disability apparent to others. Indeed, there are 33 million people in the U.S. alone who have such invisible disabilities (approximately 10\% of the U.S. population) \cite{disabledworld}. 

Mack et al. \cite{mack_towards} was the first to examine avatar representations of invisible disabilities through a broad study of both visible and invisible disability representation on digital platforms (e.g., Snapchat, Animal Crossing, Facebook). They found that users with visible disabilities wanted to implement more concrete representations of their non-virtual bodies and assistive technologies, while users with invisible disabilities wanted to use more abstract, disability-related avatar symbols with metaphorical meaning (e.g., words in the dyslexia-friendly font “Bionic”) to signal membership in a specific community. 

However, Mack et al. \cite{mack_towards} did not explicitly explore embodied avatars found in social VR spaces, focusing instead on avatars like Snapchat Bitmojis and Apple Memojis that are stickers or still photos, as well as avatars from digital video games (e.g., Animal Crossing). Preferences regarding embodied avatars are likely to differ from non-embodied avatars because VR’s affordances for capturing the nuances of physical human expression far exceed digital platforms \cite{freeman_maloney_perception_of_self}. On digital platforms, users are limited to 2D, static images of their avatars. Conversely, social VR users use embodied 3D avatars to represent themselves, which are capable of capturing much more granular nuances, extending as far as dynamic facial expressions and body language as they socialize with others.

In this paper, we examine the embodied avatar preferences of people with invisible disabilities, amplifying the voices and experiences of this marginalized group within the social VR context for the first time. To broaden our understanding of how we can best construct the offerings of a disability-inclusive avatar customization library, we conducted an interview study that investigated how people with invisible disabilities present, and may \textit{want} to present, their identities in social VR contexts. Specifically, we posed the following research questions: 

\begin{itemize}
   \item \textbf{RQ1:} How do people with invisible disabilities represent disability in social virtual reality avatars today?
    \item \textbf{RQ2:} How can social virtual reality avatars better represent the experiences and identities of people with invisible disabilities?
    \item \textbf{RQ3:} When, why, and how do people want to share invisible disability identities and experiences using avatars in social virtual reality? 
\end{itemize}

We conducted semi-structured interviews with 12 participants with invisible disabilities such as ADHD, depression, and rheumatoid arthritis. During the interviews, we included a visual brainstorming component where participants sketched an \textit{ideal} avatar self-representation, going beyond what is currently available on customization platforms to generate preliminary design ideas \cite{johnson_sketching}. Understanding that verbal brainstorming often privileges interviewees who are comfortable generating ideas and expressing themselves through voice, we wanted to offer an alternative opportunity for self-expression to accommodate a broader range of communication styles. 

We found that social VR users with invisible disabilities draw many important connections and distinctions between virtual and non-virtual social spaces (e.g., equating the experiences of non-virtual and virtual fishing, mapping on norms from non-virtual professional environments to virtual professional engagements), which can impact disclosure preferences. In addition, we discovered that while some users with invisible disabilities already customize avatar appearances to indicate dynamic preferences for social engagement in implicit ways, many might desire more options for customizing facial expressions and body language to express their disabilities. Based on our findings, we also propose a distinction in disability representation between private (i.e., implicit) representations, like knee pads that symbolize a need for self-protection from bipolar mood swings, and  public (i.e., explicit) representations like disability-related shirt graphics. We provide design recommendations to inform a more accessible avatar \textit{creation} experience (e.g., reducing the amount of arm movement required to scroll through customization offerings).

In summary, we contribute a discussion of avatar customization opportunities in social virtual reality to support the large and underserved population of people with invisible disabilities, which is another step toward making social VR more inclusive to all users. 


==> sections/2-related-work.tex <==
\section{Related Work}
Broadly, social VR platforms lack diverse customization options (e.g., regarding body and racial diversity \cite{Lee_2014_Does, lee_whose_2011, Morris_2023_hide}). Invisible disability representation in social VR is even less present. Despite the invisible nature of some disabilities, identity representation is important. For one, by rendering invisible experiences visible, doors open for building awareness of underrepresented experiences. Further, social VR offers unique affordances for users to represent aspects of their identities in different ways compared to non-virtual contexts \cite{freeman_maloney_perception_of_self}.

\subsection{Disability Disclosure}
Many people with disabilities have varied perspectives on when and why to disclose their disability. Although discrimination against individuals with disabilities is legally prohibited\footnote{The Americans with Disabilities Act (ADA) of 1990 and Section 504 of the Rehabilitation Act of 1973 both protect people with disabilities from discrimination on the basis of their disability.}, people with disabilities are still subject to discrimination, even if it is unintentional. As a result, they may have to carefully consider whether or not to disclose their disabilities. 

People with invisible disabilities may have more success at concealing their disability at their discretion compared to people with visible disabilities, 
especially if they believe their disability is “mild” and “irrelevant” to their work performance \cite{lindsay_work, schrader_workplace_climate, dalgin_hiring}. However, this invisibility also means that people with invisible disabilities struggle to be taken seriously when seeking accommodations. They may anticipate negative perceptions, which can make them hesitant to disclose \cite{mullins_invisible_uni}. Since invisible disabilities can require more steps to verify than visible disabilities, some people may experience barriers to feeling their disclosure was accepted. Moriña \cite{morina_barriers_education} found that students with invisible disabilities struggled with the stress and insecurity associated with “proving” their disability. Often, they were challenged by people who refused to believe they were “disabled,” which made them want to distance themselves from a disability identity and appear “normal” \cite{morina_barriers_education}. Therefore, while both people with visible and invisible disabilities anticipate and encounter stigma, people with invisible disabilities may struggle more with validating their disability to themselves and others. Meanwhile, they may also desire to disclose differently in different contexts.

\subsection{Social VR Use}
Recently, social VR has gained increasing popularity, enabling immersive 3D experiences by allowing users to meet, interact, and socialize in the form of virtual avatars \cite{freeman_maloney_perception_of_self}. Unlike 2D social media and digital worlds, social VR uniquely affords immersive embodied experiences \cite{falling_asleep}. For example, VR head-mounted displays allow real-time body movements and gestures to be tracked and rendered in virtual environments. 

A person’s sense of embodiment (SoE) is characterized by their ability to control their body’s movements, experience the sensations their body does, and feel they are within their body \cite{kilteni_soe}. In immersive virtual reality, SoE is enhanced through embodying avatar representations. Additionally, in headset-based social VR, users' non-virtual bodies and surroundings are occluded, increasing immersion \cite{genay_for_real}.

Social VR platforms offer a variety of activities. Users can connect with others by hosting and attending parties, playing games together, and collaborating remotely on work \cite{freeman_maloney_perception_of_self, abramczuk_remote_work}. To better understand which social VR experiences users value, Maloney and Freeman \cite{falling_asleep} interviewed 30 social VR users. Their findings indicated that users enjoyed doing full-body mirroring activities with expressive movements (e.g., dancing), experiencing everyday practices (e.g., sleeping) in novel immersive ways, and practicing self-improvement skills they normally would not focus on in non-virtual worlds (e.g., social skills and mental states). 

Social VR platforms are particularly appealing to people with disabilities since they can address accommodations needs in ways that go beyond what is possible in the physical world. For example, people with physical and intellectual disabilities can engage in activities, such as horseback riding and swimming, which are typically inaccessible in the physical world \cite{yalon_leisure}. Yalon-Chamovitz and Weiss \cite{yalon_leisure} found that VR offers people with disabilities a greater sense of autonomy over their bodies and environments. This also applies to people with invisible disabilities. For instance, in VR, neurodivergent users may remove themselves from overwhelming situations or adjust settings to reduce their sensory load \cite{boyd_leveling}. Given its increasing popularity and unique affordances, it is important to understand how people with invisible disabilities want to engage with the virtual social sphere through avatar representation.

\subsection{Avatar Self-Expression}
Avatars facilitate social interactions and allow users to control their self-presentations. Avatar customization heightens the user’s sense of connection and ownership over their virtual body, thus intensifying SoE \cite{langener_embodiment}. In fact, many social VR users choose to represent themselves as accurately as possible through their avatars \cite{freeman_maloney_perception_of_self}. However, depending on context, users may also choose to creatively express their interests and identities through their avatars, sometimes extending beyond what is possible in the non-virtual world \cite{won2023your}. A myriad of prior works have explored identity and avatar representation in social VR \cite{freeman_maloney_perception_of_self}, including perspectives from diverse user groups such as racial minorities \cite{blackwell_harassment}, women \cite{sharvit_sexual_harass}, and LGBTQ users \cite{freeman_acting_out, freeman_rediscovering}. For example, Freeman et al. \cite{freeman_maloney_perception_of_self} conducted interviews with VR users and found that most of them strove to make their avatars as similar as possible to their non-virtual counterparts because they considered avatars to be extensions of themselves in virtual worlds. Another study by Freeman et al. \cite{freeman_rediscovering} explored the avatar choices of non-cisgender users and revealed that they changed their avatar’s gender expression frequently, through outfits and accessories, to indicate their flexible and gender-fluid identities.

Social VR also facilitates significant body modification. Users may opt for fantastical, cartoonish, and non-human features, such as the red eyes and snake eyes offered in Ready Player Me \cite{readyplayerme}. They can also choose non-human avatars \textemdash{} one participant in Freeman and Maloney’s study \cite{freeman_maloney_perception_of_self} represented herself as a blue bird. Furthermore, users can enable complete or partial invisibility of their avatars by manipulating the meshes that make up the 3D model \cite{youtube_invisibility_toolbox, youtube_invisibility_PxINKY}. Such customizations allow users to communicate their individuality, explore different ways of representing their identities, and maintain greater control over how others perceive them.

Still, current avatar customization options are often limited in representing identity. For example, Ready Player Me, a popular avatar creation tool, only presents gender as a binary \cite{readyplayerme}. 
In addition, avatars generally skew toward youthful representations. Middle-aged female participants in Morris et al.’s study \cite{Morris_2023_hide} noted that  existing avatar customization options made them feel like a “caricature” of an older person.

Some recent work has begun to investigate avatar representations of disability. Zhang et al. \cite{zhang_partofme} found users disclosed disabilities by attaching assistive technology to their avatars (e.g., hearing aids) and adopted a spectrum of disclosure strategies to represent their identities in social VR. Additionally, Davis and Chansiri \cite{davis_digital_identities} found that online users with disabilities customized their digital avatars to foster a greater sense of empowerment. For instance, one user depicted herself as younger because she felt her disability removed years from her life. Mack et al. \cite{mack_towards} shed light on some challenges facing individuals with intersectional identities as they represented themselves in digital platforms, noting they often had to choose between using avatars to represent their disability or race-related identities. Their work included participants with visible and invisible disabilities, and they found the former wanted to implement representations of assistive technology while the latter wanted to use symbolic representations of disability that would resonate with their more specific community (e.g., chronic illness, ADHD). 

Our study extends the work above in several ways. First, we focus on social VR users with all types of invisible disabilities, distinct from Zhang et al.’s study \cite{zhang_partofme} which focused on people with visible disabilities (who use assistive technology). Our study investigates invisible disabilities that often do not require assistive technology. Thus, we explore social VR affordances that are not necessarily available in non-virtual spaces. In addition, we build on Mack et al.’s study \cite{mack_towards} of digital avatars, which was the first avatar study to include users with invisible disabilities. However, one study is not enough to fully capture the diverse perspectives of avatar users with invisible disabilities, and findings from a digital context do not necessarily map on to user preferences in a virtual context due to significant differences in affordances. Given there is still much work to be done on this topic, we include users with diverse invisible disabilities as a broad group to identify generative areas of research that future work can expand. We contribute a distinct discussion of invisible disability representation preferences in immersive VR spaces. In this study, we examine how users with invisible disabilities want to employ VR’s multimodal affordances for disability expression in spaces where embodied avatars mediate all social interactions. 

==> sections/3-methodology.tex <==
\section{Methodology}
We conducted semi-structured interviews with 12 participants who self-identified as having one or more invisible disabilities. We hoped to understand their perspectives on disability representation and disclosure in both non-virtual and social VR settings. In addition, we sought to discover how they want to use social VR's affordances to represent their disabilities through avatars. 

\subsection{Recruitment}
We recruited participants by emailing disability-related organization mailing lists, posting messages in relevant groups on Reddit, and partnering with an academic department’s undergraduate extra credit system at a North American university. Our inclusion criteria were as follows: Participants must 1) Be at least 18 years old, 2) Have an invisible disability, and 3) Have experience using social VR platforms. 

Our recruitment materials stated: “We define having invisible disabilities as including physical and psychological conditions that often have no visible manifestation, such as attention deficit, autism, and chronic health issues. We define social VR as a virtual platform where people communicate and interact with others in the form of avatars. Some popular social VR platforms include Rec Room, VRChat, vTime XR, and AltspaceVR.” Note that we released these recruitment materials before AltspaceVR was shut down. 

Given the driving analytical method of this study was thematic analysis \cite{braun2012thematic}, we halted recruitment once thematic saturation was reached during our 12th interview, at which point no new themes emerged. This aligned with Ando et al. \cite{ando_saturation}, which found all thematic analysis themes could be identified within 12 interviews. 

\subsection{Participants}
This study consisted of 12 participants aged 20 to 56 years old ($mean = 33.75, SD = 10.52$). Seven identified as female and five identified as male. Regarding race, six participants identified as White, two as Black, two as Mixed-Race, one as Asian, and one as Alaska Native. Eleven participants disclosed their disabilities, identifying disabilities such as dyslexia, chronic pain, ADHD, and depression. In total, 19 unique invisible disabilities were represented in this sample. All participants had experience with at least one social VR platform, but many had used multiple (e.g., VRChat, AltspaceVR, Spatial, Rec Room). Most used VR on a daily or weekly basis. See Table 1 for a more detailed demographic breakdown. Participants were compensated with a \$20 Amazon gift card after the interview’s conclusion. This study, and all procedures, were approved by our university's Institutional Review Board for Human Participants (IRB), and all participants provided informed consent.

\subsection{Procedure} We conducted semi-structured interviews via video conferencing software (Zoom), with a creative component done through a collaborative whiteboard application (Google Jamboard). Google Jamboard allowed participants to draw and paint in multiple colors, import and link images from a device or an online search, type thoughts and ideas on sticky notes, and create text boxes and shapes. Participants could also use a virtual laser pointer to emphasize different aspects of the whiteboard while describing features of their creative expression if they so chose. All interviews were conducted in English, lasted approximately 60 minutes, and were video and audio recorded with participants' consent. 

Each interview began with an introduction to the research and a review of the consent form prior to obtaining oral consent. After obtaining consent, we asked participants about how they currently used social VR and represented themselves with avatars. We probed their current use of avatars as vessels for disclosure (or not). For example, we asked: “Do you represent or conceal your invisible disability in social VR in any way? How similar is your avatar representation to your physical self?” After establishing the similarities and differences between participants’ virtual and non-virtual selves, we asked if participants were interested in representing their invisible disability / disabilities in social VR. Regardless of their responses, we followed up by discussing how context might impact their decisions to represent (or not represent) their invisible disabilities. 

In the second section, we invited participants to share ideas for their “ideal avatar representation” in social VR by using a virtual whiteboard to express their ideas through images, drawing, and/or text.  After describing the thought processes behind their visualizations, participants were asked to describe any important features that were \textit{not} currently available, as well as their ideal customization process.

In the third section, we further explored the importance of context in virtual and non-virtual disclosure. We asked questions such as, “In the physical world, how do you navigate disability disclosure? Would you consider your avatar representation to be the same or different in different settings? How does this compare to other platforms with avatar options, such as Snapchat?” Finally, we discussed the practical implications of incorporating invisible disability representation features into avatar libraries. 

\subsection{Analysis} Our data consisted of approximately 15 hours of recordings and detailed notes collected during the interviews. After transcription, we used open coding to analyze the interviews. Three researchers divided the first three transcripts so that each was double-coded, discussed code discrepancies, created the preliminary codebook, and then split up the remaining transcripts for individual coding. Throughout the coding process, we iterated and refined the codebook over the course of approximately five meetings. 

After coding, we conducted thematic analysis \cite{braun2012thematic} to identify overarching thematic takeaways and patterns across participants. Our themes were grounded in the interview codes as well as the suggestions presented by participants during the whiteboard component, which included image and drawing artifacts. Per Clarke and Braun’s thematic analysis guide \cite{clarke2013thematic}, three team members generated lists of potential themes through bulleted outlines. They then identified the connections between them as preparation for a thematic analysis meeting. Then, they reflected on the proposed themes’ connections to the study's research questions, compared areas of overlap and divergence, and reflexively confronted any potential analytical assumptions. Finally, the three coders selected the themes that overlapped between their lists and consulted with other team members to ensure themes engaged substantively with interpretative contributions, tweaking the thematic headings until they arrived at their final version. 

\subsection{Positionality} The first author lives with an invisible disability and has a background in feminist disability studies. The research team also includes social VR users, accessibility researchers, and people who have grappled with the complex issue of disability disclosure in their own lives. We believe improving avatar customization options is an important step toward maximizing the inclusiveness of social VR spaces and aim to include the voices of VR users with invisible disabilities into the important conversations surrounding how to foster positive representation and cultivate diverse spaces. 


\begin{table*}[h!]
    \footnotesize 
    \centering
    \caption{Participants' demographics.} 
    \begin{tabular}{p{0.3cm}p{0.9cm}p{1.5cm}p{2.8cm}p{3.8cm}p{2.8cm}}
    \toprule
      \textbf{ID}&  \textbf{Age/ Gender}&  \textbf{Race}&  \textbf{Disabilities}&  \textbf{Social VR Use}&   \textbf{Frequency} \\
     \midrule 
    
   \textbf{P1}&   32/F&   White&  Low Vision&  Altspace VR; Spatial&  several times/week \\ 
    \midrule
    
    \textbf{P2}&   32/F&   White& Bipolar Disorder; PTSD&  Synth Riders; VR fishing; VRChat; Walkabout Mini Golf VR; & daily\\ 
    \midrule

     \textbf{P3} & 56/F & Mixed-Race&  Dyslexia; Congestive Heart Failure; Rheumatoid Arthritis& Altspace VR; VR Fishing; VR Chat; Spatial; Big Screen; Wander& weekly\\ 
    \midrule
    
      \textbf{P4}&    38/F&    White &  Dyslexia; Epilepsy; Chronic Pain& Les Mills BODYCOMBAT VR, FedEx, Beat Sabre, Mini Golf VR& two to four or five times a week\\ 
    \midrule
    
      \textbf{P5}&    31/M&    White&   RSI; ADHD; Asperger's& two to four or five times a week&  social: monthly
VR in general: weekly\\ 
    \midrule

    \textbf{P6}&    24/F&    Black &   POTS& vTime XR; Altspace VR; Rec Room; miscellaneous& weekly\\ 
    \midrule
    
      \textbf{P7}&    33/F&    White&   Depression& VR Chat&  daily\\ 
    \midrule
    
      \textbf{P8}&    20/M&   Asian&   Chronic condition (diagnosis undisclosed)& VR Chat& one to two times a month\\ 
    \midrule
    
      \textbf{P9}&    28/M&   White, Asian&   Autism (nonverbal); Learning Impairment with Linguistics (text); Bipolar Type One&  VR Chat&  "extensive"; 5000-6000 hours\\ 
    \midrule
    
      \textbf{P10}&    52/F&  White&  Hashimoto's Disease; Social Anxiety (contextual); Osteoporosis&  VR Chat, Synth Riders& "live on there" - work, sleep, "addiction"\\ 
    \midrule
    
      \textbf{P11}&    28/M&  Black& ADHD (undiagnosed)&  Altspace VR; Spatial; Rec Room; Horizon Worlds& multiple times a month\\ 
      \midrule
    
      \textbf{P12}&    31/M&  White&  Asperger's; ADHD& Altspace VR; Oculus; Rec Room; Horizon Worlds& game and therapeutic tool since 2019 \\ 

     \bottomrule
    \end{tabular}
    \label{tab:my_label}
\end{table*}


==> sections/4-findings.tex <==
\section{Findings}
We discovered themes surrounding social VR’s reflection of (and divergence from) non-virtual social environments (4.1), VR avatars’ potential for multimodal self-expression (4.2), and distinctions between public and private disability representations (4.3), as described below. We have also compiled suggestions participants had for increasing the accessibility of customization mechanisms (4.4) and summarized them alongside suggestions derived from 4.1-4.3 (see Discussion). 

\subsection{Convergence and Divergence Between Social VR and Non-Virtual Social Contexts}

Participants noted they often used social VR spaces similarly to non-virtual social spaces. P1 described attending support groups, celebrating birthdays, watching movies and fishing in social VR. P2 indicated she feels her virtual and non-virtual social interactions are equivalent, elaborating: 
\begin{quote}
 \textit{``To engage with others while they’re doing something active in the same way you are is very similar to if I was gonna go fishing with somebody in real life. It’s the same, like being able to join a party with some of my friends and go fishing with them together in VR.”} (P2, f, 32 years old) 
\end{quote}

VR affords such a breadth of social experiences that it can facilitate much of users’ daily social interactions. P7 shared, \textit{``VR is an interesting experience. Kinda really the majority of the socialization I do these days.”} For some participants, virtual platforms provide essential access to social environments when their invisible disabilities prevent them from leaving home. P7 explained: 
\begin{quote}
\textit{``What I'm getting out of VR is a little different than what most people get out of VR. They get in there, and they want to [play games]. I'm there so that the world doesn't close in on me. I'm there to keep a tiny little porthole of the world open to me. Even though I cannot physically be in it, I can virtually be in it. You know, I can visit a museum through VR. I went up on the space station through VR. I've gone scuba diving in VR. And the social aspects. I've met friends who have been my friends for years, but we live in different states. And we've come together.”} (P7, f, 33 years old) 
\end{quote}

While many users opt to engage in social games, not all social VR contexts are casual. For P6, who maintains an avatar for work purposes, there are distinctions between how she approaches avatar customization in social and professional environments. 
\begin{quote}
\textit{``I care a lot more about what my avatar looks like if I am engaging professionally for sure, because if I’m playing ping pong with my dad, I'll just use the default avatar or show up as a cat…But yeah, professionally, I manage it similarly to how I would dress if I were going to this event in-person professionally versus if I'm just hanging out with my dad.”} (P6, f, 24 years old) 
\end{quote}

Social VR is home to diverse spaces that can offer experiences ranging from relatively safe communities to potentially harmful environments. P1 points out:  
\begin{quote}
\textit{``Personally, I’m totally fine with having [disability representations] on all the time. But I really understand why somebody would want to have an option to turn it off, especially if you're going into more of a rough and rowdy crowd, like in VR Chat. You don't want to make yourself a target for people that might look for things to hurt you with. For a lot of the communities I hang out in on social VR platforms, typically, I know the people hanging out there are going to be more kind, empathetic people. But if you're going to a place that you don't really know very well, I think it would be a good idea to be able to turn that off or on.”} (P1, f, 32 years old) 
\end{quote}

Participants identified connections between the intersecting lenses of disability, gender and race, which remained salient across virtual and non-virtual domains. For example, P12 compared disclosing invisible disabilities to disclosing sexuality and gender identity. He cited the clothing choices of LGBTQ attendees at the Tony Awards as an example of ways queer people expressed and disclosed their identities visually in non-virtual spaces. Relating this practice to his representations of his Asperger's and ADHD in virtual avatars, he described using clothing and accessories to represent his identity in implicit but visual ways. 

Despite some marked similarities between the virtual and non-virtual domains, several participants perceived social VR to be a relatively safer domain than non-virtual environments. P9 felt more open to disclosing his disabilities in social VR because, unlike in the non-virtual world, he felt a disability label would not persist beyond the present VR experience. P9 explained: \textit{``I feel like once I label myself [with a disability] in real life, it becomes something that kind of follows you around.’’}

P12 expanded on how situational disclosure might be impacted by the VR context: 
\begin{quote}
    \textit{``I don't mind disclosing, but it's on a situational basis, especially based on the virtual environment in the case of VR versus a real-life environment. I mean, I'll even give you a small example. There are times when I maybe wouldn't necessarily disclose my disability in real life if, say, I'm stressed, but I would just tell the person I'm interacting with if I personally notice myself interacting that way. That's something else with my disability, I noticed. Sometimes, I will be self-aware of how I'm feeling and how I'm interacting, but other times, it will just be impulsive, and it will feel like a blur.’’} (P12, m, 31 years old)
\end{quote}

P3 unpacked more of the nuances behind transforming non-virtual representations into embodied VR environments, indicating the factors that contribute to her decision about the extent she wants to represent herself in VR: 
\begin{quote}
\textit{``My VR Avatar is whatever I'm feeling at the moment. If I'm feeling immersed in my invisible illness, then I'm probably gonna want my avatar to be also. And if I'm feeling like, ‘okay, I'm escaping reality,’ I don't want my avatar to be even close to what I am. [In safe environments,] there will still be some days that I don't want to manifest that. And then other days where it's like, ‘yeah, I'm feeling like crap and I'll let you people know it in a non-verbal way,’ and I will come in there all crippled up with my avatar, altered to represent how I feel right now simply because I am trying to communicate it in a nonverbal way.”} (P3, f, 56 years old)
\end{quote}

P3 noted the importance of having the option to accurately reflect her non-virtual self, in a way normalizing the uncanny valley effect of embodied avatars that are: 
\begin{quote}
\textit{``A way I might have looked once upon a time. They keep me from aging…I’m not the type of person who changes [my avatar] all the time, and it puts me in a little suspended animation where I haven’t aged in six years.”} (P3, f, 56 years old)
\end{quote}

P3 elaborated on customizable avatars’ psychological role in grounding her VR experiences: 
\begin{quote}
\textit{``[Having options] gives you virtual reality with just a little bit more normalcy. Just enough normalcy to make me go, ‘Okay, I'm not gonna run from this. It's not so foreign that it's freaking me out.’...It gives you a little bit of an anchor to not overwhelm you.} (P3, f, 56 years old)
\end{quote}

\subsection{Multimodal Self-Expressions through Facial Expressions and Body Language}
VR allows for multimodal self-expression, an important affordance when participants described current and imagined preferences for disability representations on social VR platforms. 

P9 emphasized embodied avatars’ connections to his mood, especially when expressing his experience of Bipolar Type 1. He used VR avatar appearances, and especially their colors, to communicate his emotions nonverbally, strategically selecting avatars based on his goals for social interactions that day. When sharing screenshots of his current avatars, he explained his use of visual affordances and their social and psychological effects: 
\begin{quote}
\textit{``The middle avatar is the avatar I use when I’m in a playful mood. It stands out, but it's also really friendly looking. I got a lot of people that like to hang around with me in this one if I'm feeling energetic, a little bit extroverted. If we talk about bipolar phases a little bit more, like the maniac phase, I'll use the middle one. … Yeah, I like to rotate between these five. I kind of think of it as ‘How can I best express myself and kinda let others know how I’m feeling based on the avatar?’ If I’m in a really happy mood, but I pick an avatar with like no color, for few emotions, it wouldn't really match. Same thing vice versa. It also adds some novelty to VR chat as well, because if I see myself in the same avatar for too long, I feel like I start to get fixed. I start to lock myself in the avatar. So, I like to mix it around so I know there's always flexibility to iterate and change.”}  (P9, m, 28 years old) 
\end{quote}

P9 and other participants also described more of the physicality of communicating in social VR spaces. P9 spoke to the value of facial expressions: 
\begin{quote}
\textit{``I am quite expressive myself, but my invisible disability is nonverbal autism, so I wouldn't actually say what I’m feeling. I would express it through my avatar’s facial expressions. Sometimes, the number of expressions on an avatar goes as high as 30 or 40 different options. So having many different options to express myself nonverbally is a way that I can get more synchronized and comfortable using an avatar.”} (P9, m, 28 years old) 
\end{quote}

P2 hadn’t personally used the facial expressions feature of newer VR headsets but was familiar with it through friends who have shared their experiences: \textit{``Avatars already blink. They talk, they cry…When you smile, it makes the avatar smile, or when you furrow your brows it matches your facial expressions more.”} Though P2 expressed amazement at the current state of technology, she also shared some ideas for future development, including dynamic representations of energy: \textit{``An energy bar, like in a video game where you have your life meter. If it’s full, you're full of energy, and it's all the way green…And if I'm really low on energy, I've got a red bar.”} 
\begin{quote}
\textit{``Let's say I'm feeling excited or hyper. Your avatar can have a really upbeat energy to it if you're going to apply an energy to an avatar. Or if you can put in there that you're feeling slightly depressed, or that you have a low mood or that you're tired, your avatar would be a little bit lower on the energy…That way my friends could see me and then go like, ‘Oh, that's kind of the mood she's in. Let's cheer her up.’ Or, ‘Let's just give her her space.’ And they see you come in in this perky mood, and then they can kind of match their energy to your mood without you having to be so vocal about it.”} (P2, f, 32 years old) 
\end{quote}

Like P2, some participants focused their representation ideas around the movement aspect of embodied avatars. P4 shared an anecdote about the inconvenience of embodying a cat and having your avatar’s eye line low to the ground when engaging with human-sized avatars. P12 wanted to utilize two aspects of VR’s multimodality, voice and movement, for disability expression. \textit{``If I am going to disclose my disability on the platform, it would be more verbally or through using the VR controllers when I'm controlling the hands of the avatar.”} P3 described the use of VR avatar movement to facilitate community support with a physicality unique to embodied contexts. \textit{``Sometimes, our avatars will run over and give somebody a group avatar hug when they're having a particularly bad time, and I'll run over and do that.”} (P3, f, 56 years old) 

P9 summarized VR’s multimodal affordances and identified distinctions between the digital and virtual domains: 
\begin{quote}
\textit{``I'd say [VR] is an order of magnitude above anything you would see on Instagram – anything you see on any other website – because those are just two-dimensional, static images or videos. Can't interact with photos, but when you're there in virtual reality, you can see all the details on the avatar show this person is expressing themselves. See their facial expressions, their movements and their body language. And it's real-time. No other kind of social platform comes even close to VR.”} (P9, m, 28 years old) 
\end{quote}

Speaking to the affordances of other extended reality technologies (i.e., augmented reality, mixed reality), P10 wanted to take her embodied avatar from social VR and use it as her self-representation in mixed-reality social media content. 

\begin{quote}
    \textit{``Yeah, I just wish they had a lot more options for stuff. Well, I’m hoping they grow in [mixed-reality] when they come out with the next [headset], because I heard through the grapevine it's supposed to be more for mixed-reality. I would actually love using an avatar instead of my real body in my YouTube videos.”} (P10, f, 52 years old) 
\end{quote}

\subsection{Public and Private Representations of Disability}

Participants desired options for both public (or explicit) and private (or implicit) identity expression. Suggestions included clothing, accessories, icons, energy bars, or modifications to avatar bodies such as a tail. Some suggestions included both public and private meanings.

To start, participants suggested incorporating customizable clothing and patterns that featured disability-related logos. For example, P1 wanted to have an avatar wearing a zebra-print shirt and beret to advocate for Rare Disease Month. Similarly, P4 suggested an explicit representation for communicating the experience of dyslexia through apparel or logos: 

\begin{quote}
    \textit{``[On clothing,] have the word dyslexia, but then have it jumbled up so people can see what it looks like when we try to read. Then, they'll be like, `Whoa, that's not fun.’ And we're like, `Well, welcome to my hell.’ Make it a joke, but also kind of be like, `Hey, this is really what it feels like.’ } (P4, f, 38 years old)
\end{quote}

Just as P4’s suggestion combined personality and humor to inspire avatar-based education and disability advocacy efforts, P12 wished to express his personal style and disability status through a \textit{“little cool jacket [with] a label…to say my name and that I have Asperger’s and whatnot.”}

Other participants wanted customization libraries to include assistive technology (e.g., wheelchairs, canes, crutches, hearing aids), an assortment of chronic-illness specific items (e.g., a brooch that says \textit{``POTS’’}, P6), a medical alert bracelet, and \textit{``spoonie’’} gear like a giant spoon, P1) to disclose their disabilities. 

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{imgs/P1.png}
    \caption{Participant 1’s drawings and suggestions for invisible disability representation during the whiteboard component of the study, featuring a giant spoon to represent spoon theory and other assistive technologies to disclose their disability.} 
    \Description{Participant 1’s drawings and suggestions for invisible disability representation during the whiteboard component of the study. At the far left, there is a floating medication reminder inside a speech bubble that represents a floating emote. Below are examples of assistive technology such as a cane and hearing aids. Next is a person’s outline wearing a zebra print beret and shirt to represent rare disease month. The shirt also has a space for a custom disability graphic or a fact about the participant’s rare disease, both aimed at spreading invisible disability awareness. The person also wears a medical alert bracelet and carries a human-sized spoon to represent desired “spoonie” props that point to identification with spoon theory. Finally, there is a note where there would be a floating menu to enable and disable disability-related accessories.}
    \label{P1}
\end{figure*}

P11, a designer by trade, drew on his experience with video games to suggest ways to represent his disability through icons: 

\begin{quote} 
    \textit{``It's probably influenced by video games and Internet culture…where there's so much going on the screen in front of you, and you can't really remember what every icon means. … So “I” is Information…You click that…and the general notice is also a symbol…because of the sensitivity of the types of people involved. This universal image for neurodiversity.”.”} (P11, m, 28 years old)
\end{quote} 

Notably, P11 described the importance of the transient nature of this representation in facilitating social interactions:

\begin{quote} 
    \textit{``I would imagine that when the user clicks [the "I"] the image pops up for only a few moments in time, right?...That way, you can continue your interactions and virtual space without necessarily having the label on you constantly.”} (P11, m, 28 years old) 
\end{quote} 

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{imgs/P11.png}
    \caption{Participant 11’s images, sticky notes, and suggestions for invisible disability representation during the whiteboard component of the study, featuring an information icon and the ADHD rainbow butterfly symbol above the avatar.} 
    \Description{Participant 11’s images, sticky notes, and suggestions for invisible disability representation during the whiteboard component of the study. There is an image of Toad, an anthropomorphized mushroom character from the Mario franchise, wearing an astronaut suit and helmet. On his cap, there is an information icon (a lowercase i in a circle) and above Toad is the ADHD rainbow butterfly symbol. To Toad’s right, there is a sticky note that reads, “General notice of invisible disability - other users can click to reveal more information. More information is presented as a specific symbol represen-”. To the right of the ADHD symbol, there is a sticky note reading “Symbol is animated and hovers on top the avatar for a few seconds after the (i) button is clicked.”}
    \label{P11}
\end{figure*}

Some participants (P2, P6) were interested in disability representations that floated above their avatars, such as an awareness flag or a dynamic energy bar that correlated with their energy level (or “social battery”). As an accommodation feature, this interfaces interestingly with P11’s proposal of a feature that would allow an avatar to turn invisible when its user wants to avoid social interactions. Turning invisible would convey non-verbally that a person does not want to be approached.

However, P11 quickly engaged critically with the potential implications of implementing such a feature: 

\begin{quote} 
    \textit{``If you think about the other users of the space, do you really want an invisible person watching you? … Maybe there will have to be some sort of general notice that says: "Beware, there are invisible people in this space," which kind of seems creepy...Maybe rather than being invisible, you can have a grayed out version of your avatar. So my little toad astronaut, who’s red and blue, right? I can just make him more white instead, [meaning,] ‘Just don't come to me. He’s not really colorful right now.’”} (P11, m, 28 years old) 
\end{quote} 

This specific example speaks to the uniqueness of the embodied experience that social VR offers its users. It highlights an affordance impossible in the physical world, which offers humans an option to change colors like a chameleon. This idea furthers the theme of avatars affording novel self-expression through non-humanoid embodiment. Below, we describe how participants explored representations infused with personal meanings that are as invisible as their disabilities. 

For example, P8 gave his avatar earbuds during the creative exercise, explaining: \textit{``I’m not a big earbud guy, I'm a headphone wearer… [but] I feel like maybe it would be an extension of trying to conceal what invisible disabilities I would have, just pretending to be normal with stuff like that.”} While this representation of his invisible disability was not explicit to others, he acknowledged that his avatar was \textit{``more of an expression of [him].”} and preferred to keep this aspect abstract. 

Similarly, P3 preferred more subtle accessories that more closely resembled non-virtual affordances: \textit{``I would do it with accessories, [but] I don't want a big sign saying `disabled’ or a different color flashing over here that says `invisible illness is no longer invisible.’ I would do it with subtle accessories. Something a little more real.’’} 

Speaking of “real” accessories, or those rooted in non-virtual environments, P12 wanted to  use clothing or accessories that blurred private and public significance:

\begin{quote}
    \textit{``For me, I utilized my interest in cars as both something to do therapeutically but also maybe relate to others that have that same interest. Which is why I also, in real life, like to collect diecast cars and books on cars, and sometimes, I also like to wear clothing with cars on it. This is more of a social preference. I don't know how that would represent my disability entirely, but if [others] at least understand my passions and interests and how knowledgeable I am about them, then maybe they have a better understanding of me, too. On a personal level, at least.”} (P12, m, 31 years old)
\end{quote} 

Two other participants (P5, P9) were interested in representations of personal significance rather than using them exclusively to communicate with other users. For example, P9 used vibrant colors: \textit{``It's a way that I can visually differentiate myself from a room full of other people. It's my way of not just indicating to others that this person’s a little different, but it's also indicating to myself that I'm a little different.”}

P9 also established his interest in using his social VR avatar to tell a complex narrative through accessories: 
\begin{quote}
    \textit{``I really want to add knee and elbow pads. If you have ever gone roller skating, you need to put on knee and elbow pads, just in case you fall... The bipolar makes me swing really hard to the left and right. I get these mania phases and these depression phases that have a whiplash to them. And sometimes... I can get hurt or accidentally hurt others. So these pads on my knees and elbows would be a way to symbolize that if I do fall, I gotta make sure I'm protected. I don't fall too hard, and I can stand up again.’’} (P9, m, 28 years old)
\end{quote}  

On another note, P10 expressed that her avatar represented her comfort zone and personal bubble, a current customization option she valued: 

\begin{quote} 
    \textit{``Its tail wraps around it a lot as it's moving, or if you stand still… but I like that one because, in some weird way, it gives me a comfort zone of hiding me in a bubble. I don't know, I never found one that did that. So, when I came across that one, I just liked it. Even in real life, people have said I have a bubble, like a huge bubble around me. It’s like you get too close to me, and I’m kinda like… I just back away a little.”} (P10, f, 52 years old)
\end{quote}

P10 described using her humanoid and avatar-based self-expression as a metaphor for her non-virtual personality, further emphasizing the unique affordances of social VR in expanding the bounds of self-expression by allowing fantastical and metaphorical representations of the self. 

While P5 suggested glowing veins could represent chronic pain, he acknowledged that other users might not understand the disability-related symbolism: \textit{``[The glowing veins] would show things more, but they still wouldn't even show pain, because people are gonna look at that and just go like, ‘cool.’ They just see glowing things on your arm.’’} 

To P5’s point, these private and often implicit representations of disability were valuable to participants even though most other social VR users would not make the logical leap necessary to understand that a disability was being expressed.  

\subsection{Suggested Features for Customizing Disability Representations}

Five participants (P1, P2, P4, P5, P7) expressed interest in easier processes for importing and creating custom designs. P4 suggested: \textit{``It'd be nice to have different options with different logos or quotes you want to put on shirts. It'd be nice to have a set-up so that you can do it pretty easily [because] I definitely don't have the coding experience to be able to go any further.’’}

Even though invisible disabilities often have unrecognizable and misinterpreted features, some have physical manifestations that can impact mobility. P5's constrained arm movements due to a Repetitive Strain Injury shaped his vision for an ideal customization process. He wanted to minimize arm movement requirements and shared ideas for optimizing user experiences through evolving technology: 
\begin{quote} 
    \textit{``I could copy and paste it. That's my ideal customization because I don't like the menus. If you have the option of pressing a bunch of buttons or just being able to think it and it appears on the page, why would anyone want to have all the billion options when they could do the exact same thing? It has occurred to me, though, like with the recent AI developments, where you can produce pictures, it seems like it's not too far away they could just produce a 3D model using those systems. Like if there was a system where you could describe it, and it would generate one.’’} (P5, m, 31 years old) 
 \end{quote}

P11 also had a wealth of ideas for ways to customize avatars, including: \textit{``Simple sliders and buttons…3D models you can customize…options to select what types of disabilities and neurodivergent conditions you identify with, and then you get a chance to customize the symbols or the icons.”} He further explained: \textit{``I think an ability for you to type in what you’re saying or what you want through image generation or text-to-3D tools would be a great way to do that,”} which would reduce the burden of users navigating complex customization systems within social VR systems. Participants also mentioned that text-to-avatar pipelines could lower the barrier to avatar customization, which was perceived as intimidating for participants without coding experience.

==> sections/5-discussion.tex <==
\section{Discussion}
In our study, we found that people with invisible disabilities are interested in representing their disabilities through social VR avatars. Unlike people with visible disabilities, who often want to depict disabilities through adding assistive technology to their avatars \cite{zhang_diarystudy}, representations of invisible disabilities tend to adopt more nuanced and symbolic approaches,  including clothing-based designs (such as disability-related graphics) and accessory-based features (such as a floating energy bar). Additionally, a distinction emerged between public representations with explicit meaning and private representations with implicit meaning. Sometimes motivated by educational and awareness-raising goals, sometimes motivated by traumatic non-virtual disclosure experiences, we discovered that social context informed participants' virtual disclosure preferences. It is important to note that social VR offers users a distinct set of verbal and non-verbal cues that can powerfully communicate shifting needs and preferences. Through recommendations that utilized the multimodal interactions uniquely afforded by social VR avatars (e.g., synchronous voice chat, motion tracking, facial expressions), we found participants moved beyond solely visual representations of disability. 

\subsection{Multimodality as an important distinction between embodied and non-embodied contexts.}
We found disability disclosure preferences often vary by context and disability, a nuanced choice that becomes more pronounced with social VR embodiment and real-time immersion \cite{freeman_maloney_perception_of_self}. Mack et al. \cite{mack_towards} explored contextual differences across digital gaming and social platforms such as Roblox and Snapchat. They focused on non-embodied avatars, and they found that non-digital experiences can inform expectations of digital spaces. Similarly, though we examined different types of avatars, we discovered non-virtual experiences inform virtual preferences. One major distinction that arose was VR's facilitation of both social engagements and professional interactions that might mirror non-virtual experiences. VR is uniquely able to map non-virtual experiences (e.g., fishing) onto virtual interfaces in ways that feel synchronous and immersive to users.  We attribute this to P9's acknowledgment that the added levels of sensory engagement afforded by social VR can greatly influence avatar perceptions. Since embodied avatars are the predominant form of self-expression in social VR, mediating all social encounters, it is imperative that users have maximum flexibility in representing their identities in ways that are personally meaningful. We extend prior findings on invisible disability representation by examining social VR’s multimodal affordances for identity expression. While social media limits disability disclosure to 2D visuals and text, social VR offers multiple channels for sensory-based expression in addition to dynamic disability representations (e.g., a floating energy bar that represents a user's energy level during embodied social interactions). 

\subsection{Enabling adaptive disability representation for context-specific needs.}
Based on our findings, we recommend that social VR platforms allow users to toggle disability representations on and off. Deciding whether to disclose is an ongoing negotiation across both digital (non-embodied) and virtual (embodied) platforms. In the context of embodied social VR, a recent study revealed that avatars with disability representations were more likely to experience ableism and harassment during group social interactions \cite{zhang_diarystudy}. As such, it is important to offer an easy-to-use toggle on and off feature with disability representations so users can operate with the utmost autonomy in their avatar disclosure decisions. At present, avatar design processes are complex. Customization platforms such as Ready Player Me \cite{readyplayerme} offer “hundreds of options” but are often inaccessible to people from non-technical backgrounds. To streamline the customization process, we suggest that avatar design processes implement more built-in options relevant to invisible disabilities so that invisible disability representation is also accessible for users from non-technical backgrounds. Further, taking inspiration from participant suggestions like the dynamic energy bar, we suggest that future avatar designs incorporate intuitive and universally applicable design conventions (e.g., traffic light color guidelines \cite{traffic_light}), to allow users to effectively express themselves.

Our findings support preliminary discussions of invisible disability representation in avatars by offering actionable implementations of disability expression across various modalities. We believe the creativity of our participants' recommendations for invisible disability representation speaks to VR's diverse affordances. Their suggestions spanned a range of implicit and explicit meanings, ranging from accessories with highly specific personal metaphors to apparel that transmits more communal awareness-building efforts. We hope VR designers can take these recommendations and apply them to customization library offerings as well as avatars' physical movement affordances. See the list below for a more detailed summary of suggestions based on our findings. 

\subsection{VR Customization Design Recommendations} 
Based on our findings, we offer the following list of design recommendations to VR designers: 

\begin{enumerate}
\item \textbf{Create more options for multimodal customization.} 
        \begin{itemize}
            \item For some users with invisible disabilities, certain forms of communication are more accessible than others (e.g., verbal, visual, etc.). 
	\item Allowing users to fine-tune their movements and facial expressions can facilitate avatar-based representations of accommodations needs as well as communicate dynamic capacities for social interaction. By offering these options, social VR platforms can maximize new opportunities for making social VR a better experience for users with invisible disabilities.
        \end{itemize}
\item \textbf{Include explicit (i.e., public) options for invisible disability representation on social VR customization platforms.} 
        \begin{itemize}
            \item Even though some participants suggested highly individualized representation ideas, \textbf{we recommend including awareness-building apparel and accessory options in customization libraries} (e.g., zebra print for rare disease month, dyslexia-related t-shirt designs, spoon accessories for representing chronic illness) as a first step. Navigating customization can be challenging for multiple reasons (see examples below), so offering a number of pre-set invisible disability representation features can help eliminate barriers to boosting awareness and facilitating self-expression. Our findings offer a generative set of ideas. As a next step, it might be helpful for designers to research more disability awareness symbols and calendar events (e.g., awareness months) to guide their inclusion of community representations. 
        \end{itemize}
\item \textbf{Make the avatar customization process more accessible.}
        \begin{itemize}
            \item Many social VR users \textbf{do not have the programming background} necessary to manually fine-tune more individualized customization features like those that might implicitly represent invisible disabilities.
            \item People with invisible disabilities want to be able to \textbf{upload custom apparel logos and t-shirt designs} that represent their disabilities. 
            \item Because of the \textbf{personal significance of many suggested disability representations}, a number of invisible disability-related customizations would need to be individually uploaded by social VR users.
            \item Consider ways to \textbf{minimize or remove the physical burden of swiping} through long lists of customization options to enhance accessibility, including customization by way of text or drawing. 
        \end{itemize}
\end{enumerate}



==> sections/6-limitations.tex <==
\section{Limitations}
The study was somewhat limited by challenges in the recruitment process. Due to the invisible nature of the disabilities in our population of interest, participants had to feel comfortable disclosing their invisible disability to engage in the interview. We also considered that some people with chronic illnesses, neurodivergence, or other invisible disabilities might not identify as having an invisible disability. To address this possibility, we altered our language in different rounds of recruitment, ensuring we included examples of invisible disabilities in every note. Additionally, because we only included consenting adults ages 18+ in the present study, we were unable to connect with the large population of youth and teen VR users and gamers. Understanding that age, among other characteristics, might mediate disclosure preferences, future work could benefit from examining its impact. Ultimately, we recruited a strong sample of 12 participants who shared many overlapping experiences while also bringing to their interviews diverse suggestions and rich viewpoints. We halted recruitment once thematic saturation was achieved. While this study relied on thematic analysis as its core analytical method, we believe there are generative methods of triangulating these findings that can build upon this work in future (e.g., implementing the design recommendations from this study for users to test).  

Given that we recruited from primarily (though not entirely) U.S.-based mailing lists, we recognize the geographic limitations of this study and acknowledge the importance of situating findings in diverse cultural and socioeconomic contexts. We understand that disability representation preferences, especially those linked to established symbolism, are culturally and geographically dependent. For example, while symbols like spoon theory’s spoon are globally recognized for representations of invisible disability, others, like the Australian use of the sunflower on apparel and accessories, are less universally known. Though we recruited from organizations, listservs, and social media threads globally (with some exceptions due to legal restrictions), our present demographics collection process did not include the participant country of origin.  We acknowledge that future projects would benefit from a more globally situated and culturally sensitive lens. 



==> sections/7-conclusion.tex <==
\section{Conclusion}

Avatars mediate interpersonal interactions between social VR users, but at present, no built-in options exist for people to explicitly represent invisible disabilities. In this study, we explored the avatar customization preferences of people with invisible disabilities. Users wanted to tap into VR’s multimodal affordances (e.g., facial expressions, body language) to communicate their invisible disabilities. More broadly, users were interested in representing their invisible disabilities through various explicit avatar features (e.g., clothing, floating icons), and many expressed a need for an easily usable mechanism that could toggle disability representations on and off in different contexts. Interestingly, there emerged a distinction between public and private representations of disability, introducing a new level of nuance to our prior understanding of what it means to represent disability. We offer a new perspective that takes into consideration the importance of personal significance during self-expression, in addition to explicit and widely understood symbols for invisible disabilities. To our knowledge, this is the first study to focus solely on the avatar representation wants and needs of social VR users with invisible disabilities. Broadly, our findings contribute to the ongoing conversation of designing with and for people with invisible disabilities. We hope this study inspires more researchers to offer future contributions to the valuable study of invisible disability representation and accessibility in VR. 


==> sections/diff.tex <==
\section{Introduction}
Like anyone else, people with disabilities want to represent their unique identities through their avatars when interacting with others in social \DIFdelbegin \DIFdel{VR }\DIFdelend \DIFaddbegin \DIFadd{virtual reality (VR) }\DIFaddend spaces. Among other functions, avatars are vessels for self-expression in VR \cite{freeman_maloney_perception_of_self}, and their characteristics provide cues that mediate interpersonal interactions. Social VR platforms offer users a strong sense of embodiment and freedom from some forms of physical constraint, and as more people turn to social VR for social connection, the importance of diverse mechanisms for self-expression grows \cite{falling_asleep, yalon_leisure}. However, \DIFdelbegin \DIFdel{more work needs to be done to understand what kinds of avatar representations can highlight disability identities accurately despite stigma, }\DIFdelend given the varying needs of potential users of social virtual reality spaces\DIFaddbegin \DIFadd{, the accessibility community has yet to understand what kinds of avatar features  can authentically represent diverse disability identities}\DIFaddend . 

Previous research has investigated the avatar representation preferences of people with visible disabilities (e.g., \DIFdelbegin \DIFdel{deaf}\DIFdelend \DIFaddbegin \DIFadd{d}\DIFaddend /\DIFaddbegin \DIFadd{Deaf and }\DIFaddend hard of hearing people\DIFdelbegin \DIFdel{and }\DIFdelend \DIFaddbegin \DIFadd{, }\DIFaddend blind and low vision people) in social VR platforms. Zhang et al. \cite{zhang_partofme} found \DIFaddbegin \DIFadd{that }\DIFaddend users with visible disabilities wanted to use their avatars to disclose their disabilities, highlight their \DIFaddbegin \DIFadd{access }\DIFaddend needs, and raise awareness through their VR interactions. Some desired to incorporate components like signing ASL through their avatars and adding realistic and customizable assistive technology (e.g., hearing aids) to better align their avatar representations with their non-virtual self-presentations. 

However, many \DIFdelbegin \DIFdel{people with disabilities }\DIFdelend \DIFaddbegin \DIFadd{disabled people }\DIFaddend do not have characteristics that are immediately visible, nor do they use \DIFaddbegin \DIFadd{commonly recognized }\DIFaddend assistive technologies. \DIFdelbegin \DIFdel{Indeed, there are }\DIFdelend 33 million people in the \DIFdelbegin \DIFdel{U.S. alone who have such }\DIFdelend \DIFaddbegin \DIFadd{United States alone have }\DIFaddend invisible disabilities (approximately 10\% of the U.S. population) \cite{disabledworld}. \DIFdelbegin %DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdelend Mack et al. \cite{mack_towards} \DIFdelbegin \DIFdel{was the first to examine avatar representations of }\DIFdelend \DIFaddbegin \DIFadd{examined the avatar representation preferences of people with visible and }\DIFaddend invisible disabilities through a broad study of \DIFdelbegin \DIFdel{both visible and invisible }\DIFdelend disability representation on digital platforms (e.g., Snapchat, Animal Crossing, Facebook). They found that users with visible disabilities wanted to implement representations of their non-virtual bodies and assistive technologies, while users with invisible disabilities wanted to use disability-related avatar symbols (e.g., words in the dyslexia-friendly font “Bionic”) to signal membership in a specific community. This distinction in preferences supports the idea that representation needs differ between visible and invisible experiences, highlighting the importance of \DIFdelbegin \DIFdel{delving further into }\DIFdelend \DIFaddbegin \DIFadd{further understanding }\DIFaddend the avatar representation wants and needs of \DIFdelbegin \DIFdel{users with invisible disabilities }\DIFdelend \DIFaddbegin \DIFadd{invisibly disabled users }\DIFaddend in technology-mediated contexts. 
\DIFaddbegin 

\DIFaddend Avatars provide users with invisible disabilities an opportunity to make their invisible identities visible through affordances that are not available in the non-virtual world. \DIFdelbegin %DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{However, Mack et al. \mbox{%DIFAUXCMD
\cite{mack_towards} }\hskip0pt%DIFAUXCMD
did not explore }\DIFdelend \DIFaddbegin \DIFadd{However, prior work has not yet explored invisible disability representation in }\DIFaddend embodied avatars like those found in social VR spaces. \DIFdelbegin \DIFdel{Preferences regarding embodied avatars are likely to be different because VR’s affordances for capturing the nuances of physical human expression far exceed digital platforms \mbox{%DIFAUXCMD
\cite{freeman_maloney_perception_of_self}}\hskip0pt%DIFAUXCMD
. }\DIFdelend On digital platforms, users are limited to 2D, static images of their avatars. Conversely, social VR users use embodied 3D avatars to represent themselves\DIFdelbegin \DIFdel{, which }\DIFdelend \DIFaddbegin \DIFadd{; VR avatars }\DIFaddend are capable of capturing much more granular nuances, extending as far as dynamic facial expressions\DIFdelbegin \DIFdel{and body language}\DIFdelend \DIFaddbegin \DIFadd{, body language, and movement patterns }\DIFaddend as they socialize with others. \DIFaddbegin \DIFadd{Given that VR’s affordances for capturing the nuances of physical human expression far exceed digital platforms \mbox{%DIFAUXCMD
\cite{freeman_maloney_perception_of_self}}\hskip0pt%DIFAUXCMD
, more research is needed to understand invisibly disabled users’ unique preferences for identity representation in embodied avatars and social VR spaces. 
}\DIFaddend 

In this paper, we \DIFdelbegin \DIFdel{expand on }\DIFdelend \DIFaddbegin \DIFadd{extend }\DIFaddend previous work by examining the embodied avatar preferences of people with invisible disabilities, amplifying the voices and experiences of this marginalized group within \DIFdelbegin \DIFdel{the }\DIFdelend \DIFaddbegin \DIFadd{a }\DIFaddend social VR context\DIFdelbegin \DIFdel{for the first time}\DIFdelend . To broaden our understanding of how we can best construct the offerings of a disability-inclusive avatar customization library, we \DIFdelbegin \DIFdel{conducted an interview study that }\DIFdelend investigated how people with invisible disabilities \DIFdelbegin \DIFdel{present, and may }\textit{\DIFdel{want}} %DIFAUXCMD
\DIFdel{to present, their identities in }\DIFdelend \DIFaddbegin \DIFadd{currently represent themselves, their desired representation mechanisms, and how these preferences might differ across }\DIFaddend social VR contexts. Specifically, we posed the following research questions: 

\begin{itemize}
	\item \textbf{RQ1:} How do \DIFaddbegin \DIFadd{embodied vs. non-embodied avatars differ, and how do  those differences impact identity representation?
	}\item \textbf{\DIFadd{RQ2:}} \DIFadd{How do }\DIFaddend people with invisible disabilities represent \DIFdelbegin \DIFdel{disability in avatars today}\DIFdelend \DIFaddbegin \DIFadd{their disability identities in social virtual reality avatars today, and how do they wish to represent themselves on social VR avatars}\DIFaddend ?
	\item \DIFdelbegin \textbf{\DIFdel{RQ2:}} %DIFAUXCMD
\DIFdel{How can avatars better represent the experiences and identities of people with invisible disabilities?
    }%DIFDELCMD < \item %%%
\item%DIFAUXCMD
\DIFdelend \textbf{RQ3:} \DIFdelbegin \DIFdel{When, why and how do people want to share invisible }\DIFdelend \DIFaddbegin \DIFadd{In what social VR contexts (when and why) do people with invisible disabilities wish to disclose their }\DIFaddend disability identities and experiences\DIFdelbegin \DIFdel{using avatars}\DIFdelend ?
\end{itemize}

We conducted semi-structured interviews with \DIFdelbegin \DIFdel{12 }\DIFdelend \DIFaddbegin \DIFadd{14 }\DIFaddend participants with invisible disabilities\DIFaddbegin \DIFadd{, }\DIFaddend such as ADHD, dyslexia, and rheumatoid arthritis. During the interviews, we included \DIFdelbegin \DIFdel{a visual }\DIFdelend \DIFaddbegin \DIFadd{an interactive }\DIFaddend brainstorming component where participants drew\DIFdelbegin \DIFdel{an }\DIFdelend \DIFaddbegin \DIFadd{, typed, or otherwise visualized their }\DIFaddend \textit{ideal} avatar self-representation, going beyond what is currently available on customization platforms. Understanding that verbal brainstorming often privileges interviewees who are comfortable generating ideas and expressing themselves through voice, we \DIFdelbegin \DIFdel{wanted }\DIFdelend \DIFaddbegin \DIFadd{chose this method }\DIFaddend to offer an alternative opportunity for self-expression \DIFdelbegin \DIFdel{to }\DIFdelend \DIFaddbegin \DIFadd{and }\DIFaddend accommodate a broader range of communication styles. 

We found that social VR users with invisible disabilities \DIFdelbegin \DIFdel{draw many important }\DIFdelend \DIFaddbegin \DIFadd{drew }\DIFaddend connections and distinctions between virtual and non-virtual social spaces\DIFdelbegin \DIFdel{, which can impact }\DIFdelend \DIFaddbegin \DIFadd{; the embodied nature of social VR impacted their }\DIFaddend disclosure preferences. \DIFdelbegin \DIFdel{In addition, we discovered that while }\DIFdelend \DIFaddbegin \DIFadd{For example, some perceived social VR to be a safer space than non-virtual social spaces and felt comfortable disclosing their disability, while others preferred not to disclose due to prior uncomfortable experiences in social VR. Additionally, while }\DIFaddend some users with invisible disabilities already \DIFdelbegin \DIFdel{customize }\DIFdelend \DIFaddbegin \DIFadd{customized }\DIFaddend avatar appearances to indicate dynamic preferences for social engagement, many \DIFdelbegin \DIFdel{might want }\DIFdelend \DIFaddbegin \DIFadd{wished }\DIFaddend to lean further into customized facial expressions and body language to express their disabilities. 
\DIFaddbegin 

\DIFaddend We also propose a \DIFdelbegin \DIFdel{shift in how we think }\DIFdelend \DIFaddbegin \DIFadd{paradigm for thinking }\DIFaddend about disability representation and \DIFdelbegin \DIFdel{the }\DIFdelend \DIFaddbegin \DIFadd{compare their }\DIFaddend private (i.e., implicit representations like knee pads that symbolize a need for self-protection from bipolar mood swings) vs. public (i.e., explicit representations like disability-related shirt graphics) significance\DIFdelbegin \DIFdel{of these representations. We also provide }\DIFdelend \DIFaddbegin \DIFadd{. Based on our findings, we conclude with }\DIFaddend design recommendations to inform a more \DIFdelbegin \DIFdel{accessible avatar creation }\DIFdelend \DIFaddbegin \DIFadd{inclusive and accessible avatar }\DIFaddend experience (e.g., reducing the amount of arm movement required to scroll through customization offerings).

In summary, we contribute \DIFdelbegin \DIFdel{a discussion of avatar customization opportunities to }\DIFdelend \DIFaddbegin \DIFadd{novel insights on how avatar customization can }\DIFaddend support the large and underserved population of people with invisible disabilities, which is another step toward making social VR more inclusive to all users. 
\DIFaddbegin 

\DIFaddend \section{Related Work}
\DIFaddbegin \DIFadd{Despite the invisible nature of some disabilities, identity representation is important. }\DIFaddend Broadly, social VR platforms lack diverse customization options (e.g., regarding body and racial diversity \cite{Lee_2014_Does, lee_whose_2011, Morris_2023_hide}). Invisible disability representation in social VR is \DIFaddbegin \DIFadd{also valuable, but }\DIFaddend even less present. \DIFdelbegin \DIFdel{Despite the invisible nature of some disabilities, identity representation is important. For one, by }\DIFdelend \DIFaddbegin \DIFadd{By }\DIFaddend rendering invisible experiences visible, doors open for building awareness of underrepresented experiences. Further, social VR offers unique affordances for users to represent aspects of their identities in different ways compared to non-virtual contexts \cite{freeman_maloney_perception_of_self}. \DIFaddbegin \DIFadd{We build on prior literature regarding disability disclosure in employment and social contexts, social VR experiences, and avatar customization and identity expression.
}\DIFaddend 

\subsection{Disability Disclosure}
Many \DIFdelbegin \DIFdel{people with disabilities }\DIFdelend \DIFaddbegin \DIFadd{disabled people }\DIFaddend have varied perspectives on when and why to disclose their disability. Although discrimination against individuals with disabilities is legally prohibited\footnote{\DIFdelbegin \DIFdel{The }\DIFdelend \DIFaddbegin \DIFadd{Both the }\DIFaddend Americans with Disabilities Act (ADA) of 1990 and Section 504 of the Rehabilitation Act of 1973 \DIFdelbegin \DIFdel{both }\DIFdelend protect people \DIFdelbegin \DIFdel{with disabilities }\DIFdelend from discrimination on the basis of \DIFdelbegin \DIFdel{their }\DIFdelend \DIFaddbegin \DIFadd{a }\DIFaddend disability.}, \DIFdelbegin \DIFdel{people with disabilities are still subject to discrimination }\DIFdelend \DIFaddbegin \DIFadd{disabled people face discrimination and ableism}\DIFaddend , even if it is unintentional. As a result, they may have to carefully consider whether or not to disclose their disabilities. 

At school and the workplace, people with disabilities may require accommodations to perform their roles successfully, but this disclosure heightens the risk of experiencing disability-related discrimination \cite{lindsay_barriers_education, lindsay_work, wilton_work, schrader_workplace_climate, dalgin_hiring}. They may have less favorable outcomes than their non-disabled peers in the job application process, be socially rejected by their peers and supervisors, and fear being “reduced” to their disability \cite{pearson_job_apps, lindsay_work, lindsay_barriers_education}. They may also fear that disclosure will indirectly impact their academic and professional success due to the damage to their social image \cite{rocco_social}. People with invisible disabilities have been more successful than people with visible disabilities at concealing their disability at their discretion, especially if their condition is mild and they believe their conditions are “irrelevant” to their performance \cite{lindsay_work, schrader_workplace_climate, dalgin_hiring}. 

However, this invisibility also means that people with invisible disabilities struggle to be taken seriously when seeking accommodations. People with invisible disabilities may specifically anticipate negative perceptions stemming from a lack of understanding of their disabilities, which may make them hesitant to disclose \cite{mullins_invisible_uni}. Since invisible disabilities can require more steps to verify than visible disabilities, some people may experience barriers to feeling their disclosure was accepted. Moriña \cite{morina_barriers_education} found that students with invisible disabilities struggled with the stress and insecurity associated with “proving” their disability. Often, they were challenged by people who refused to believe they were “disabled,” which made them want to distance themselves from a disability identity and appear “normal” \cite{morina_barriers_education}. Therefore, while people with both visible and invisible disabilities anticipate and encounter stigma, people with invisible disabilities may struggle more with validating their disability to themselves and others.

\DIFaddbegin \DIFadd{In our work, we extend prior work on disability disclosure in more formal settings, such as in the workplace and in education, and explore the nuances of invisible disability disclosure in social environments. 
}

\DIFaddend \subsection{Social VR Use}
Recently, social VR has gained increasing popularity, enabling immersive 3D virtual experiences by allowing users to meet, interact, and socialize in the form of avatars \cite{freeman_maloney_perception_of_self}. Unlike 2D social media and virtual worlds, social VR uniquely affords immersive embodied experiences \cite{falling_asleep}. VR head-mounted displays allow real-time body movements and gestures to be tracked and rendered in virtual environments. Although most commercial headsets do not track a user’s full body or subtler physical cues, like facial expressions and gaze, they still facilitate a greater sense of embodiment and social presence than other platforms. A person’s sense of embodiment (SoE) is characterized by their ability to control their body’s movements, experience the sensations their body does, and feel that they are within their body \cite{kilteni_soe}. By placing the user within their avatar’s body and mimicking their physical body’s experiences through first-person perspective, body tracking, and haptic and audio feedback, virtual reality facilitates SoE through avatars. Additionally, users can no longer see their physical selves and environments, resulting in them being fully immersed in VR and their virtual bodies \cite{genay_for_real}.

With these unique affordances, social VR platforms offer a variety of avatar-mediated activities and social interactions. To understand what people actually do in social VR, Maloney and Freeman \cite{falling_asleep} interviewed 30 social VR users. Their findings indicated that users enjoyed doing full-body mirroring activities with expressive movements (e.g., dancing), experiencing everyday practices (e.g., sleeping) in novel immersive ways, and practicing self-improvement skills that they normally wouldn’t do in offline worlds (e.g., social skills and mental states). Furthermore, users can connect with other users by hosting and attending parties and other gatherings, playing games together, and working remotely \cite{freeman_maloney_perception_of_self, abramczuk_remote_work}.

Social VR platforms are particularly appealing to people with disabilities since they can address accommodations in ways that go beyond what is possible in the physical world. Virtual reality enables people with physical and intellectual disabilities to engage in active leisure activities, such as horseback riding and swimming, which are typically inaccessible to them in the physical world \cite{yalon_leisure}. Yalon-Chamovitz and Weiss \cite{yalon_leisure} found that \DIFdelbegin \DIFdel{people with disabilities }\DIFdelend \DIFaddbegin \DIFadd{disabled people }\DIFaddend react favorably to VR leisure activities due to their greater sense of autonomy over their bodies and environments. Virtual reality can also be leveraged to help people with invisible disabilities. For instance, in VR, neurodivergent users have greater control over their environment, so they may remove themselves from overwhelming situations or adjust settings to reduce their sensory load \cite{boyd_leveling}. Given its increasing popularity and unique affordances, it is important to understand how people with invisible disabilities want to engage with this social sphere, especially through avatar representation.

\subsection{Traditional and Creative Avatar Expression}
Avatars enable users to develop a greater social presence in social VR. Langener et al. determined that avatar customization heightens the user’s sense of connection and ownership over their virtual body, thus intensifying SoE \cite{langener_embodiment}. Many social VR users choose to represent themselves as accurately as possible through their avatars \cite{freeman_maloney_perception_of_self}. However, avatars can also creatively express their users’ interests and identities, sometimes extending beyond what is possible in the physical world. A myriad of prior works have explored identity and avatar representation in social VR \cite{freeman_maloney_perception_of_self}, including diverse user groups such as racial minorities \cite{blackwell_harassment}, women \cite{sharvit_sexual_harass}, and LGBTQ users \cite{freeman_acting_out, freeman_rediscovering}. For example, Freeman et al. \cite{freeman_maloney_perception_of_self} interviewed 30 people to study their avatar perceptions and found that most of them strove to make their avatars as similar as possible to their non-virtual counterparts because they considered avatars an extension of themselves in virtual worlds. Another study \DIFdelbegin \DIFdel{by Freeman et al. \mbox{%DIFAUXCMD
\cite{freeman_rediscovering} }\hskip0pt%DIFAUXCMD
}\DIFdelend explored the avatar choices of non-cisgender users and revealed that they changed their avatar’s gender expression frequently, through outfits and accessories, to indicate their flexible and gender-fluid identities \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\cite{freeman_rediscovering}}\hskip0pt%DIFAUXCMD
}\DIFaddend .

Unfortunately, current avatar representation options are generally inadequate at capturing the diverse range of human appearances and identities. Marginalized and stigmatized groups are especially under-represented. For example, Ready Player Me, a popular avatar creation tool, presents gender as a binary, which neglects the diversity of gender identity and forces gender-nonconforming people to abide by societal standards \cite{readyplayerme}. Furthermore, the middle-aged female participants in Morris et al.’s study noted that most avatars they encountered skewed towards youthful appearances, and existing avatar customization made them feel like a “caricature” of an older person \cite{Morris_2023_hide}.

Social VR also facilitates significant body modification. Users may opt for fantastical, cartoonish, and non-human features, such as the red eyes and snake eyes offered in Ready Player Me \cite{readyplayerme}. They can also choose non-human avatars \textemdash{} one participant in Freeman and Maloney’s study represented herself as a blue bird \cite{freeman_maloney_perception_of_self}. Furthermore, users can enable complete or partial invisibility of their avatars by manipulating the meshes that make up the 3D model \cite{youtube_invisibility_toolbox, youtube_invisibility_PxINKY}. Through these affordances, users can communicate their uniqueness, explore life as their avatar, and hold greater control over how others perceive them.  

Avatar representation of disability is particularly understudied, with some recent exceptions. Zhang et al. \cite{zhang_partofme} found users disclosed disabilities by attaching assistive technology to their avatars (e.g., hearing aids) and adopted a spectrum of disclosure strategies to represent themselves in social VR. Additionally, Davis and Chansiri found that online users with disabilities customized their avatars to foster a greater sense of empowerment and embodiment \cite{davis_digital_identities}. For instance, one user depicted herself as younger because she felt that her disability removed years from her life. Mack et al. \cite{mack_towards} shed light on some challenges facing individuals with intersectional identities as they represented themselves in digital platforms, noting they often had to choose between using avatars to represent their disability or race-related identities.

Our study includes social VR users with all types of invisible disabilities, distinct from Zhang et al.’s study \cite{zhang_partofme} focused on people with visible disabilities who use assistive technology. Given that many participants with visible disabilities were interested in translating their non-virtual assistive technology into their virtual avatars, little is known about the preferences of invisibly disabled people for embodied representations. Our study investigates invisible disabilities that often do not require assistive technology, which shifts the focus to exploring social VR affordances that are not necessarily available in non-virtual spaces. In addition, we build on Mack et al.’s study \cite{mack_towards} of digital avatars. Though their work included participants with invisible disabilities and found they wanted to use symbolic representations of disability that would resonate with their more specific community (e.g., chronic illness, ADHD), we extend our inquiry to study invisible disability representation preferences into virtual, embodied contexts. In this study, we examine how users want to employ VR’s multimodal affordances for disability expression in spaces where avatars mediate all social interaction. 

\section{Methodology}
We conducted semi-structured interviews with \DIFdelbegin \DIFdel{12 participants who +}\DIFdelend \DIFaddbegin \DIFadd{15 participants who }\DIFaddend self-identified as having one or more invisible disabilities. We hoped to understand their perspectives on disability representation and visual disclosure in both non-virtual and social VR settings.

\subsection{Recruitment}
We recruited participants by emailing disability-related organization mailing lists, posting messages in relevant \DIFdelbegin \DIFdel{groups on Reddit}\DIFdelend \DIFaddbegin \DIFadd{subreddits}\DIFaddend , and partnering with \DIFdelbegin \DIFdel{an academic department}\DIFdelend \DIFaddbegin \DIFadd{our university}\DIFaddend ’s undergraduate extra credit system\DIFdelbegin \DIFdel{at a North American university}\DIFdelend . Our inclusion criteria were as follows: \DIFdelbegin \DIFdel{Participants must }\DIFdelend \DIFaddbegin \DIFadd{participants must (}\DIFaddend 1) \DIFdelbegin \DIFdel{Be }\DIFdelend \DIFaddbegin \DIFadd{be }\DIFaddend at least 18 years old, \DIFaddbegin \DIFadd{(}\DIFaddend 2) \DIFdelbegin \DIFdel{Have }\DIFdelend \DIFaddbegin \DIFadd{have }\DIFaddend an invisible disability, and \DIFaddbegin \DIFadd{(}\DIFaddend 3) \DIFdelbegin \DIFdel{Have }\DIFdelend \DIFaddbegin \DIFadd{have }\DIFaddend experience using social VR platforms. 

Our recruitment materials stated: “We define having invisible disabilities as including physical and psychological conditions that often have no visible manifestation, such as attention deficit, autism, and chronic health issues. We define social VR as a virtual platform where people communicate and interact with others in the form of avatars. Some popular social VR platforms include Rec Room, VRChat, vTime XR, and AltspaceVR.” \DIFdelbegin \DIFdel{Note that we }\DIFdelend \DIFaddbegin \DIFadd{We }\DIFaddend released these recruitment materials before AltspaceVR was shut down. 

\subsection{Participants}
This study consisted of \DIFdelbegin \DIFdel{12 }\DIFdelend \DIFaddbegin \DIFadd{14 }\DIFaddend participants aged 20 to 56 years old (\DIFdelbegin \DIFdel{$mean = 33.75, SD = 10.52$}\DIFdelend \DIFaddbegin \DIFadd{$mean = 33.14, SD = 10.13$}\DIFaddend ). Seven identified as female and \DIFdelbegin \DIFdel{five }\DIFdelend \DIFaddbegin \DIFadd{seven }\DIFaddend identified as male. Regarding race, \DIFdelbegin \DIFdel{six }\DIFdelend \DIFaddbegin \DIFadd{seven }\DIFaddend participants identified as White, \DIFdelbegin \DIFdel{two as Black }\DIFdelend \DIFaddbegin \DIFadd{three as Black or African American}\DIFaddend , two as mixed-race, one as Asian, and one as Alaskan Native. \DIFdelbegin \DIFdel{Eleven participants disclosed their disabilities, identifying disabilities }\DIFdelend \DIFaddbegin \DIFadd{All participants disclosed that they had at least one invisible disability, }\DIFaddend such as dyslexia, chronic pain, ADHD, and \DIFdelbegin \DIFdel{depression. }\DIFdelend \DIFaddbegin \DIFadd{autism. Two participants did not disclose their specific disabilities but shared the general type of disability (e.g., chronic condition, learning disability). }\DIFaddend In total, \DIFdelbegin \DIFdel{19 }\DIFdelend \DIFaddbegin \DIFadd{22 }\DIFaddend unique invisible disabilities were represented in this sample. All participants had experience with at least one social VR platform, but many had used multiple (e.g., VRChat, AltspaceVR, Spatial, Rec Room). Most used VR on a daily or weekly basis. \DIFdelbegin \DIFdel{See Table 1 for a more }\DIFdelend \DIFaddbegin \DIFadd{We present a }\DIFaddend detailed demographic breakdown \DIFaddbegin \DIFadd{in Table \ref{table:participants}}\DIFaddend . Participants were compensated with a \$20 \DIFdelbegin \DIFdel{Amazon gift card and recognition of participation after the interview’s conclusion}\DIFdelend \DIFaddbegin \DIFadd{digital gift card upon completion of the interview}\DIFaddend . This study and all procedures were approved by our university\DIFdelbegin \DIFdel{'}\DIFdelend \DIFaddbegin \DIFadd{’}\DIFaddend s Institutional Review Board (IRB), and all participants completed informed consent.

\subsection{Procedure}
We conducted semi-structured interviews via video conferencing software (Zoom)\DIFdelbegin \DIFdel{, with a creative component done through }\DIFdelend \DIFaddbegin \DIFadd{. As part of the interview, we engaged participants in a creative activity on }\DIFaddend a collaborative whiteboard application (Google Jamboard), which allowed participants to draw and paint in multiple colors, import or link images from a device or online, type thoughts and ideas on sticky notes, and create text boxes and shapes. Participants could also use a virtual laser pointer to emphasize different aspects of the whiteboard while describing features of their creative expression if they so chose. All interviews were conducted in English, lasted approximately 60 minutes, and were video and audio recorded with the participants\DIFdelbegin \DIFdel{' }\DIFdelend \DIFaddbegin \DIFadd{’ }\DIFaddend consent. We provide our full interview protocol in Supplementary Materials.

Each interview began with an introduction to the research and a review of the consent form prior to obtaining oral consent. We began the interview portion by asking participants about their uses for social VR and existing avatar representations in social VR, followed by questions that probed their current use of avatars as vessels for disclosure (or not). For example, we asked: “Do you represent or conceal your invisible disability in social VR in any way? How similar is your avatar representation to your physical self?” After establishing the similarities and differences between participants’ virtual and non-virtual selves, we asked if participants were interested in representing their invisible disability / disabilities in social VR. Regardless of their responses, we followed up by discussing how context might impact their decisions to represent (or not represent) their invisible disabilities. We wrapped up the first section by broadly exploring participants’ granular customization preferences.

The second section encouraged idea generation through creative brainstorming. We invited participants to share ideas for their “ideal avatar representation” in social VR by using the virtual whiteboard to express their ideas through images, drawing, or text.  After completing their visualizations and describing the thought processes behind them, participants were asked to describe any important features that were not currently available as well as their ideal customization process.

In the third section, we further explored the importance of context in virtual and non-virtual disclosure. We asked questions such as, “In the physical world, how do you navigate disability disclosure? Would you consider your avatar representation to be the same or different in different settings? How does this compare to other platforms with avatar options, such as Snapchat?” Finally, we discussed the practical implications of incorporating invisible disability representation features into avatar libraries. 

\subsection{Analysis}
Our data consisted of approximately 15 hours of recordings and detailed notes collected during the interviews. We transcribed all recordings and then used open coding to analyze the interviews. Three researchers divided the first three transcripts so that each was double-coded, discussed code discrepancies, created the preliminary codebook, and then split up the remaining transcripts for individual coding. Throughout the coding process, we iterated and refined the codebook over the course of approximately five meetings. 

After coding, we conducted thematic analysis \cite{braun2012thematic} to identify overarching thematic takeaways and patterns across participants. Our themes were grounded in the interview codes as well as the suggestions presented by participants during the whiteboard component, which included image and drawing artifacts. Per Clarke and Braun’s thematic analysis guide \cite{clarke2013thematic}, three team members generated lists of potential themes and bulleted outlines of the connections between them as preparation for a thematic analysis meeting. Then, we reflected on the proposed themes’ connections to our research questions, compared areas of overlap and divergence, and reflexively confronted any potential analytical assumptions. Finally, the three coders selected the themes that overlapped between their lists, and consulted with other team members to ensure themes engaged substantively with interpretative contributions, tweaking the thematic headings until they arrived at their final version. 

\subsection{Positionality}
\DIFdelbegin \DIFdel{The first author }\DIFdelend \DIFaddbegin \DIFadd{One of the first authors }\DIFaddend lives with an invisible disability and has a background in feminist disability studies. The research team also includes social VR users, accessibility researchers, and people who have grappled with the complex issue of disability disclosure in their own lives. We believe avatar customization reform is an important step toward maximizing the inclusiveness of social VR spaces and aim to include the voices of VR users with invisible disabilities into the important conversations surrounding fostering positive representation and cultivating diverse spaces. 


\begin{table*}[h!]
    \footnotesize 
    \centering
    \caption{Participants\DIFdelbeginFL \DIFdelFL{' }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{’ }\DIFaddendFL demographics.} 
    \begin{tabular}{p{0.3cm}p{0.9cm}p{1.5cm}p{2.8cm}p{3.8cm}p{2.8cm}}
    \toprule
      \textbf{ID}&  \textbf{Age/ Gender}&  \textbf{Race}&  \textbf{Disabilities}&  \textbf{Social VR Use}&   \textbf{Frequency} \\
     \midrule 

   \textbf{P1}&   32/F&   White&  Low vision&  Altspace VR; Spatial&  several times/week \\ 
    \midrule

    \textbf{P2}&   32/F&   White& Bipolar disorder; PTSD&  synth Riders; VR fishing; VRChat; Walk about Mini Golf; & daily\\ 
    \midrule

     \textbf{P3} & 56/F & Mixed-race&  Dyslexia; rheumatoid arthritis; congestive heart failure& Altspace VR; VR fishing; VR Chat; Spatial; Big Screen; Wander& weekly\\ 
    \midrule

      \textbf{P4}&    38/F&    White &  Dyslexia; epilepsy; chronic pain&  the limps, Les Mills, body cam, FedEx, Sabre, the mini golf&   two to four or five times a week\\ 
    \midrule

      \textbf{P5}&    31/M&    White&   RSI; ADHD; Asperger\DIFdelbeginFL \DIFdelFL{'}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{’}\DIFaddendFL s& two to four or five times a week&  social: monthly
VR in general: weekly\\ 
    \midrule

    \textbf{P6}&    24/F&    Black &   POTS& vTime XR; Altspace VR; miscellaneous; Rec Room; Ping-pong& weekly\\ 
    \midrule

      \textbf{P7}&    33/F&    White&   Depression& VR Chat&  daily\\ 
    \midrule

      \textbf{P8}&    20/M&   Asian&   Chronic condition (diagnosis undisclosed)& VR Chat& one to two times a month\\ 
    \midrule

      \textbf{P9}&    28/M&   White, Asian&   Autism (nonverbal); learning impairment with linguistics (text); bipolar type one&  VR Chat&  "extensive"; 5000-6000 hours\\ 
    \midrule

      \textbf{P10}&    52/F&  White&  Hashimoto\DIFdelbeginFL \DIFdelFL{'}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{’}\DIFaddendFL s disease; contextual social anxiety; osteoporosis&  VR Chat, Synth Riders& "live on there" - work, sleep, "addiction"\\ 
    \midrule

      \textbf{P11}&    28/M&  Black& ADHD (undiagnosed)&  Altspace VR; Spatial; Rec Room; Horizon Worlds& multiple times a month\\ 
      \midrule

      \textbf{P12}&    31/M&  White&  Asperger\DIFdelbeginFL \DIFdelFL{'}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{’}\DIFaddendFL s; ADHD& Altspace VR; Oculus; Rec Room; Facebook Horizon& game and therapeutic tool since 2019 \\ 

     \bottomrule
    \end{tabular}
    \DIFdelbeginFL %DIFDELCMD < \label{tab:my_label}
%DIFDELCMD < %%%
\DIFdelendFL \DIFaddbeginFL \label{table:participants}
\DIFaddendFL \end{table*}

\section{Findings}
\DIFdelbegin \DIFdel{We discovered themes surrounding social VR’s reflection of (and divergence from) non-virtual social environments (4.1), VR avatars’ potential for multimodal self-expression (4.2), and distinctions between public and private disability representations (4.3), as described below. We have also compiled suggestions participants had for increasing the accessibility of customization mechanisms (4.4) and summarized them alongside suggestions derived from the three themes (see Discussion). 
}\subsection{\DIFdel{Convergence and Divergence Between Social VR and Non-Virtual Social Contexts}}
%DIFAUXCMD
\addtocounter{subsection}{-1}%DIFAUXCMD
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdelend Social virtual reality spaces often reflect many of the norms and utilities of non-virtual social spaces. \DIFdelbegin \DIFdel{Participant responses provided us with an understanding of }\DIFdelend \DIFaddbegin \DIFadd{Participants shared more about }\DIFaddend their social VR uses \DIFdelbegin \DIFdel{as foundations for why diverse avatar representation matters. }\DIFdelend \DIFaddbegin \DIFadd{and experiences, and how they were similar or even equivalent to their non-virtual social interactions. 
}

\DIFadd{Participants used social VR for a variety of purposes, including entertainment (e.g., playing games), conversational (e.g., chatting with others), and professional (e.g., for work). For example, }\DIFaddend P1 described attending support groups, celebrating birthdays, \DIFdelbegin \DIFdel{watching movies and fishing }\DIFdelend \DIFaddbegin \DIFadd{and watching movies }\DIFaddend in social VR\DIFdelbegin \DIFdel{. }\DIFdelend \DIFaddbegin \DIFadd{, and }\DIFaddend P2 \DIFdelbegin \DIFdel{indicated she feels her virtual and non-virtual social interactions are equivalent, elaborating: 
}%DIFDELCMD < \begin{quote}
%DIFDELCMD <  %%%
\textit{\DIFdel{``To engage with others while they’re doing something active in the same way you are is very similar to if I was gonna go fishing with somebody in real life. It’s the same, like being able to join a chat party with some of my friends and go fishing with them together in VR.”}} %DIFAUXCMD
\DIFdel{(P2, f, 32 years old) 
}%DIFDELCMD < \end{quote}
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{VR affords such a breadth of social experiences that it can facilitate much of users’ daily social interactions. P7 shared, }\textit{\DIFdel{``VR is an interesting experience. Kinda really the majority of the socialization I do these days.”}} %DIFAUXCMD
\DIFdel{This transferral of social outlets from the non-virtual to the virtual world can occur for any number of reasons, but for }\DIFdelend \DIFaddbegin \DIFadd{felt that }\textit{\DIFadd{“}[\DIFadd{engaging}] \DIFadd{with others while they’re doing something active in the same way you are is very similar to if I was gonna go fishing with somebody in real life. It’s the same, like being able to join a chat party with some of my friends and go fishing with them together in VR.”}} \DIFadd{Additionally, for }\DIFaddend some participants, virtual platforms \DIFdelbegin \DIFdel{provide }\DIFdelend \DIFaddbegin \DIFadd{provided them }\DIFaddend essential access to environments when their invisible disabilities \DIFdelbegin \DIFdel{prevent }\DIFdelend \DIFaddbegin \DIFadd{prevented }\DIFaddend them from leaving home. 
\DIFdelbegin \DIFdel{P7 shared: 
}%DIFDELCMD < \begin{quote}
%DIFDELCMD < %%%
\textit{\DIFdel{``What I'm getting out of VR is a little different than what most people get out of VR. They get in there, and they want to }%DIFDELCMD < [%%%
\DIFdel{play games}%DIFDELCMD < ]%%%
\DIFdel{. I'm there so that the world doesn't close in on me. I'm there to keep a tiny little porthole of the world open to me. Even though I cannot physically be in it, I can virtually be in it. You know, I can visit a museum through VR. I went up on the space station through VR. I've gone scuba diving in VR. And the social aspects. I've met friends who have been my friends for years, but we live in different states. And we've come together.”}} %DIFAUXCMD
\DIFdel{(P7, f, 33 years old) 
}%DIFDELCMD < \end{quote}
%DIFDELCMD < %%%
\DIFdelend 

\DIFdelbegin \DIFdel{While many users opt to engage in social games, not all social VR contexts are casual. For P6, who maintains an avatar for work purposes, there are distinctions between how she approaches avatar customization in different environments. 
}\DIFdelend \begin{quote}
\DIFdelbegin \textit{\DIFdel{``I care a lot more about what my avatar looks like if I am engaging professionally for sure, because if I’m playing ping pong with my dad, I'll just use the default avatar or show up as a cat…But yeah, professionally, I manage it similarly to how I would dress if I were going to this event in-person professionally versus if I'm just hanging out with my dad.”}} %DIFAUXCMD
\DIFdel{(P6, f, 24 years old) 
}%DIFDELCMD < \end{quote}
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{Just as social VR can host a number of social and professional engagements like those found in the non-virtual world, it is also home to diverse spaces that can offer experiences ranging from relatively safe communities to potentially harmful environments. P1 points out:  
}%DIFDELCMD < \begin{quote}
%DIFDELCMD < %%%
\textit{\DIFdel{``Personally, I’m totally fine with having }%DIFDELCMD < [%%%
\DIFdel{disability representations}%DIFDELCMD < ] %%%
\DIFdel{on all the time. But I really understand why somebody wouldn’t want to have that option to turn it off, especially if you're going into more of a rough and rowdy crowd, like in VR Chat. You don't want to make yourself a target for people that might look for things to hurt you with. A lot of the communities that I hang out in on all social VR platforms, typically, I know that the people that are hanging out there are going to be more kind, empathetic people. But if you're going to a place that you don't really know very well, I think it would be a good idea to be able to turn that off or on.”}} %DIFAUXCMD
\DIFdel{(P1, f, 32 years old) 
}%DIFDELCMD < \end{quote}
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{Despite some marked similarities between the virtual and non-virtual domains, several participants perceived social VR to be a relatively safe space where they could freely express their disability-related identities without worrying as much about the stigma they face in the non-virtual world }\DIFdelend \DIFaddbegin \DIFadd{“What I’m getting out of VR is a little different than what most people get out of VR. They get in there, and they want to }[\DIFadd{play games}]\DIFadd{. I’m there so that the world doesn’t close in on me… to keep a tiny little porthole of the world open to me. Even though I cannot physically be in it, I can virtually be in it. I can visit a museum through VR}\DIFaddend . \DIFdelbegin \DIFdel{P9 felt more open to disclosing his disabilities in social VR because, unlike in the non-virtual world, he felt a disability label would not persist beyond the current VRexperience. P9 explained: }\textit{\DIFdel{``I feel like once I label myself }%DIFDELCMD < [%%%
\DIFdel{with a disability}%DIFDELCMD < ] %%%
\DIFdel{in real life, it becomes something that kind of follows you around.’’}}
%DIFAUXCMD
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{P12 expanded on how situational disclosure might be impacted by the VR context: 
}%DIFDELCMD < \begin{quote}
%DIFDELCMD <     %%%
\textit{\DIFdel{``I don't mind disclosing, but it's on a situational basis, especially based on the virtual environment in the case of VR versus a real-life environment. I mean, I'll even give you a small example. There are times when I maybe wouldn't necessarily disclose my disability in real life if, say, I'm stressed, but I would just tell the person I'm interacting with if I personally notice myself interacting that way. That's something else with my disability, I noticed. Sometimes, I will be self-aware of how I'm feeling and how I'm interacting, but other times, it will just be impulsive, and it will feel like a blur.’’}} %DIFAUXCMD
\DIFdel{(P12, m, 31 years old)
}%DIFDELCMD < \end{quote}
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{P3 unpacked more of the nuances behind transforming non-virtual representations into embodied VRenvironments, indicating the factors that contribute to her decision about the extent she wants to represent herself in VR: 
}%DIFDELCMD < \begin{quote}
%DIFDELCMD < %%%
\textit{\DIFdel{``My VR Avatar is whatever I'm feeling at the moment. If I'm feeling immersed in my invisible illness, then I'm probably gonna want my avatar to be also. And if I'm feeling like, ‘okay, I'm escaping reality,’ I don't want my avatar to be even close to what I am. }%DIFDELCMD < [%%%
\DIFdel{In support group,}%DIFDELCMD < ] %%%
\DIFdel{there will still be some days that I don't want to manifest that. And then other days where it's like, ‘yeah, I'm feeling like crap and I'll let you people know it in a non-verbal way,’ and I will come in there all crippled up with my avatar, altered to represent how I feel right now simply because I am trying to communicate it in a nonverbal way.”}} %DIFAUXCMD
\DIFdel{(P3, f, 56 years old}\DIFdelend \DIFaddbegin \DIFadd{I went up }[\DIFadd{to}] \DIFadd{the space station through VR. I’ve gone scuba diving in VR. And the social aspects \textemdash{} I’ve met friends who have been my friends for years, but we live in different states. And we’ve come together.” (P7, 33F}\DIFaddend ) 
\end{quote}

\DIFdelbegin \DIFdel{Beyond the support group setting, she noted the importance of having the option to accurately reflect her non-virtual self, in a way normalizing the uncanny valley effect of embodied avatars that are: 
}%DIFDELCMD < \begin{quote}
%DIFDELCMD < %%%
\textit{\DIFdel{``A way I might have looked once upon a time. They keep me from aging…I’m not the type of person who changes }%DIFDELCMD < [%%%
\DIFdel{my avatar}%DIFDELCMD < ] %%%
\DIFdel{all the time, and it puts me in a little suspended animation where I haven’t aged in six years.”}} %DIFAUXCMD
\DIFdel{(P3, f, 56 years old)
}%DIFDELCMD < \end{quote}
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{She elaborated on customizable avatars}\DIFdelend \DIFaddbegin \DIFadd{In this section, we present participants}\DIFaddend ’ \DIFdelbegin \DIFdel{psychological role in grounding her VR experiences: 
}%DIFDELCMD < \begin{quote}
%DIFDELCMD < %%%
\textit{\DIFdel{``}%DIFDELCMD < [%%%
\DIFdel{Having options}%DIFDELCMD < ] %%%
\DIFdel{gives you virtual reality with just a little bit of more normalcy. Just enough normalcy to make me go, ‘Okay, I'm not gonna run from this. It's not so foreign that it's freaking me out.’...It gives you a little bit of an anchor to not overwhelm you.}} %DIFAUXCMD
\DIFdel{(P3, f, 56 years old)
}%DIFDELCMD < \end{quote}
%DIFDELCMD <  

%DIFDELCMD < %%%
\subsection{\DIFdel{VR Avatars as Multimodal Reflections of Physical Human Expression}}
%DIFAUXCMD
\addtocounter{subsection}{-1}%DIFAUXCMD
\DIFdel{VR allows }\DIFdelend \DIFaddbegin \DIFadd{perceptions on the unique affordances of embodied VR avatars, detail current and imagined invisible disability representations for social VR avatars, and explore disclosure preferences across different social VR contexts.
}\subsection{\DIFadd{Embodied VR Avatars are Dynamic, Contextual, and Multimodal}}
\DIFadd{Participants identified key differences in their perceptions of non-embodied and embodied avatars. In general, they viewed non-embodied avatars, such as Facebook profile pictures, Facebook avatars, and Snapchat Bitmojis, as a single snapshot of their identity. On the other hand, participants found embodied VR avatars to be more dynamic and authentic representations of themselves. Additionally, one key affordance of VR avatars is that they allow }\DIFaddend for multimodal self-expression, \DIFdelbegin \DIFdel{an affordance that left a big impression when it came to describing }\DIFdelend \DIFaddbegin \DIFadd{which greatly influenced participants’ }\DIFaddend current and imagined preferences for disability representations on social VR platforms. 
\DIFdelbegin \DIFdel{Among other affordances, they offer avenues for self-expression through visuals, voice, movement, body language, and facial expression}\DIFdelend \DIFaddbegin 

\subsubsection{\DIFadd{Differences Between Embodied and Non-Embodied Avatars}}
\DIFadd{Though participants had experience using non-embodied avatars to represent themselves, they felt as though the static nature made it difficult for them to convey their true, current identity. For example, P1 said that her Facebook avatar }\textit{\DIFadd{“doesn’t look like me at all. I hate it.”}} \DIFadd{P3 also shared how her experiences with using Facebook and social VR for different purposes, and for different audiences, influenced her degree of comfort with representing herself in embodied and non-embodied contexts}\DIFaddend .

\DIFdelbegin \DIFdel{P9 emphasized embodied avatars}\DIFdelend \DIFaddbegin \begin{quote}
\DIFadd{“With Facebook, of course my avatar is a photo of me. But it}\DIFaddend ’\DIFdelbegin \DIFdel{connections to his mood, especially when expressing his experience of Bipolar Type 1. He uses VRavatar appearances, and especially their colors, to communicate his emotions nonverbally, strategically selecting avatars based on his goals for social interactions that day. 
When sharing screenshots of his current avatars, he explained his use of visual affordances and their social and psychological effects: 
}\DIFdelend \DIFaddbegin \DIFadd{s a photo of me 20 years ago. So my avatar doesn’t age there… and I have not changed it to be what I am now. Because the people that are on my Facebook, many of them are people that know me in this physical reality. They know what I look like. I don’t have to make it a picture from yesterday. But it’s also something that I’m not gonna change, you know. I cannot pretend in Facebook that I’m well or not well… I don’t represent a cause, I don’t represent a disease, I don’t represent anything by myself. … Whereas in VR, I do change those things. It doesn’t mean that I’m two-faced, or anything like that. … Virtual reality, there are people there that know and love me, but most people are acquaintances or strangers. So my interaction with them is going to be different }[\DIFadd{from}] \DIFadd{my interaction on Facebook.” (P3, 56F)
}\end{quote}

\DIFadd{Others also expressed that the embodied nature of social VR avatars encouraged them to be more authentic. P14 mentioned that the }\textit{\DIFadd{“immersive experience }[\DIFadd{of being}] \DIFadd{around a lot of people, seeing the avatar move around”}} \DIFadd{made him wish to represent himself in greater detail on a social VR avatar as opposed to a static avatar on Facebook. 
}

\DIFadd{Referring to the overall experience of using mainstream social media networks, P13 also mentioned that he actively chose to not engage with these platforms to avoid }\textit{\DIFadd{“engagement loops that keep you coming back to it… they’ll track you with their pixel tracker on other websites and start sending you advertisements.”}} \DIFadd{In contrast to text-only communication on social media, he found the different communication modes in social VR to be easier to process: }\textit{\DIFadd{“you can take in text easier… it’s basically reading text messages versus voice chat, digital avatar, }[\DIFadd{or}] \DIFadd{motion capture”}} \DIFadd{(P13). Additionally, he mentioned that the discomfort and fatigue associated with VR headsets was helpful for preventing him from spending excessively long on these platforms. 
}

\DIFadd{When discussing the distinctions between social media and social VR, P9 summarized how his interactions differed between the two environments and emphasized that the immersive affordances of social VR avatars enabled him to not only better express himself, but understand others as well.
}

\DIFaddend \begin{quote}
\textit{\DIFdelbegin \DIFdel{``The middle avatar is the avatar }\DIFdelend \DIFaddbegin \DIFadd{“}\DIFaddend I\DIFdelbegin \DIFdel{use when I}\DIFdelend ’\DIFdelbegin \DIFdel{m in a playful mood. It stands out, but it's also really friendly looking. I got a lot }\DIFdelend \DIFaddbegin \DIFadd{d say }[\DIFadd{VR}] \DIFadd{is an order }\DIFaddend of \DIFdelbegin \DIFdel{people }\DIFdelend \DIFaddbegin \DIFadd{magnitude above anything }\DIFaddend that \DIFdelbegin \DIFdel{like to hang around with me in this one if I'm feeling energetic, a little bit extroverted}\DIFdelend \DIFaddbegin \DIFadd{you would see on Instagram \textemdash{} anything that you see on any other website \textemdash{} because those are just two-dimensional static images or videos}\DIFaddend . \DIFdelbegin \DIFdel{If we talk about bipolar phases a little bit more, like the maniac phase, I'll use the middle one. … Yeah, I like to rotate between these 5. I kind of think of it as ‘How }\DIFdelend \DIFaddbegin [\DIFadd{You}] \DIFaddend can\DIFdelbegin \DIFdel{I best express myself and kinda let others know how I}\DIFdelend ’\DIFdelbegin \DIFdel{m feeling based on the avatar?}\DIFdelend \DIFaddbegin \DIFadd{t interact with photos, but when you}\DIFaddend ’\DIFdelbegin \DIFdel{If I’m }\DIFdelend \DIFaddbegin \DIFadd{re there }\DIFaddend in \DIFdelbegin \DIFdel{a really happy mood}\DIFdelend \DIFaddbegin \DIFadd{virtual reality}\DIFaddend , \DIFdelbegin \DIFdel{but I pick an avatar with like no color, for few emotions, it wouldn't really match. Same thing vice versa. It also adds some novelty to VR chat as well, because if I }\DIFdelend \DIFaddbegin \DIFadd{you can }\DIFaddend see \DIFdelbegin \DIFdel{myself in }\DIFdelend \DIFaddbegin \DIFadd{all }\DIFaddend the \DIFdelbegin \DIFdel{same avatar for too long, I feel like I start to get fixed. I start to lock myself in }\DIFdelend \DIFaddbegin \DIFadd{details on }\DIFaddend the avatar \DIFaddbegin \DIFadd{showing that this person is expressing themselves}\DIFaddend . \DIFdelbegin \DIFdel{So}\DIFdelend \DIFaddbegin [\DIFadd{You can}] \DIFadd{see their facial expressions}\DIFaddend , \DIFdelbegin \DIFdel{I like to mix it around}\DIFdelend \DIFaddbegin \DIFadd{their movements}\DIFaddend , \DIFdelbegin \DIFdel{so I know there'}\DIFdelend \DIFaddbegin \DIFadd{and their body language. And it’}\DIFaddend s \DIFdelbegin \DIFdel{always flexibility }\DIFdelend \DIFaddbegin \DIFadd{real time. No other kind of social platform comes even close }\DIFaddend to \DIFdelbegin \DIFdel{iterate and change}\DIFdelend \DIFaddbegin \DIFadd{VR}\DIFaddend .”} (P9, \DIFdelbegin \DIFdel{m, 28 years old}\DIFdelend \DIFaddbegin \DIFadd{28M}\DIFaddend ) 
\end{quote}

\DIFdelbegin \DIFdel{P9 and other participants also }\DIFdelend \DIFaddbegin \subsubsection{\DIFadd{Multimodal Affordances Can Represent Physical Human Expression}}
\DIFadd{Participants also discussed the multimodal expressiveness of embodied avatars, which manifested primarily through avatar visuals, voices, movements, body language, and facial expressions. For example, participants }\DIFaddend described more of the physicality of communicating in social VR spaces. P9 \DIFdelbegin \DIFdel{spoke to }\DIFdelend \DIFaddbegin \DIFadd{discussed }\DIFaddend the value of facial expressions: 
\DIFaddbegin 

\DIFaddend \begin{quote}
\DIFdelbegin \textit{\DIFdel{``I am quite expressive myself, but my invisible disability is nonverbal autism, so I wouldn't actually say what I’m feeling. I would express it through my avatar’s facial expressions. Sometimes, the number of expressions on an avatar goes as high as 30 or 40 different options. So having many different options to express myself nonverbally is a way that I can get more synchronized and comfortable using an avatar.”}} %DIFAUXCMD
\DIFdelend \DIFaddbegin \DIFadd{“I am quite expressive myself, but my invisible disability is nonverbal autism, so I wouldn’t actually say what I’m feeling. I would express it through my avatar’s facial expressions. Sometimes, the number of expressions on an avatar goes as high as 30 or 40 different options. So having many different options to express myself nonverbally is a way that I can get more synchronized and comfortable using an avatar.” }\DIFaddend (\DIFdelbegin \DIFdel{P9, m}\DIFdelend \DIFaddbegin \DIFadd{P9}\DIFaddend , \DIFdelbegin \DIFdel{28 years old}\DIFdelend \DIFaddbegin \DIFadd{28M}\DIFaddend ) 
\end{quote}

\DIFaddbegin \DIFadd{While }\DIFaddend P2 \DIFdelbegin \DIFdel{hadn’t personally }\DIFdelend \DIFaddbegin \DIFadd{had not }\DIFaddend used the facial \DIFdelbegin \DIFdel{expressions feature }\DIFdelend \DIFaddbegin \DIFadd{expression features }\DIFaddend of newer VR headsets\DIFdelbegin \DIFdel{but was familiar with it through friends who have shared their experiences: }\textit{\DIFdel{``Avatars already blink. They talk, they cry…When you smile, it makes the avatar smile, or when you furrow your brows it matches your facial expressions more.”}} %DIFAUXCMD
\DIFdel{Though P2 expressed amazement at the current state of technology, she also shared some ideas for future development, including dynamic representations of energy: }\textit{\DIFdel{``An energy bar, like in a video game where you have your life meter. If it’s full, you're full of energy, and it's all the way green…And if I'm really low on energy, I've got a red bar.”}} 
%DIFAUXCMD
\DIFdelend \DIFaddbegin \DIFadd{, as someone with bipolar disorder, she was interested in using body language to represent changes in her mood. 
}

\DIFaddend \begin{quote} 
\DIFdelbegin \textit{\DIFdel{``Let's say I'm feeling excited or hyper. Your avatar can have a really upbeat energy to it if you're going to apply an energy to an avatar. Or if you can put in there that you're feeling slightly depressed, or that you have a low mood or that you're tired, your avatar would be a little bit lower on the energy…That way my friends could see me and then go like, ‘Oh, that's kind of the mood she's in. Let's cheer her up.’ Or, ‘Let's just give her her space.’ And they see you come in in this perky mood, and then they can kind of match their energy to your mood without you having to be so vocal about it.”}} %DIFAUXCMD
\DIFdelend \DIFaddbegin \DIFadd{“Let’s say I’m feeling excited or hyper. Your avatar can have a really upbeat energy to it if you’re going to apply an energy to an avatar. Or if you can put in there that you’re feeling slightly depressed, or that you have a low mood or that you’re tired, your avatar would be a little bit lower on the energy… That way my friends could see me and then go like, ‘Oh, that’s kind of the mood she’s in. Let’s cheer her up.’ Or, ‘Let’s just give her her space.’ And they see you come in in this perky mood, and then they can kind of match their energy to your mood without you having to be so vocal about it.” }\DIFaddend (P2, \DIFdelbegin \DIFdel{f, 32 years old}\DIFdelend \DIFaddbegin \DIFadd{32F}\DIFaddend ) 
\end{quote}

\DIFdelbegin \DIFdel{Like P2’s energy-related suggestion, some participants focused their representation ideas around the movement aspect of embodied avatars . }\DIFdelend \DIFaddbegin \DIFadd{Some participants focused on how the embodied movement of VR avatars could represent or support their disability identities. For example, P12 wanted to utilize either voice or movement: }\textit{\DIFadd{“if I am going to disclose my disability on the platform, it would be verbally or through using the VR controllers when I’m controlling the hands of the avatar.”}} \DIFadd{Conversely, though his experiences with arthritis sometimes impacted his mobility in the non-virtual world, P14 did not want to disclose his disability through this modality \textemdash{} he preferred for his avatar to move in the same ways as others. Regarding support of the disabled experience, P3 described how embodied VR avatar interactions could facilitate community empowerment and connection in a disability support group: }\textit{\DIFadd{“sometimes, our avatars will run over and give somebody a group avatar hug when they’re having a particularly bad time.”}} \DIFaddend P4 shared an anecdote about the inconvenience of embodying a cat and having your avatar’s eye line to the ground when engaging with human-sized avatars. 
\DIFdelbegin \DIFdel{P12 wanted to utilize two aspects of VR’s multimodality to use voice and movement for disability expression. }\textit{\DIFdel{``If I am going to disclose my disability on the platform, it would be more verbally or through using the VR controllers when I'm controlling the hands of the avatar.”}} %DIFAUXCMD
\DIFdel{P3 described the use of VR avatar movement to facilitate community support with a physicality unique to embodied contexts. }\textit{\DIFdel{``Sometimes, our avatars will run over and give somebody a group avatar hug when they're having a particularly bad time, and I'll run over and do that.”}} %DIFAUXCMD
\DIFdel{(P3, f, 56 years old) 
}\DIFdelend 

\DIFdelbegin \DIFdel{P9 summarized VR’s multimodal affordances well while identifying perceived distinctions from the digital domain: 
}%DIFDELCMD < \begin{quote}
%DIFDELCMD < %%%
\textit{\DIFdel{``I'd say }%DIFDELCMD < [%%%
\DIFdel{VR}%DIFDELCMD < ] %%%
\DIFdel{is an order of magnitude above anything that you would see on Instagram – anything that you see on any other website – because those are just two-dimensional static images or videos. Can't interact with photos, but when you're there in virtual reality, you can see all the details on the avatar show this person is expressing themselves. See their facial expressions, their movements and their body language. And it's real time. No other kind of social platform comes even close to VR.”}} %DIFAUXCMD
\DIFdel{(P9, m, 28 years old) 
}%DIFDELCMD < \end{quote}
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{Speaking to the affordances of other }\DIFdelend \DIFaddbegin \DIFadd{Other }\DIFaddend extended reality technologies\DIFdelbegin \DIFdel{(i.e., augmented reality, mixed reality), }\DIFdelend \DIFaddbegin \DIFadd{, such as augmented or mixed reality, were also of interest. }\DIFaddend P10 wanted to \DIFdelbegin \DIFdel{take her embodied avatar from social VR and star it in her social media content using mixed-reality, merging representations of the }\DIFdelend \DIFaddbegin \DIFadd{use her embodied social VR avatar in her content creation process to merge her representations in }\DIFaddend virtual and non-virtual domains\DIFdelbegin \DIFdel{. 
}\DIFdelend \DIFaddbegin \DIFadd{:
}\DIFaddend 

\begin{quote}
\DIFdelbegin \textit{\DIFdel{``Yeah, I just wish they had a lot more options for stuff. Well, I’m hoping they grow in that area }%DIFDELCMD < [%%%
\DIFdel{mixed-reality}%DIFDELCMD < ] %%%
\DIFdel{when they come out with the next }%DIFDELCMD < [%%%
\DIFdel{headset}%DIFDELCMD < ]%%%
\DIFdel{, because I heard through the grapevine it's supposed to be more for mixed-reality. I would actually love using an avatar instead of my real body in my YouTube videos.”}} %DIFAUXCMD
\DIFdelend \DIFaddbegin \DIFadd{“I just wish they had a lot more options for stuff. I’m hoping they grow in that area }[\DIFadd{mixed reality}] \DIFadd{when they come out with the next }[\DIFadd{headset}]\DIFadd{, because I heard through the grapevine it’s supposed to be more for mixed reality. I would actually love using an avatar instead of my real body in my YouTube videos.” }\DIFaddend (P10, \DIFdelbegin \DIFdel{f}\DIFdelend \DIFaddbegin \DIFadd{F}\DIFaddend , 52 years old) 
\end{quote}

\subsection{\DIFdelbegin \DIFdel{Public }\DIFdelend \DIFaddbegin \DIFadd{Current }\DIFaddend and \DIFdelbegin \DIFdel{Private Representations of }\DIFdelend \DIFaddbegin \DIFadd{Imagined Invisible }\DIFaddend Disability \DIFaddbegin \DIFadd{Representations}\DIFaddend }
\DIFaddbegin \DIFadd{Throughout the interviews, participants shared the ways they currently represented or disclosed their invisible disability and brainstormed ways to improve avatar systems to make them more inclusive. Generally, social VR offers users unique affordances that shape avatar customization and self-expression. P11 described his avatar to be }\textit{\DIFadd{“an exaggeration of }[\DIFadd{his}] \DIFadd{physical identity \textemdash{} anonymous, but also close enough to be recognized if you know }[\DIFadd{him}] \DIFadd{personally.”}} \DIFadd{P12 had a similar description: }\textit{\DIFadd{“I try to represent myself as I am, of course, and for me, that involves maybe making an avatar that looks like me but is a little bit cooler if possible.”}}
\DIFaddend 

\DIFaddbegin \DIFadd{We found that desired methods of representing invisible disabilities in social VR did not always align with non-virtual disclosure practices. }\DIFaddend Participants desired options for both public (\DIFdelbegin \DIFdel{or }\DIFdelend \DIFaddbegin \DIFadd{i.e., }\DIFaddend explicit) and private (\DIFdelbegin \DIFdel{or }\DIFdelend \DIFaddbegin \DIFadd{i.e., }\DIFaddend implicit) identity expression. Suggestions \DIFdelbegin \DIFdel{included }\DIFdelend \DIFaddbegin \DIFadd{for both public and private representations encompassed }\DIFaddend clothing, accessories, icons, energy bars, or modifications to avatar bodies\DIFdelbegin \DIFdel{such as a tail, and some suggestion categories included both public and private meanings}\DIFdelend .

\DIFdelbegin \DIFdel{To start, }\DIFdelend \DIFaddbegin \subsubsection{\DIFadd{Public Representations and Expressions of Disability}}
\DIFadd{Some participants were interested in representing their disability identities in public and explicit ways, meaning that other social VR users could identify their specific disability or their symptoms from their avatar. 
}

\DIFadd{Ten }\DIFaddend participants suggested incorporating customizable clothing\DIFdelbegin \DIFdel{and patterns}\DIFdelend \DIFaddbegin \DIFadd{, patterns, or accessories }\DIFaddend that featured disability-related logos. \DIFaddbegin \DIFadd{These suggestions often supported participants’ goals of expressing their personal style and advocating or educating about their disability. }\DIFaddend For example, P1 wanted to have an avatar wearing a zebra-printed shirt and beret to advocate for Rare Disease Month. Similarly, \DIFdelbegin \DIFdel{P4 suggested }\DIFdelend \DIFaddbegin \DIFadd{P12 wished to express his personal style and disability status through a }\textit{\DIFadd{“little cool jacket }[\DIFadd{with}] \DIFadd{a label…to say my name and that I have Asperger’s and whatnot.”}} \DIFadd{Others suggested having accessories specific to their disability (e.g., a brooch saying “POTS” as suggested by P6, or a PTSD ribbon as suggested by P13). P4 wished to have }\DIFaddend an explicit representation for communicating the experience of dyslexia through apparel\DIFdelbegin \DIFdel{or logos}\DIFdelend : 

\begin{quote}
\DIFdelbegin \textit{\DIFdel{``}%DIFDELCMD < [%%%
\DIFdel{On clothing,}%DIFDELCMD < ] %%%
\DIFdel{have the word dyslexia, but then have it jumbled up so people can see what it looks like when we try to read. Then, they'll be like, `Whoa, that's not fun.’ And we're like, `Well, welcome to my hell.’ Make it a joke, but also kind of be like, `Hey, this is really what it feels like.’ }} %DIFAUXCMD
\DIFdelend \DIFaddbegin \DIFadd{“}[\DIFadd{On clothing,}] \DIFadd{have the word dyslexia, but then have it jumbled up so people can see what it looks like when we try to read. Then, they’ll be like, ‘Whoa, that’s not fun.’ And we’re like, ‘Well, welcome to my hell.’ Make it a joke, but also kind of be like, ‘Hey, this is really what it feels like.’” }\DIFaddend (\DIFdelbegin \DIFdel{P4,f, 38 years old)
}\DIFdelend \DIFaddbegin \DIFadd{P4, 38F)
}\DIFaddend \end{quote}

\DIFdelbegin \DIFdel{Just as P4’s suggestion combined personality and humor to inspire avatar-based education and disability advocacy efforts, P12 wished to express his personal style and disability status through a }\textit{\DIFdel{“little cool jacket }%DIFDELCMD < [%%%
\DIFdel{with}%DIFDELCMD < ] %%%
\DIFdel{a label…to say my name and that I have Asperger’s and whatnot.”}}
%DIFAUXCMD
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdelend Other participants wanted customization libraries to include assistive technology (e.g., wheelchairs, canes, crutches, hearing aids), \DIFdelbegin \DIFdel{an assortment of chronic-illness specific items (e.g., a brooch that says }\textit{\DIFdel{``POTS’’}}%DIFAUXCMD
\DIFdel{, P6), a }\DIFdelend \DIFaddbegin \DIFadd{a }\DIFaddend medical alert bracelet, and \textit{\DIFdelbegin \DIFdel{``}\DIFdelend \DIFaddbegin \DIFadd{“}\DIFaddend spoonie\DIFdelbegin \DIFdel{’’}\DIFdelend \DIFaddbegin \DIFadd{”}\DIFaddend } gear \DIFdelbegin \DIFdel{like }\DIFdelend \DIFaddbegin \DIFadd{(e.g., }\DIFaddend a giant spoon, \DIFaddbegin \DIFadd{as suggested by }\DIFaddend P1) to disclose their disabilities. 

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{imgs/P1.png}
    \caption{Participant 1’s drawings and suggestions for invisible disability representation during the whiteboard component of the study, featuring a giant spoon to represent spoon theory and other assistive technologies to disclose their disability.} 
    \Description{Participant 1’s drawings and suggestions for invisible disability representation during the whiteboard component of the study. At the far left, there is a floating medication reminder inside a speech bubble that represents a floating emote. Below are examples of assistive technology such as a cane and hearing aids. Next is a person’s outline wearing a zebra print beret and shirt to represent rare disease month. The shirt also has a space for a custom disability graphic or a fact about the participant’s rare disease, both aimed at spreading invisible disability awareness. The person also wears a medical alert bracelet and carries a human-sized spoon to represent desired “spoonie” props that point to identification with spoon theory. Finally, there is a note where there would be a floating menu to enable and disable disability-related accessories.}
    \label{P1}
\end{figure*}

\DIFaddbegin \DIFadd{Icons and graphics around an avatar could also help with representing someone’s disability in a more subtle, but still public, way. Four participants were interested in disability representations that floated above their avatars, such as an awareness flag or a dynamic energy bar that correlated with their energy level or “social battery”. For example, P2 proposed }\textit{\DIFadd{“an energy bar, like in a video game where you have your life meter. If it’s full, you’re full of energy, and it’s all the way green… And if I’m really low on energy, I’ve got a red bar.”}} \DIFadd{Recognizable icons, such as the rainbow infinity symbol to represent neurodiversity, were also valued; however, participants specifically criticized harmful iconography, such as the light blue puzzle piece representing the Autism Speaks organization. Additionally, }\DIFaddend P11, a designer by trade, \DIFdelbegin \DIFdel{drew on his experience with video games to suggest ways to represent his disability through icons: 
}%DIFDELCMD < 

%DIFDELCMD < \begin{quote} 
%DIFDELCMD <     %%%
\textit{\DIFdel{``It's probably influenced by video games and Internet culture…where there's so much going on the screen in front of you, and you can't really remember what every icon means. … So “I” is Information…You click that…and the general notice is also a symbol…because of the sensitivity of the types of people involved. This universal image for neurodiversity.”.”}} %DIFAUXCMD
\DIFdel{(P11, m, 28 years old)
}%DIFDELCMD < \end{quote} 
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{Notably, P11 }\DIFdelend \DIFaddbegin \DIFadd{proposed a specific idea for disclosing his disability through design patterns and iconography. Notably, he }\DIFaddend described the importance of the transient nature of this representation \DIFdelbegin \DIFdel{in facilitating social interactions:
}\DIFdelend \DIFaddbegin \DIFadd{so as not to greatly disrupt social interactions.
}\DIFaddend 

\begin{quote} 
\DIFdelbegin \textit{\DIFdel{``I would imagine that when the user clicks }%DIFDELCMD < [%%%
\DIFdel{the "I"}%DIFDELCMD < ] %%%
\DIFdel{the image pops up for only a few moments in time, right?...That way, you can continue your interactions and virtual space without necessarily having the label on you constantly.”}} %DIFAUXCMD
\DIFdelend \DIFaddbegin \DIFadd{“}[\DIFadd{This idea is}] \DIFadd{probably influenced by video games and internet culture… where there’s so much going on the screen in front of you, and you can’t really remember what every icon means. … So “i” is Information… You click that… }[\DIFadd{and it pops up}] \DIFadd{this universal image for neurodiversity. … I would imagine that when the user clicks }[\DIFadd{the “i”}]\DIFadd{, the image pops up for only a few moments… That way, you can continue your interactions and virtual space without necessarily having the label on you constantly.” }\DIFaddend (P11, \DIFdelbegin \DIFdel{m, 28 years old}\DIFdelend \DIFaddbegin \DIFadd{28M}\DIFaddend )
\end{quote} 

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{imgs/P11.png}
    \caption{Participant 11’s images, sticky notes, and suggestions for invisible disability representation during the whiteboard component of the study, featuring an information icon and the ADHD rainbow butterfly symbol above the avatar.} 
    \Description{Participant 11’s images, sticky notes, and suggestions for invisible disability representation during the whiteboard component of the study. There is an image of Toad, an anthropomorphized mushroom character from the Mario franchise, wearing an astronaut suit and helmet. On his cap, there is an information icon (a lowercase i in a circle) and above Toad is the ADHD rainbow butterfly symbol. To Toad’s right, there is a sticky note that reads, “General notice of invisible disability - other users can click to reveal more information. More information is presented as a specific symbol represen-”. To the right of the ADHD symbol, there is a sticky note reading “Symbol is animated and hovers on top the avatar for a few seconds after the (i) button is clicked.”}
    \label{P11}
\end{figure*}

\DIFdelbegin \DIFdel{Some participants (P2, P6) were interested in disability representations that floated above their avatars, such as an awareness flag or a dynamic energy bar that correlated with their energy level or “social battery. ” As an accommodation feature, this interfaces interestingly with P11}\DIFdelend \DIFaddbegin \DIFadd{Disability representations also included temporary adjustments to the avatar to indicate a user}\DIFaddend ’\DIFdelbegin \DIFdel{s proposal of }\DIFdelend \DIFaddbegin \DIFadd{s interest in engaging with others. Similar to the energy bar example, P11 proposed }\DIFaddend a feature that would allow an avatar to turn invisible when \DIFdelbegin \DIFdel{its user wants }\DIFdelend \DIFaddbegin \DIFadd{a user wanted }\DIFaddend to avoid social interactions\DIFdelbegin \DIFdel{. Turning invisible would convey nonverbally that a person does not want to be approached.
}%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdelend \DIFaddbegin \DIFadd{, which he dubbed as a }\textit{\DIFadd{“stealth mode.”}} \DIFaddend However, P11 \DIFdelbegin \DIFdel{quickly engaged critically with the potential }\DIFdelend \DIFaddbegin \DIFadd{assessed the potential privacy }\DIFaddend implications of implementing such a feature\DIFdelbegin \DIFdel{: 
}\DIFdelend \DIFaddbegin \DIFadd{, and concluded that turning an avatar translucent could convey a similar message of wishing to keep to themself while still alerting other users to the fact that there was another user within the space.
}\DIFaddend 

\begin{quote} 
\DIFdelbegin \textit{\DIFdel{``If you think about the other users of the space, do you really want an invisible person watching you? Because you can see them. … I guess if you are engaging in this space, you sort of have to descend. Maybe rather than being invisible, you can have a great observation of your avatar. So my }%DIFDELCMD < [%%%
\DIFdel{avatar}%DIFDELCMD < ]%%%
\DIFdel{, who’s red and blue, right? I can just make him more white }%DIFDELCMD < [%%%
\DIFdel{translucent}%DIFDELCMD < ] %%%
\DIFdel{instead, so he’s like one of them. ‘Just don't come to me. }%DIFDELCMD < [%%%
\DIFdel{He’s}%DIFDELCMD < ] %%%
\DIFdel{not really colorful right now.’”}} %DIFAUXCMD
\DIFdelend \DIFaddbegin \DIFadd{“If I’m in }[\DIFadd{a}] \DIFadd{VR space and I just want to enjoy myself, and I don’t want anyone coming up to me, I should be able to say that. … }[\DIFadd{but}] \DIFadd{if you think about the other users of the space, do you really want an invisible person watching you? … Maybe rather than being invisible… I can just make him more white }[\DIFadd{translucent}] \DIFadd{instead… ‘Just don’t come to me. }[\DIFadd{My avatar’s}] \DIFadd{not really colorful right now.’” }\DIFaddend (P11, \DIFdelbegin \DIFdel{m, 28 years old}\DIFdelend \DIFaddbegin \DIFadd{28M}\DIFaddend ) 
\end{quote} 

\DIFdelbegin \DIFdel{This specific example speaks to the uniqueness of the embodied experience that social VR offers its users highlighting an affordance impossible in the physical world and offering humans an option to change colors like a chameleon, continuing the theme of avatars affording novel self-expression through non-humanoid embodiment. 
}\DIFdelend \DIFaddbegin \DIFadd{Participants’ public representations of their disability utilized unique affordances of the embodied avatar experience, such as wearing custom-designed clothes and accessories to advocate for invisible disabilities, having a visible “energy bar” to indicate mood and energy level, and changing colors to express one’s willingness to interact with others. 
}

\subsubsection{\DIFadd{Private Representations and Expressions of Disability}}
\DIFaddend Below, we describe how participants explored \DIFdelbegin \DIFdel{representations }\DIFdelend \DIFaddbegin \DIFadd{different expressions }\DIFaddend infused with personal meanings\DIFdelbegin \DIFdel{that are as invisible as their disabilities. 
}%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{For example, P8 gave his avatar earbuds during the creative exercise, explaining: }\textit{\DIFdel{``I’m not a big earbud guy, I'm a headphone wearer… }%DIFDELCMD < [%%%
\DIFdel{but}%DIFDELCMD < ] %%%
\DIFdel{I feel like maybe it would be an extension of you trying to conceal what invisible disabilities I would have, just pretending to be normal with stuff like that.”}} %DIFAUXCMD
\DIFdel{While this representation of his invisible disability was not explicit to others, he acknowledged that his avatar was }\textit{\DIFdel{``more of an expression of }%DIFDELCMD < [%%%
\DIFdel{him}%DIFDELCMD < ]%%%
\DIFdel{.”}} %DIFAUXCMD
\DIFdel{and preferred to keep this aspect abstract}\DIFdelend \DIFaddbegin \DIFadd{, such that they could still represent their invisible disability without necessarily disclosing a disability identity to other social VR users}\DIFaddend .

\DIFdelbegin \DIFdel{Similarly}\DIFdelend \DIFaddbegin \DIFadd{Participants primarily suggested representing their disability identities or experiences through accessories that matched those that they would wear in non-virtual settings. For example}\DIFaddend , P3 preferred more subtle accessories that would more closely resemble non-virtual affordances: \textit{\DIFdelbegin \DIFdel{``}\DIFdelend \DIFaddbegin \DIFadd{“}\DIFaddend I would do it with accessories, [but] I don\DIFdelbegin \DIFdel{'}\DIFdelend \DIFaddbegin \DIFadd{’}\DIFaddend t want a big sign saying, \DIFdelbegin \DIFdel{`}\DIFdelend \DIFaddbegin \DIFadd{‘}\DIFaddend disabled’ or a different color flashing over here that says \DIFdelbegin \DIFdel{`}\DIFdelend \DIFaddbegin \DIFadd{‘}\DIFaddend invisible illness is no longer invisible.’\DIFdelbegin \DIFdel{But I would do it with subtle accessories. Something a little more real.’’}}%DIFDELCMD < \MBLOCKRIGHTBRACE 
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{Speaking of “real}\DIFdelend ”\DIFdelbegin \DIFdel{accessories, or those rooted in non-virtual environments, }\DIFdelend \DIFaddbegin \DIFaddend P12 \DIFaddbegin \DIFadd{also }\DIFaddend wanted to use clothing or accessories that blurred private and public significance: 

\begin{quote}
\DIFdelbegin \textit{\DIFdel{``For me, I utilized my interest in cars as both something to therapeutically do but also maybe relate to others that have that same interest. Which is why I also, in real life, like to collect diecast cars and books on cars and, sometimes, I also like to wear clothing with cars on it. This is more of a social preference. I don't know how that would represent my disability entirely, but if }%DIFDELCMD < [%%%
\DIFdel{others}%DIFDELCMD < ] %%%
\DIFdel{at least understand my passions and interests and how knowledgeable I am about them, then maybe they have a better understanding of me, too. On a personal level, at least.”}} %DIFAUXCMD
\DIFdelend \DIFaddbegin \DIFadd{“For me, I utilized my interest in cars as both something to therapeutically do but also maybe relate to others that have that same interest. Which is why I also, in real life, like to collect diecast cars and books on cars and, sometimes, I also like to wear clothing with cars on it. This is more of a social preference. I don’t know how that would represent my disability entirely, but if }[\DIFadd{others}] \DIFadd{at least understand my passions and interests and how knowledgeable I am about them, then maybe they have a better understanding of me, too. On a personal level, at least.” }\DIFaddend (P12, \DIFdelbegin \DIFdel{m, 31 years old}\DIFdelend \DIFaddbegin \DIFadd{31M}\DIFaddend )
\end{quote} 

\DIFdelbegin \DIFdel{Two other participants (P5, }\DIFdelend \DIFaddbegin \DIFadd{Others used accessories that they didn’t wear in the physical world, but still carried meaning to the participant. During the creative exercise, P8 gave his avatar earbuds, explaining: }\textit{\DIFadd{“I’m not a big earbud guy, I’m a headphone wearer }[\DIFadd{in the physical world}]\DIFadd{… }[\DIFadd{but}] \DIFadd{I feel like maybe it would be an extension of you trying to conceal what invisible disabilities I would have, just pretending to be normal with stuff like that.”}} \DIFadd{While this representation of his invisible disability was not explicit to others, he acknowledged that the earbuds were }\textit{\DIFadd{“more of an expression of }[\DIFadd{him}]\DIFadd{”}} \DIFadd{and preferred to keep this aspect abstract. P14 also utilized headphones and a mask as symbolism for }\textit{\DIFadd{“blocking out all the noise”}} \DIFadd{in the environment. Similarly, }\DIFaddend P9 \DIFdelbegin \DIFdel{) were interested in representations of personal significance rather than using them to communicate with other users. For example, P9 used vibrant colors: }\textit{\DIFdel{``It's a way that I can visually differentiate myself from a room full of other people. It's my way of not just indicating to others that this person’s a little different, but it's also indicating to myself that I'm a little different.”}}
%DIFAUXCMD
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{P9 also established his interest in using his social VR avatar to tell a complex and storied narrative through the deceptively commonplace selection of elbow and knee pads in }\DIFdelend \DIFaddbegin \DIFadd{also described how }\DIFaddend his ideal avatar representation \DIFdelbegin \DIFdel{: 
}\DIFdelend \DIFaddbegin \DIFadd{included elbow and knee pads: 
}

\DIFaddend \begin{quote}
\DIFdelbegin \textit{\DIFdel{``I really want to add knee and elbow pads. If you have ever gone roller skating, you need to put on knee and elbow pads, just in case you fall... The bipolar makes me swing really hard to the left and right. I get these mania phases and these depression phases that have a whiplash to them. And sometimes... I can get hurt or accidentally hurt others. So these pads on my knees and elbows would be a way to symbolize that if I do fall, I gotta make sure I'm protected. I don't fall too hard, and I can stand up again.’’}} %DIFAUXCMD
\DIFdelend \DIFaddbegin \DIFadd{“I really want to add knee and elbow pads. If you have ever gone roller skating, you need to put on knee and elbow pads, just in case you fall… The bipolar makes me swing really hard to the left and right. I get these mania phases and these depression phases that have a whiplash to them. And sometimes… I can get hurt or accidentally hurt others. So these pads on my knees and elbows would be a way to symbolize that if I do fall, I gotta make sure I’m protected. I don’t fall too hard, and I can stand up again.” }\DIFaddend (\DIFdelbegin \DIFdel{P9, m, 28 years old)
}\DIFdelend \DIFaddbegin \DIFadd{P9, 28M)
}\DIFaddend \end{quote}

\DIFdelbegin \DIFdel{Disability is one facet of a complex human experience that is filtered through intersecting lenses of other identities like gender and race.Participants identified connections between the experiences of people in distinct marginalized groups. P12 also compared disclosing invisible disabilities to disclosing sexuality and gender identity, citing LGBTQ award-winners at the Tony Awards as examples of ways that queer people expressed and disclosed their identity through clothing and other visual means. }%DIFDELCMD < 

%DIFDELCMD < \begin{figure*}[t]
%DIFDELCMD <     \centering
%DIFDELCMD <     \includegraphics[width=\linewidth]{imgs/P12.png}
%DIFDELCMD <     %%%
%DIFDELCMD < \caption{%
{%DIFAUXCMD
\DIFdelFL{Participant 12’s images, sticky notes, and suggestions for invisible disability representation during the whiteboard component of the study, featuring screenshots of two different avatars he uses. The images are blurred to preserve the participant's anonymity.}} 
    %DIFAUXCMD
%DIFDELCMD < \Description{Participant 12’s images, sticky notes, and suggestions for invisible disability representation during the whiteboard component of the study. On the top there are four sticky notes, reading “Important notes for Autism and Aspergers with Avatars in VR: 1. Make sure facial expressions and non verbal expressions are accurate and can also include descriptions as needed.” / “For those who also may be LGBTQ or have a physical disability, have accurate representations of them.” / “Offer opportunity to have a community for those to share similar interests as a way of  improving socialization” / “Learn behavioural techniques in virtual environments and inhibit restrictions to help.” Below the sticky notes are three screenshots of P12’s avatar. On the left is a screenshot of his avatar’s head and torso with a box sketched to the right of his head. The avatar is 3D, light-skinned, has a beard, short hair, sunglasses, and a Unity sweatshirt. The middle screenshot shows a 2D avatar with glasses, a goatee, and wearing a blue shirt with a brown vest; the avatar’s hands are raised and it says “Happy New Year!” above his head. The screenshot on the right is a zoomed out version of the screenshot on the left, showing the 3D avatar’s whole body.}
%DIFDELCMD <     \label{P12}
%DIFDELCMD < \end{figure*}
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{On another note, }\DIFdelend \DIFaddbegin \DIFadd{Three participants were interested in alterations to their avatar itself, beyond accessories, that could indicate their difference from other users in an implicit way. For example, P9 used vibrant colors: }\textit{\DIFadd{“It’s a way that I can visually differentiate myself from a room full of other people. It’s my way of not just indicating to others that this person’s a little different, but it’s also indicating to myself that I’m a little different.”}} \DIFaddend P10 \DIFaddbegin \DIFadd{also }\DIFaddend expressed that her avatar\DIFaddbegin \DIFadd{’s large bushy tail }\DIFaddend represented her comfort zone and personal bubble\DIFdelbegin \DIFdel{, a current customization option she valued (and the only current yet implicit example of disability representation we found available on customization platforms at present): 
}%DIFDELCMD < 

%DIFDELCMD < \begin{quote} 
%DIFDELCMD <     %%%
\textit{\DIFdel{``Its tail wraps around it a lot as it's moving, or if you stand still… but I like that one because, in some weird way, it gives me a comfort zone of hiding me in a bubble. I don't know, I never found one that did that. So, when I came across that one, I just liked it. Even in real life, people have said I have a bubble, like a huge bubble around me. It’s like you get too close to me, and I’m kinda like… I just back away a little.”}} %DIFAUXCMD
\DIFdel{(P10, f, 52 years old)
}%DIFDELCMD < \end{quote}
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{P10 }\DIFdelend \DIFaddbegin \DIFadd{. She }\DIFaddend described using her humanoid and avatar-based self-expression as a metaphor for her non-virtual personality, further emphasizing the unique affordances of social VR in expanding the bounds of self-expression by \DIFdelbegin \DIFdel{alllowing }\DIFdelend \DIFaddbegin \DIFadd{allowing }\DIFaddend fantastical and metaphorical representations of the self. 

\DIFdelbegin \DIFdel{While }\DIFdelend \DIFaddbegin \begin{quote} 
\DIFadd{“Its tail wraps around it a lot as it’s moving, or if you stand still… but I like that one because, in some weird way, it gives me a comfort zone of hiding me in a bubble. … Even in real life, people have said I have a bubble, like a huge bubble around me. It’s like you get too close to me, and I’m kinda like… I just back away a little.” (P10, 52F)
}\end{quote}

\DIFadd{Though some participants brainstormed representations of disability were intended to be explicit, they realized that their ideas could still be implicit to other social VR users. For example, P9 emphasized how his embodied avatar reflected his mood, especially related to his experiences with Bipolar Type 1. He used VR avatar appearances to communicate his emotions nonverbally, strategically selecting avatars based on his goals for social interactions that day. He explained his use of colors and their social and psychological effects: 
}

\begin{quote}
\DIFadd{“The middle avatar is the avatar I use when I’m in a playful mood. It stands out, but it’s also really friendly looking. I got a lot of people that like to hang around with me in this one if I’m feeling energetic, a little bit extroverted. If we talk about bipolar phases a little bit more, like the manic phase, I’ll use the middle one. … If I’m in a really happy mood, but I pick an avatar with like no color, for few emotions, it wouldn’t really match. Same thing vice versa. It also adds some novelty to VR chat as well, because if I see myself in the same avatar for too long, I feel like I start to get fixed. I start to lock myself in the avatar. So, I like to mix it around, so I know there’s always flexibility to iterate and change.” (P9, 28M) 
}\end{quote}

\DIFadd{Similarly, while }\DIFaddend P5 wished to use glowing veins to represent chronic pain, he acknowledged that other users might not understand the disability-related symbolism: \textit{\DIFdelbegin \DIFdel{``That would show things more, but that }\DIFdelend \DIFaddbegin \DIFadd{“}[\DIFadd{the glowing veins}] \DIFaddend still wouldn\DIFdelbegin \DIFdel{'}\DIFdelend \DIFaddbegin \DIFadd{’}\DIFaddend t even show pain, because people are gonna look at that and just go like, ‘cool.’ They just see glowing things on your arm.\DIFdelbegin \DIFdel{’’}\DIFdelend \DIFaddbegin \DIFadd{”}\DIFaddend } \DIFdelbegin %DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{To P5’s point}\DIFdelend \DIFaddbegin \DIFadd{Even though most other social VR users would not understand that a disability was being expressed}\DIFaddend , these private and often implicit representations of disability were \DIFaddbegin \DIFadd{still }\DIFaddend valuable to participants\DIFdelbegin \DIFdel{even though most other social VR users would not make the logical leap necessary to understand that a disability was being expressed }\DIFdelend .

\DIFdelbegin \subsection{\DIFdel{Suggested Features for Customizing Disability Representations}}
%DIFAUXCMD
\addtocounter{subsection}{-1}%DIFAUXCMD
\DIFdelend \DIFaddbegin \subsection{\DIFadd{Invisible Disability Disclosure Practices Differed Based on A User’s Context}}
\DIFadd{In this section, we explore participants’ varied motivations for disclosing or sharing their disability identity, informed by both different social VR environments and the dynamic nature of their disabilities. Then, we highlight participants’ suggested customization features and methods for making the customization process more accessible. 
}\DIFaddend 

\DIFaddbegin \DIFadd{A variety of social factors influenced participants’ disclosure strategies: some were comfortable with disclosing their identity at all times, some preferred disclosing only some of the time, and others did not want to disclose in social VR at all. We found that participants generally belonged to one of three groups: }\textbf{\DIFadd{Activists}}\DIFadd{, }\textbf{\DIFadd{Non-Disclosers}}\DIFadd{, and }\textbf{\DIFadd{Situational Disclosers}}\DIFadd{. }\textbf{\DIFadd{Activists}} \DIFadd{were always open to disclosing to spread education and awareness, often tying into advocacy work that the participants did outside of social VR contexts. }\textbf{\DIFadd{Non-Disclosers}} \DIFadd{did not want to disclose their invisible disability to others in any circumstances. Lastly, }\textbf{\DIFadd{Situational Disclosers}} \DIFadd{were sometimes open to disclosing their identity, and would rely on context cues to make their disclosure decisions. 
}

\subsubsection{\DIFadd{Activists and Non-Disclosers}}
\DIFadd{One participant was part of the }\textbf{\DIFadd{Activist}} \DIFadd{group: P1 identified as an outspoken disability activist and felt comfortable openly sharing her disability identity in social VR. She felt that disclosing her chronic condition was helpful not only for raising awareness but also for indicating her access needs.
 }

\begin{quote}
\DIFadd{“I am an activist and an advocate for folks that have invisible disabilities… I’m an open book. So anything that can start a conversation or encourage people to ask questions is really valuable to me, and I feel like having that option is just really important in terms of raising awareness for things like that. And I like people to actually know. If I’m going to start a friendship with somebody, I want them to be aware of the fact that I have a chronic illness, because that is a pretty large part of my life, and it does affect my ability to socialize sometimes. So you know, being open about that is important to me personally.” (P1, 32F)
}\end{quote}

\DIFadd{On the other hand, one participant was not comfortable disclosing their disability identity in social VR at all. P8, a }\textbf{\DIFadd{Non-Discloser}}\DIFadd{, concealed his invisible disability in all non-virtual social situations and did not want to disclose in social VR either, as he felt that }\textit{\DIFadd{“}[\DIFadd{others}] \DIFadd{wouldn't be very receptive or kind to that”}} \DIFadd{and he did not want to be treated as }\textit{\DIFadd{“lesser than someone else.”}} \DIFadd{He emphasized that his invisible disability was not a core part of his identity, especially as it was }\textit{\DIFadd{“a condition that didn’t come until the last five years or so, so it’s not like I grew up with it”}} \DIFadd{(P5). Additionally, having observed others face negative stigmas strengthened his opinion of not disclosing his identity in any contexts, VR or otherwise: 
}

\begin{quote}
\DIFadd{“It comes from personal experience, because I've known people in the past… friends that have also had }[\DIFadd{my condition}]\DIFadd{, it's like you're treated differently. … It probably wouldn’t come up unless someone else brought it up… I’m trying to hide it so much that, outside of my family, I don’t think I ever opened up to anyone about it.” (P8, 20M)
}\end{quote}

\subsubsection{\DIFadd{Situational Disclosers: Disclosure Practices Informed by Perceptions of Stigma}}
\DIFadd{Participants’ different contexts, which encompassed both the VR environment and their day-to-day disability experience, had a strong impact on when and why they chose to disclose their invisible disability. While only a couple of participants identified as Activists or Non-Disclosers, the remaining 12 participants expressed varying degrees of excitement and hesitancy to represent their disability identity. Most did not want to disclose their disabilities in large group contexts because of their perceptions of the stigma they would face and due to prior negative experiences with disclosure. For example, P9 mentioned how he tried to mask or pass as nondisabled when interacting with others in social VR: }\textit{\DIFadd{“I don’t really represent my disability too much, but I also don’t conceal it.”}}

\DIFadd{For six Situational Disclosers, their intended audience significantly influenced their avatar design choices, and they often chose to disclose to support other disabled people in a safe space. For example, P3, P4, P6, and P9 stated that they were more likely to disclose in a disability-specific community rather than a large social situation. P9 also specifically mentioned that disclosing in this context allowed them to empathize and engage by sharing }\textit{\DIFadd{“something that I struggle with as well”}} \DIFadd{(P9). Similarly, P2 felt that sharing more about their experience through their bio could provide support to others who were having trouble navigating their invisible disability: }\textit{\DIFadd{“I very much enjoy }[\DIFadd{being}] \DIFadd{open with people, especially once I’ve made a connection with them. I don’t feel like it puts me at any risk or any danger… if anything, it adds to my support system.”}} \DIFadd{P4 also acknowledged that she did not want to disclose her disability to just any person in social VR: }\textit{\DIFadd{“we would mostly have to become friends outside of the virtual reality world for me to feel comfortable to disclose it.”}}

\DIFadd{Regardless of the scale of a social context, some felt as though certain disabilities carried more stigma compared to others. P4 was interested in disclosing two of her invisible disabilities but not a third \textemdash{} she felt comfortable representing dyslexia and chronic pain, but not epilepsy: }\textit{\DIFadd{“I’ve had more hatred for }[\DIFadd{having epilepsy}] \DIFadd{than dyslexia because most people understand dyslexia.”}} \DIFadd{Furthermore, P5 mentioned that the stigmas associated with Asperger’s and ADHD were }\textit{\DIFadd{“embarrassing”}} \DIFadd{and commonly }\textit{\DIFadd{“poked fun at a lot online,”}} \DIFadd{which furthered his concerns of being disrespected due to the }\textit{\DIFadd{“negative public perception”}} \DIFadd{of his disabilities. P12 also described their prior experiences of facing discrimination against neurodivergent people: 
}

\begin{quote}
\DIFadd{“I don't go out of my way all the time in VR to disclose my disability. Some, if not many, people may not fully understand what the disability is about. Or, they'll jump to conclusions and assume… I don't want to get labeled that way. I don't want to be labeled as someone who's }[\DIFadd{r-word}]\DIFadd{. Unfortunately, which you know, that word has been thrown around a lot recently and with very negative connotations.” (P12, 31M)
}\end{quote}

\DIFadd{Given the dynamic and fluctuating nature of some invisible disabilities, some participants expressed that their disclosure preferences changed as needed. For example, P2, P6, and P10 chose to disclose their disability based on their mood or flare-ups. P2 mentioned that she would sometimes disclose their disability to help others }\textit{\DIFadd{“understand what I’m going through… to avoid conflict,”}} \DIFadd{especially in a work setting. P6 also noted that }\textit{\DIFadd{“I really only disclose if I feel like I’m about to have a flare up.”}} \DIFadd{Similarly, P10 mentioned: }\textit{\DIFadd{“when my Hashimoto’s flares up, I lose lots of hair, I have no energy, and I am just tired… So people }[\DIFadd{can be like}]\DIFadd{, ‘Okay, she’s dealing with that today.’”}} \DIFadd{P3 elaborated on how having customizable avatars played a psychological role in grounding her VR experiences: }\textit{\DIFadd{“}[\DIFadd{having options}] \DIFadd{gives you virtual reality with just a little bit of more normalcy. … It gives you a little bit of an anchor to not overwhelm you”}} \DIFadd{(P3).
}

\DIFadd{Participants also shared how they wished to toggle specific avatar features on and off to support  their dynamic disclosure preferences. P9 shared that he felt comfortable and open to disclosing their disability in social VR, but that having a toggle for disclosure features could be crucial for avoiding ableism in unwelcoming settings. As someone with social anxiety, P10 also thought that having options to both (1) have her disability representation permanently fixed to their avatar and (2) select her disability representation on a daily basis would be most helpful: }\textit{\DIFadd{“if you have social anxiety every single day, there’s no reason to switch that on and off. That gives you anxiety, having to go do that every day.”}} \DIFadd{P3 explained how the toggles could be used for not only representing, but also managing her invisible disability: 
}

\begin{quote}
\DIFadd{“My VR Avatar is whatever I’m feeling at the moment. If I’m feeling immersed in my invisible illness, then I’m probably gonna want my avatar to be also. And if I’m feeling like, ‘okay, I’m escaping reality,’ I don’t want my avatar to be even close to what I am. }[\DIFadd{In our support group,}] \DIFadd{there will still be some days that I don’t want to manifest }[\DIFadd{my disability}]\DIFadd{. And then other days where it’s like, ‘Yeah, I’m feeling like crap and I’ll let you people know it in a non-verbal way,’ and I will come in there all crippled up with my avatar, altered to represent how I feel right now simply because I am trying to communicate it in a nonverbal way.” (P3, 56F)
}\end{quote}

\subsubsection{\DIFadd{Social VR vs. Non-Virtual Disclosure Preferences}}
\DIFadd{Some participants perceived social VR to be a relatively safe space where they could freely express their disability-related identities without worrying as much about the stigma they faced in the non-virtual world. For example, a few participants felt more open to disclosing disabilities in social VR because a disability label would not persist beyond their VR experience. P9 explained: }\textit{\DIFadd{“I feel like once I label myself }[\DIFadd{with a disability}] \DIFadd{in real life, it becomes something that kind of follows you around.”}} 

\DIFadd{However, others felt as though social VR experiences ranged from relatively safe communities to potentially harmful environments. For example, P13 recalled a news article reporting about a woman being assaulted in social VR spaces, and briefly mentioned his own experiences of being assaulted in VR. When speaking about specific VR platforms, P1 acknowledged how disability disclosure in social VR could potentially result in harassment:  
}

\begin{quote}
\DIFadd{“Personally, I’m totally fine with having }[\DIFadd{disability representations}] \DIFadd{on all the time. But I really understand why somebody wouldn’t want to have that option to turn it off, especially if you’re going into more of a rough and rowdy crowd, like in VR Chat. You don’t want to make yourself a target for people that might look for things to hurt you with. A lot of the communities that I hang out in on all social VR platforms, typically, I know that the people that are hanging out there are going to be more kind, empathetic people. But if you’re going to a place that you don’t really know very well, I think it would be a good idea to be able to turn that off or on.” (P1, 32F) 
}\end{quote}

\subsubsection{\DIFadd{Intersectional Identity Representation}}
\DIFadd{Disability is one facet of the complex human experience, filtered through intersecting lenses of other identities like gender and race. Participants identified connections between the experiences of people in multiple marginalized groups. Speaking to experiences of other identities, P6 acknowledged her intersectional identities of race and invisible disability but had varying perspectives on whether to represent them in her avatars. Her daily experiences in social and workplace settings also informed her avatar disclosure preferences:
}

\begin{quote}
\DIFadd{“I feel like I’m seen as unreliable. Obviously, I’m also a Black woman, so that compounds things \textemdash{} that intersection of discrimination. But I do feel like I actively do not get treated well when I talk about it. I guess in social situations, I'm not concerned about it the way that I am in professional circumstances. … The intersection of disability and race has made me a lot less likely to disclose over the years. As I’ve seen, figures of authority are not necessarily empathetic or respectful about it.” (P6, 24F)
}\end{quote}

\DIFadd{When speaking about the personal importance of disclosing his invisible disability identity, P12 drew parallels between LGBTQ and disability representation in media. He cited LGBTQ award-winners at the Tony Awards as examples of ways that queer people expressed and disclosed their identity through clothing and other visual means.
}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{imgs/P12.png}
    \caption{\DIFaddFL{Participant 12’s images, sticky notes, and suggestions for invisible disability representation during the whiteboard component of the study, featuring screenshots of two different avatars he uses. The images are blurred to preserve the participant’s anonymity.}} 
    \Description{Participant 12’s images, sticky notes, and suggestions for invisible disability representation during the whiteboard component of the study. On the top there are four sticky notes, reading “Important notes for Autism and Aspergers with Avatars in VR: 1. Make sure facial expressions and non verbal expressions are accurate and can also include descriptions as needed.” / “For those who also may be LGBTQ or have a physical disability, have accurate representations of them.” / “Offer opportunity to have a community for those to share similar interests as a way of  improving socialization” / “Learn behavioural techniques in virtual environments and inhibit restrictions to help.” Below the sticky notes are three screenshots of P12’s avatar. On the left is a screenshot of his avatar’s head and torso with a box sketched to the right of his head. The avatar is 3D, light-skinned, has a beard, short hair, sunglasses, and a Unity sweatshirt. The middle screenshot shows a 2D avatar with glasses, a goatee, and wearing a blue shirt with a brown vest; the avatar’s hands are raised and it says “Happy New Year!” above his head. The screenshot on the right is a zoomed out version of the screenshot on the left, showing the 3D avatar’s whole body.}
    \label{P12}
\end{figure*}

\subsection{\DIFadd{Accessible Methods for Customizing Avatars}}
\DIFaddend Five participants (P1, P2, P4, P5, P7) expressed interest in easier processes for importing and creating custom designs. P4 suggested \DIFdelbegin \DIFdel{: }\DIFdelend \DIFaddbegin \DIFadd{having }\DIFaddend \textit{\DIFdelbegin \DIFdel{``It'd be nice to have }\DIFdelend \DIFaddbegin \DIFadd{“}\DIFaddend different options, like with different logos or different quotes that you want to put on shirts. It\DIFdelbegin \DIFdel{'}\DIFdelend \DIFaddbegin \DIFadd{’}\DIFaddend d be nice to have a set-up so that you can do it pretty easily [because] I definitely don\DIFdelbegin \DIFdel{'}\DIFdelend \DIFaddbegin \DIFadd{’}\DIFaddend t have the coding experience to be able to go any further.\DIFdelbegin \DIFdel{’’}\DIFdelend \DIFaddbegin \DIFadd{”}\DIFaddend } \DIFdelbegin %DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{Additionally, }\DIFdelend \DIFaddbegin \DIFadd{Another participant explained that current avatar customization processes were inaccessible due to the physical manifestations of their disability that impacted their mobility. }\DIFaddend P5 \DIFdelbegin \DIFdel{wanted }\DIFdelend \DIFaddbegin \DIFadd{wished }\DIFaddend to minimize arm movement requirements due to Repetitive Strain Injury\DIFaddbegin \DIFadd{, }\DIFaddend and shared ideas for optimizing user experiences through evolving technology: 

\begin{quote} 
\DIFdelbegin \textit{\DIFdel{``I could copy and paste it. That's my ideal customization because I don't like the menus. If you have the option of pressing a bunch of buttons or just being able to think it and it appears on the page, why would anyone want to have all the billion options when they could do the exact same thing? It has occurred to me, though, like with the recent AI developments, where you can produce pictures, it seems like it's not too far away that they could just produce a 3D model using those systems. Like if there was a system where you could describe it, and it would generate one.’’}} %DIFAUXCMD
\DIFdelend \DIFaddbegin \DIFadd{“I could copy and paste it. That’s my ideal customization because I don’t like the menus. If you have the option of pressing a bunch of buttons or just being able to think it and it appears on the page, why would anyone want to have all the billion options when they could do the exact same thing? It has occurred to me, though, with the recent AI developments, where you can produce pictures, it seems like it’s not too far away that they could just produce a 3D model using those systems. Like if there was a system where you could describe it, and it would generate one.” }\DIFaddend (P5\DIFdelbegin \DIFdel{, m, 31 years old) 
 }\DIFdelend \DIFaddbegin \DIFadd{, 31M) 
 }\DIFaddend \end{quote}

\DIFdelbegin \DIFdel{Even though invisible disabilities often have unrecognizable and misinterpreted features, some have physical manifestations that can impact mobility. For P5, his constrained arm movements shaped the way he approached avatar customization and ultimately his vision for an ideal customization process. }%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{P11 also had a wealth of ideas for ways to customize avatars, including }\textit{\DIFdel{``simple sliders and buttons…3D models you can customize…options to select what types of disabilities and neurodivergent conditions you identify as, and then you get a chance to customize the symbols or the icons.”}} %DIFAUXCMD
\DIFdel{He explained: }\textit{\DIFdel{``I think an ability for you to be able to type in what you’re saying or what you want through maybe image generation or text to 3D tools would be a great way to do that,”}} %DIFAUXCMD
\DIFdel{which would reduce the burden of users navigating complex customization systemswithin social VR systems themselves. }\DIFdelend Participants also mentioned that text-to-avatar pipelines could lower the barrier to avatar customization, which was perceived as intimidating for participants who did not know how to use Unity or other platforms that rely on user coding. \DIFaddbegin \DIFadd{P11 had multiple ideas for ways to customize avatars, including }\textit{\DIFadd{“simple sliders and buttons… 3D models you can customize… options to select what types of disabilities and neurodivergent conditions you identify as, and then you get a chance to customize the symbols or the icons.”}} \DIFadd{He felt that }\textit{\DIFadd{“}[\DIFadd{being}] \DIFadd{able to type in what you’re }[\DIFadd{thinking}]\DIFadd{, or what you want through maybe image generation or text to 3D tools, would be a great way to do that,”}} \DIFadd{as it would reduce the burden of users navigating complex customization systems within social VR systems themselves. 
}\DIFaddend 

\DIFdelbegin \DIFdel{As technology continues to evolve, it is no surprise that social VR users are eager to see emerging technologies implemented in the pursuit of improving the accessibility of social VR spaces. 
A key component of building an inclusive society is purposefully using resources, such as technology, to further our societal goals. Though our participants offer only a couple of examples here, designers should consider which features of emerging technologies could help shape a more inclusive tomorrow as they are being designed and implemented across the globe. 
}\DIFdelend \section{Discussion}

Avatar customization libraries decide who gets to express what identity, and current options do not enable the explicit expression of invisible disabilities. In our study, we found that people with invisible disabilities are interested in representing their disabilities through social VR platforms. Unlike people with visible disabilities who often depict disabilities through adding assistive technology to their avatars \cite{zhang_diarystudy}, representation of invisible disabilities tend to adopt more nuanced and symbolic approaches, including clothing-based designs (such as custom disability-related graphics) as well as accessory-based features (such as a floating energy bar). Additionally, a distinction emerged between public representations with explicit meaning and more private representations with personal significance and implicit meaning. Sometimes motivated by educational and awareness-raising goals, sometimes motivated by traumatic non-virtual disclosure experiences, we discovered that context informs virtual disclosure preferences.  It is important to note that social VR offers users access to a distinct set of verbal and non-verbal cues that can powerfully communicate shifting needs and preferences. Through the unique multimodal interactions afforded by social VR avatars (e.g., synchronous voice chat, motion tracking, facial expression), we found participants leveraged disability representation in more varied ways than on social media. 

\DIFaddbegin \subsection{\DIFadd{Taxonomy for Disability Disclosure}}
\DIFadd{We discovered themes surrounding disclosure, perceptions of stigma, and novel representations of invisible disabilities, as described below. We begin by highlighting the perceptions of stigma that impact disclosure decisions. Then, we examine three motivational groups that emerged from the data: }\textbf{\DIFadd{Activists}}\DIFadd{, }\textbf{\DIFadd{Situational Disclosers}}\DIFadd{, and }\textbf{\DIFadd{Non-Disclosers}}\DIFadd{. Throughout, we examine the unique affordances of social VR that facilitate novel disability expression and disclosure considerations.
}

\DIFadd{The data indicated that participant motivations for disclosure fell into three groups. The first group, Activists, were always open to disclosing to spread education and awareness. The second group, Situational Disclosers who were sometimes open to disclosing, would rely on context cues and environmental culture to make their disclosure decisions. The third group, Non-Disclosers, could not think of a situation where they would disclose their invisible disability to others. 
}

\DIFadd{As alluded to by the taxonomy above, 
}

\DIFaddend \subsection{Leveraging multimodality to represent disability in social VR.}
Disability disclosure preferences often vary by context and condition, a nuanced choice that becomes more pronounced with social VR embodiment and real-time immersion \cite{freeman_maloney_perception_of_self}. Mack et al. \cite{mack_towards} explored contextual differences across digital gaming and social platforms such as Roblox and Snapchat but did not explore embodied avatars, yet they found that non-digital experiences can inform expectations of digital spaces, just as we discovered non-virtual experiences inform virtual preferences. Despite this area of overlap, as acknowledged by P9, the engagement afforded by social VR, compared to digital social media platforms, can greatly influence avatar perceptions. Since avatars are the predominant form of self-expression in social VR, it is imperative to ensure that people have just as much, if not more, flexibility in representing their identities as they do in non-virtual spaces. We extend prior findings on invisible disability representation by examining social VR’s multimodal affordances for identity expression. While social media limits open disclosure to 2-D visual and text, social VR offers users multiple channels for sensory expression in addition to adding wearable disability representation through embodied avatars that might not be practical to carry around in still photos (e.g., a floating and dynamic energy bar to represent the user’s energy level during embodied social interactions). 

\subsection{Enabling adaptive disability representation for context-specific needs.}
Deciding whether to disclose is an ongoing negotiation across both digital (non-embodied) and virtual (embodied) platforms. In the context of embodied social VR, a recent study revealed that avatars with disability representations were more likely to experience ableism harassment during group social interactions \cite{zhang_diarystudy}. As such, it is important to offer an easy-to-use toggle on and off feature with disability representations so users can operate with the utmost autonomy in their avatar disclosure decisions. At present, avatar design processes are complex. Customization platforms such as Ready Player Me \cite{readyplayerme} offer “hundreds of options” but are often inaccessible to people from non-technical backgrounds. To streamline the customization process, we suggest that avatar design processes implement more options relevant to invisible disabilities so that self-representation is also accessible for users from non-technical backgrounds. Further, taking inspiration from participant suggestions like the dynamic energy bar, we suggest that future avatar designs incorporate intuitive and universally applicable design conventions (e.g., traffic light color guidelines \cite{traffic_light}), allowing users to effectively express themselves.

Our findings support preliminary discussions of invisible disability representation in non-virtual contexts, where there was interest in symbolically representing and disclosing invisible disabilities through toggling representations on and off. In a higher education context, Canadian university students expressed interest in a concealable invisible disability identity marker to generate greater understanding, such as a blue dot in place of the handicapped sign associated with visible disabilities \cite{mullins_invisible_uni}. The present study’s participants strengthened and expanded on this initial suggestion by offering more actionable implementations of disability expression across various modalities, which speaks to the creativity and self-exploration offered in VR affordances versus non-virtual settings. 

\DIFaddbegin [\DIFadd{copied from the last findings section}]
\DIFadd{As technology continues to evolve, social VR users hope that emerging technologies can improve the accessibility of social VR spaces and interactions. Though our participants offer only a couple of examples here, designers should consider which features of emerging technologies could help shape a more inclusive tomorrow as they are being designed and implemented across the globe. 
}\DIFaddend \subsection{VR Customization Design Recommendations} 

Based on our findings, we offer the following list of design recommendations. 

\begin{enumerate}
\item \textbf{Create more options for multimodal customization.} 
        \begin{itemize}
            \item For some users with invisible disabilities, certain forms of communication are more comfortable than others (e.g., verbal, visual, etc.). 
	\item By making it possible for users to dive further into fine-tuning their movements and facial expressions to represent physical communication of accommodations needs and dynamic thresholds for social interaction, social VR platforms can maximize a breadth of opportunities for making social VR a better experience for those with invisible disabilities.
        \end{itemize}
\item \textbf{Include explicit options for invisible disability representation on social VR customization platforms.} 
        \begin{itemize}
            \item Even though some participants suggested highly individualized representation ideas, \textbf{we recommend including awareness-building apparel and accessory options in customization libraries} (e.g., zebra print for rare disease month, dyslexia-oriented t-shirt design, giant spoon accessory for representing chronic illness). Navigating customization can be challenging for multiple reasons (see examples below), so offering a number of pre-set invisible disability representation features can help eliminate barriers to boosting awareness and facilitating self-expression. 
        \end{itemize}
\item \textbf{Make the avatar customization process more accessible.}
        \begin{itemize}
            \item Many social VR users \textbf{do not have the programming background} necessary to manually fine-tune more individualized customization features like those that might represent invisible disabilities.
            \item People with invisible disabilities want to be able to \textbf{upload custom apparel logos and t-shirt designs} that represent their disabilities. 
            \item Because of the \textbf{personal significance of many suggested disability representations}, a number of invisible disability-related customizations would need to be individually uploaded by social VR users.
            \item Consider ways to \textbf{minimize or remove the physical burden of swiping} through long lists of customization options to enhance accessibility, including customization by way of text or drawing. 
        \end{itemize}



\section{Limitations}

The recruitment process for this study was challenging in multiple ways.  Due to the invisible nature of the disabilities in our population of interest, participants had to feel comfortable disclosing they had an invisible disability to engage in the interview. We also considered that some people with chronic illnesses, neurodivergence, or other invisible disabilities might not identify as having an invisible disability. So, we altered our language in different rounds of recruitment, ensuring we included examples of invisible disabilities in every note. Additionally, because we only included consenting adults ages 18+ in the present study, we were unable to connect with the large population of youth and teen VR users and gamers. Despite these challenges, we recruited a strong sample of 12 participants who shared many overlapping experiences while also bringing to their interviews diverse suggestions and rich viewpoints. We halted recruitment once thematic saturation was achieved. 

Given that we recruited from primarily U.S. mailing lists, we recognize the geographic limitations of this study and acknowledge the importance of situating findings in diverse cultural and socioeconomic contexts. We understand that disability representation preferences, especially those linked to established symbolism, are culturally and geographically dependent. For example, while symbols  like spoon theory’s spoon are globally recognized for representations of invisible disability, others, like the Australian use of the sunflower on apparel and accessories, are less universal. Though we recruited from organizations, listservs, and social media threads globally (with some exceptions due to legal restrictions), our present demographics collection process did not include the participant country of origin.  We acknowledge that future projects would benefit from a more globally situated and culturally sensitive lens. 

\section{Conclusion}

Avatars mediate interpersonal interactions between social VR users, but at present, no built-in options exist for people to explicitly represent invisible disabilities. In this study, we explored the avatar customization preferences of people with invisible disabilities. Users wanted to tap into VR’s multimodal affordances (e.g., facial expressions, body language) to communicate their invisible disabilities. More broadly, users were interested in representing their invisible disabilities through various explicit avatar features (e.g., clothing, floating icons), and many expressed a need for an easily usable mechanism that could toggle disability representations on and off in different contexts. Interestingly, there emerged a distinction between public and private representations of disability, introducing a new level of nuance to our prior understanding of what it means to represent disability. We offer a new perspective that takes into consideration the importance of personal significance during self-expression, in addition to explicit and widely understood symbols for invisible disabilities. To our knowledge, this is the first study to capture the avatar representation wants and needs of social VR users with invisible disabilities. Broadly, our findings contribute to the ongoing conversation of designing with and for people with invisible disabilities. We hope this study inspires more researchers to offer future contributions to the valuable study of invisible disability representation and accessibility in VR. 



==> sections/diff1.tex <==
\section{Introduction}
Like anyone else, people with disabilities want to represent their unique identities through their avatars when interacting with others in social virtual reality (VR) spaces. Among other functions, avatars are vessels for self-expression in VR \cite{freeman_maloney_perception_of_self}, and their characteristics provide cues that mediate interpersonal interactions. Social VR platforms offer users a strong sense of embodiment and freedom from some forms of physical constraint, and as more people turn to social VR for social connection, the importance of diverse mechanisms for self-expression grows \cite{falling_asleep, yalon_leisure}. However, given the varying needs of potential users of social virtual reality spaces, the accessibility community has yet to understand what kinds of avatar features  can authentically represent diverse disability identities. 

Previous research has investigated the avatar representation preferences of people with visible disabilities (e.g., d/Deaf and hard of hearing people, blind and low vision people) in social VR platforms. Zhang et al. \cite{zhang_partofme} found that users with visible disabilities wanted to use their avatars to disclose their disabilities, highlight their access needs, and raise awareness through their VR interactions. Some desired to incorporate components like signing ASL through their avatars and adding realistic and customizable assistive technology (e.g., hearing aids) to better align their avatar representations with their non-virtual self-presentations. 

However, many disabled people do not have characteristics that are immediately visible, nor do they use commonly recognized assistive technologies. 33 million people in the United States alone have invisible disabilities (approximately 10% of the U.S. population) \cite{disabledworld}. Mack et al. \cite{mack_towards} examined the avatar representation preferences of people with visible and invisible disabilities through a broad study of disability representation on digital platforms (e.g., Snapchat, Animal Crossing, Facebook). They found that users with visible disabilities wanted to implement representations of their non-virtual bodies and assistive technologies, while users with invisible disabilities wanted to use disability-related avatar symbols (e.g., words in the dyslexia-friendly font “Bionic”) to signal membership in a specific community. This distinction in preferences supports the idea that representation needs differ between visible and invisible experiences, highlighting the importance of further understanding the avatar representation wants and needs of invisibly disabled users in technology-mediated contexts. 

Avatars provide users with invisible disabilities an opportunity to make their invisible identities visible through affordances that are not available in the non-virtual world. However, prior work has not yet explored invisible disability representation in embodied avatars like those found in social VR spaces. On digital platforms, users are limited to 2D, static images of their avatars. Conversely, social VR users use embodied 3D avatars to represent themselves; VR avatars are capable of capturing much more granular nuances, extending as far as dynamic facial expressions, body language, and movement patterns as they socialize with others. Given that VR’s affordances for capturing the nuances of physical human expression far exceed digital platforms \cite{freeman_maloney_perception_of_self}, more research is needed to understand invisibly disabled users’ unique preferences for identity representation in embodied avatars and social VR spaces. 

In this paper, we extend previous work by examining the embodied avatar preferences of people with invisible disabilities, amplifying the voices and experiences of this marginalized group within a social VR context. To broaden our understanding of how we can best construct the offerings of a disability-inclusive avatar customization library, we investigated how people with invisible disabilities currently represent themselves, their desired representation mechanisms, and how these preferences might differ across social VR contexts. Specifically, we posed the following research questions: 

\begin{itemize}
	\item \textbf{RQ1:} How do embodied vs. non-embodied avatars differ, and how do  those differences impact identity representation?
	\item \textbf{RQ2:} How do people with invisible disabilities represent their disability identities in social virtual reality avatars today, and how do they wish to represent themselves on social VR avatars?
	\item \textbf{RQ3:} In what social VR contexts (when and why) do people with invisible disabilities wish to disclose their disability identities and experiences?
\end{itemize}

We conducted semi-structured interviews with 14 participants with invisible disabilities, such as ADHD, dyslexia, and rheumatoid arthritis. During the interviews, we included an interactive brainstorming component where participants drew, typed, or otherwise visualized their \textit{ideal} avatar self-representation, going beyond what is currently available on customization platforms. Understanding that verbal brainstorming often privileges interviewees who are comfortable generating ideas and expressing themselves through voice, we chose this method to offer an alternative opportunity for self-expression and accommodate a broader range of communication styles. 

We found that social VR users with invisible disabilities drew connections and distinctions between virtual and non-virtual social spaces; the embodied nature of social VR impacted their disclosure preferences. For example, some perceived social VR to be a safer space than non-virtual social spaces and felt comfortable disclosing their disability, while others preferred not to disclose due to prior uncomfortable experiences in social VR. Additionally, while some users with invisible disabilities already customized avatar appearances to indicate dynamic preferences for social engagement, many wished to lean further into customized facial expressions and body language to express their disabilities. 

We also propose a paradigm for thinking about disability representation and compare their private (i.e., implicit representations like knee pads that symbolize a need for self-protection from bipolar mood swings) vs. public (i.e., explicit representations like disability-related shirt graphics) significance. Based on our findings, we conclude with design recommendations to inform a more inclusive and accessible avatar experience (e.g., reducing the amount of arm movement required to scroll through customization offerings).

In summary, we contribute novel insights on how avatar customization can support the large and underserved population of people with invisible disabilities, which is another step toward making social VR more inclusive to all users. 

\section{Related Work}
Despite the invisible nature of some disabilities, identity representation is important. Broadly, social VR platforms lack diverse customization options (e.g., regarding body and racial diversity \cite{Lee_2014_Does, lee_whose_2011, Morris_2023_hide}). Invisible disability representation in social VR is also valuable, but even less present. By rendering invisible experiences visible, doors open for building awareness of underrepresented experiences. Further, social VR offers unique affordances for users to represent aspects of their identities in different ways compared to non-virtual contexts \cite{freeman_maloney_perception_of_self}. We build on prior literature regarding disability disclosure in employment and social contexts, social VR experiences, and avatar customization and identity expression.

\subsection{Disability Disclosure}
Many disabled people have varied perspectives on when and why to disclose their disability. Although discrimination against individuals with disabilities is legally prohibited\footnote{Both the Americans with Disabilities Act (ADA) of 1990 and Section 504 of the Rehabilitation Act of 1973 protect people from discrimination on the basis of a disability.}, disabled people face discrimination and ableism, even if it is unintentional. As a result, they may have to carefully consider whether or not to disclose their disabilities. 

At school and the workplace, people with disabilities may require accommodations to perform their roles successfully, but this disclosure heightens the risk of experiencing disability-related discrimination \cite{{lindsay_barriers_education, lindsay_work, wilton_work, schrader_workplace_climate, dalgin_hiring}. They may have less favorable outcomes than their non-disabled peers in the job application process, be socially rejected by their peers and supervisors, and fear being “reduced” to their disability \cite{pearson_job_apps, lindsay_work, lindsay_barriers_education}. They may also fear that disclosure will indirectly impact their academic and professional success due to the damage to their social image \cite{rocco_social}. People with invisible disabilities have been more successful than people with visible disabilities at concealing their disability at their discretion, especially if their condition is mild and they believe their conditions are “irrelevant” to their performance \cite{lindsay_work, schrader_workplace_climate, dalgin_hiring}. 

However, this invisibility also means that people with invisible disabilities struggle to be taken seriously when seeking accommodations. People with invisible disabilities may specifically anticipate negative perceptions stemming from a lack of understanding of their disabilities, which may make them hesitant to disclose \cite{mullins_invisible_uni}. Since invisible disabilities can require more steps to verify than visible disabilities, some people may experience barriers to feeling their disclosure was accepted. Moriña \cite{morina_barriers_education} found that students with invisible disabilities struggled with the stress and insecurity associated with “proving” their disability. Often, they were challenged by people who refused to believe they were “disabled,” which made them want to distance themselves from a disability identity and appear “normal” \cite{morina_barriers_education}. Therefore, while people with both visible and invisible disabilities anticipate and encounter stigma, people with invisible disabilities may struggle more with validating their disability to themselves and others.

In our work, we extend prior work on disability disclosure in more formal settings, such as in the workplace and in education, and explore the nuances of invisible disability disclosure in social environments. 

\subsection{Social VR Use}
Recently, social VR has gained increasing popularity, enabling immersive 3D virtual experiences by allowing users to meet, interact, and socialize in the form of avatars \cite{freeman_maloney_perception_of_self}. Unlike 2D social media and virtual worlds, social VR uniquely affords immersive embodied experiences \cite{falling_asleep}. VR head-mounted displays allow real-time body movements and gestures to be tracked and rendered in virtual environments. Although most commercial headsets do not track a user’s full body or subtler physical cues, like facial expressions and gaze, they still facilitate a greater sense of embodiment and social presence than other platforms. A person’s sense of embodiment (SoE) is characterized by their ability to control their body’s movements, experience the sensations their body does, and feel that they are within their body \cite{kilteni_soe}. By placing the user within their avatar’s body and mimicking their physical body’s experiences through first-person perspective, body tracking, and haptic and audio feedback, virtual reality facilitates SoE through avatars. Additionally, users can no longer see their physical selves and environments, resulting in them being fully immersed in VR and their virtual bodies \cite{genay_for_real}.

With these unique affordances, social VR platforms offer a variety of avatar-mediated activities and social interactions. To understand what people actually do in social VR, Maloney and Freeman \cite{falling_asleep} interviewed 30 social VR users. Their findings indicated that users enjoyed doing full-body mirroring activities with expressive movements (e.g., dancing), experiencing everyday practices (e.g., sleeping) in novel immersive ways, and practicing self-improvement skills that they normally wouldn’t do in offline worlds (e.g., social skills and mental states). Furthermore, users can connect with other users by hosting and attending parties and other gatherings, playing games together, and working remotely \cite{freeman_maloney_perception_of_self, abramczuk_remote_work}.

Social VR platforms are particularly appealing to people with disabilities since they can address accommodations in ways that go beyond what is possible in the physical world. Virtual reality enables people with physical and intellectual disabilities to engage in active leisure activities, such as horseback riding and swimming, which are typically inaccessible to them in the physical world \cite{yalon_leisure}. Yalon-Chamovitz and Weiss \cite{yalon_leisure} found that disabled people react favorably to VR leisure activities due to their greater sense of autonomy over their bodies and environments. Virtual reality can also be leveraged to help people with invisible disabilities. For instance, in VR, neurodivergent users have greater control over their environment, so they may remove themselves from overwhelming situations or adjust settings to reduce their sensory load \cite{boyd_leveling}. Given its increasing popularity and unique affordances, it is important to understand how people with invisible disabilities want to engage with this social sphere, especially through avatar representation.

\subsection{Traditional and Creative Avatar Expression}
Avatars enable users to develop a greater social presence in social VR. Langener et al. determined that avatar customization heightens the user’s sense of connection and ownership over their virtual body, thus intensifying SoE \cite{langener_embodiment}. Many social VR users choose to represent themselves as accurately as possible through their avatars \cite{freeman_maloney_perception_of_self}. However, avatars can also creatively express their users’ interests and identities, sometimes extending beyond what is possible in the physical world. A myriad of prior works have explored identity and avatar representation in social VR \cite{freeman_maloney_perception_of_self}, including diverse user groups such as racial minorities \cite{blackwell_harassment}, women \cite{sharvit_sexual_harass}, and LGBTQ users \cite{freeman_acting_out, freeman_rediscovering}. For example, Freeman et al. \cite{freeman_maloney_perception_of_self} interviewed 30 people to study their avatar perceptions and found that most of them strove to make their avatars as similar as possible to their non-virtual counterparts because they considered avatars an extension of themselves in virtual worlds. Another study explored the avatar choices of non-cisgender users and revealed that they changed their avatar’s gender expression frequently, through outfits and accessories, to indicate their flexible and gender-fluid identities \cite{freeman_rediscovering}.

Unfortunately, current avatar representation options are generally inadequate at capturing the diverse range of human appearances and identities. Marginalized and stigmatized groups are especially under-represented. For example, Ready Player Me, a popular avatar creation tool, presents gender as a binary, which neglects the diversity of gender identity and forces gender-nonconforming people to abide by societal standards \cite{readyplayerme}. Furthermore, the middle-aged female participants in Morris et al.’s study noted that most avatars they encountered skewed towards youthful appearances, and existing avatar customization made them feel like a “caricature” of an older person \cite{Morris_2023_hide}.

Social VR also facilitates significant body modification. Users may opt for fantastical, cartoonish, and non-human features, such as the red eyes and snake eyes offered in Ready Player Me \cite{readyplayerme}. They can also choose non-human avatars \textemdash{} one participant in Freeman and Maloney’s study represented herself as a blue bird \cite{freeman_maloney_perception_of_self}. Furthermore, users can enable complete or partial invisibility of their avatars by manipulating the meshes that make up the 3D model \cite{youtube_invisibility_toolbox, youtube_invisibility_PxINKY}. Through these affordances, users can communicate their uniqueness, explore life as their avatar, and hold greater control over how others perceive them.  

Avatar representation of disability is particularly understudied, with some recent exceptions. Zhang et al. \cite{zhang_partofme} found users disclosed disabilities by attaching assistive technology to their avatars (e.g., hearing aids) and adopted a spectrum of disclosure strategies to represent themselves in social VR. Additionally, Davis and Chansiri found that online users with disabilities customized their avatars to foster a greater sense of empowerment and embodiment \cite{davis_digital_identities}. For instance, one user depicted herself as younger because she felt that her disability removed years from her life. Mack et al. \cite{mack_towards} shed light on some challenges facing individuals with intersectional identities as they represented themselves in digital platforms, noting they often had to choose between using avatars to represent their disability or race-related identities.

Our study includes social VR users with all types of invisible disabilities, distinct from Zhang et al.’s study \cite{zhang_partofme} focused on people with visible disabilities who use assistive technology. Given that many participants with visible disabilities were interested in translating their non-virtual assistive technology into their virtual avatars, little is known about the preferences of invisibly disabled people for embodied representations. Our study investigates invisible disabilities that often do not require assistive technology, which shifts the focus to exploring social VR affordances that are not necessarily available in non-virtual spaces. In addition, we build on Mack et al.’s study \cite{mack_towards} of digital avatars. Though their work included participants with invisible disabilities and found they wanted to use symbolic representations of disability that would resonate with their more specific community (e.g., chronic illness, ADHD), we extend our inquiry to study invisible disability representation preferences into virtual, embodied contexts. In this study, we examine how users want to employ VR’s multimodal affordances for disability expression in spaces where avatars mediate all social interaction. 

\section{Methodology}
We conducted semi-structured interviews with 15 participants who self-identified as having one or more invisible disabilities. We hoped to understand their perspectives on disability representation and visual disclosure in both non-virtual and social VR settings.

\subsection{Recruitment}
We recruited participants by emailing disability-related organization mailing lists, posting messages in relevant subreddits, and partnering with our university’s undergraduate extra credit system. Our inclusion criteria were as follows: participants must (1) be at least 18 years old, (2) have an invisible disability, and (3) have experience using social VR platforms. 

Our recruitment materials stated: “We define having invisible disabilities as including physical and psychological conditions that often have no visible manifestation, such as attention deficit, autism, and chronic health issues. We define social VR as a virtual platform where people communicate and interact with others in the form of avatars. Some popular social VR platforms include Rec Room, VRChat, vTime XR, and AltspaceVR.” We released these recruitment materials before AltspaceVR was shut down. 

\subsection{Participants}
This study consisted of \DIFdelbegin \DIFdel{15 }\DIFdelend \DIFaddbegin \DIFadd{14 }\DIFaddend participants aged 20 to 56 years old (\DIFdelbegin \DIFdel{$mean = 32.47, SD = 10.11$}\DIFdelend \DIFaddbegin \DIFadd{$mean = 33.14, SD = 10.13$}\DIFaddend ). Seven identified as female and \DIFdelbegin \DIFdel{eight }\DIFdelend \DIFaddbegin \DIFadd{seven }\DIFaddend identified as male. Regarding race, seven participants identified as White, \DIFdelbegin \DIFdel{four as Black }\DIFdelend \DIFaddbegin \DIFadd{three as Black or African American}\DIFaddend , two as mixed-race, one as Asian, and one as Alaskan Native. All participants disclosed that they had at least one invisible disability, such as dyslexia, chronic pain, ADHD, and autism. Two participants did not disclose their specific disabilities but shared the general type of disability (e.g., chronic condition, learning disability). In total, \DIFdelbegin \DIFdel{23 }\DIFdelend \DIFaddbegin \DIFadd{22 }\DIFaddend unique invisible disabilities were represented in this sample. All participants had experience with at least one social VR platform, but many had used multiple (e.g., VRChat, AltspaceVR, Spatial, Rec Room). Most used VR on a daily or weekly basis. We present a detailed demographic breakdown in Table \ref{table:participants}. Participants were compensated with a \$20 \DIFdelbegin \DIFdel{Amazon }\DIFdelend \DIFaddbegin \DIFadd{digital }\DIFaddend gift card upon completion of the interview. This study and all procedures were approved by our university’s Institutional Review Board (IRB), and all participants completed informed consent.

\subsection{Procedure}
We conducted semi-structured interviews via video conferencing software (Zoom). As part of the interview, we engaged participants in a creative activity on a collaborative whiteboard application (Google Jamboard), which allowed participants to draw and paint in multiple colors, import or link images from a device or online, type thoughts and ideas on sticky notes, and create text boxes and shapes. Participants could also use a virtual laser pointer to emphasize different aspects of the whiteboard while describing features of their creative expression if they so chose. All interviews were conducted in English, lasted approximately 60 minutes, and were video and audio recorded with the participants’ consent. We provide our full interview protocol in Supplementary Materials.

Each interview began with an introduction to the research and a review of the consent form prior to obtaining oral consent. We began the interview portion by asking participants about their uses for social VR and existing avatar representations in social VR, followed by questions that probed their current use of avatars as vessels for disclosure (or not). For example, we asked: “Do you represent or conceal your invisible disability in social VR in any way? How similar is your avatar representation to your physical self?” After establishing the similarities and differences between participants’ virtual and non-virtual selves, we asked if participants were interested in representing their invisible disability / disabilities in social VR. Regardless of their responses, we followed up by discussing how context might impact their decisions to represent (or not represent) their invisible disabilities. We wrapped up the first section by broadly exploring participants’ granular customization preferences.

The second section encouraged idea generation through creative brainstorming. We invited participants to share ideas for their “ideal avatar representation” in social VR by using the virtual whiteboard to express their ideas through images, drawing, or text.  After completing their visualizations and describing the thought processes behind them, participants were asked to describe any important features that were not currently available as well as their ideal customization process.

In the third section, we further explored the importance of context in virtual and non-virtual disclosure. We asked questions such as, “In the physical world, how do you navigate disability disclosure? Would you consider your avatar representation to be the same or different in different settings? How does this compare to other platforms with avatar options, such as Snapchat?” Finally, we discussed the practical implications of incorporating invisible disability representation features into avatar libraries. 

\subsection{Analysis}
Our data consisted of approximately 15 hours of recordings and detailed notes collected during the interviews. We transcribed all recordings and then used open coding to analyze the interviews. Three researchers divided the first three transcripts so that each was double-coded, discussed code discrepancies, created the preliminary codebook, and then split up the remaining transcripts for individual coding. Throughout the coding process, we iterated and refined the codebook over the course of approximately five meetings. 

After coding, we conducted thematic analysis \cite{braun2012thematic} to identify overarching thematic takeaways and patterns across participants. Our themes were grounded in the interview codes as well as the suggestions presented by participants during the whiteboard component, which included image and drawing artifacts. Per Clarke and Braun’s thematic analysis guide \cite{clarke2013thematic}, three team members generated lists of potential themes and bulleted outlines of the connections between them as preparation for a thematic analysis meeting. Then, we reflected on the proposed themes’ connections to our research questions, compared areas of overlap and divergence, and reflexively confronted any potential analytical assumptions. Finally, the three coders selected the themes that overlapped between their lists, and consulted with other team members to ensure themes engaged substantively with interpretative contributions, tweaking the thematic headings until they arrived at their final version. 

\subsection{Positionality}
One of the first authors lives with an invisible disability and has a background in feminist disability studies. The research team also includes social VR users, accessibility researchers, and people who have grappled with the complex issue of disability disclosure in their own lives. We believe avatar customization reform is an important step toward maximizing the inclusiveness of social VR spaces and aim to include the voices of VR users with invisible disabilities into the important conversations surrounding fostering positive representation and cultivating diverse spaces. 


\begin{table*}[h!]
    \footnotesize 
    \centering
    \caption{Participants’ demographics.} 
    \begin{tabular}{p{0.3cm}p{0.9cm}p{1.5cm}p{2.8cm}p{3.8cm}p{2.8cm}}
    \toprule
      \textbf{ID}&  \textbf{Age/ Gender}&  \textbf{Race}&  \textbf{Disabilities}&  \textbf{Social VR Use}&   \textbf{Frequency} \\
     \midrule 

   \textbf{P1}&   32/F&   White&  Low vision&  Altspace VR; Spatial&  several times/week \\ 
    \midrule

    \textbf{P2}&   32/F&   White& Bipolar disorder; PTSD&  synth Riders; VR fishing; VRChat; Walk about Mini Golf; & daily\\ 
    \midrule

     \textbf{P3} & 56/F & Mixed-race&  Dyslexia; rheumatoid arthritis; congestive heart failure& Altspace VR; VR fishing; VR Chat; Spatial; Big Screen; Wander& weekly\\ 
    \midrule

      \textbf{P4}&    38/F&    White &  Dyslexia; epilepsy; chronic pain&  the limps, Les Mills, body cam, FedEx, Sabre, the mini golf&   two to four or five times a week\\ 
    \midrule

      \textbf{P5}&    31/M&    White&   RSI; ADHD; Asperger’s& two to four or five times a week&  social: monthly
VR in general: weekly\\ 
    \midrule

    \textbf{P6}&    24/F&    Black &   POTS& vTime XR; Altspace VR; miscellaneous; Rec Room; Ping-pong& weekly\\ 
    \midrule

      \textbf{P7}&    33/F&    White&   Depression& VR Chat&  daily\\ 
    \midrule

      \textbf{P8}&    20/M&   Asian&   Chronic condition (diagnosis undisclosed)& VR Chat& one to two times a month\\ 
    \midrule

      \textbf{P9}&    28/M&   White, Asian&   Autism (nonverbal); learning impairment with linguistics (text); bipolar type one&  VR Chat&  "extensive"; 5000-6000 hours\\ 
    \midrule

      \textbf{P10}&    52/F&  White&  Hashimoto’s disease; contextual social anxiety; osteoporosis&  VR Chat, Synth Riders& "live on there" - work, sleep, "addiction"\\ 
    \midrule

      \textbf{P11}&    28/M&  Black& ADHD (undiagnosed)&  Altspace VR; Spatial; Rec Room; Horizon Worlds& multiple times a month\\ 
      \midrule

      \textbf{P12}&    31/M&  White&  Asperger’s; ADHD& Altspace VR; Oculus; Rec Room; Facebook Horizon& game and therapeutic tool since 2019 \\ 

     \bottomrule
    \end{tabular}
    \label{table:participants}
\end{table*}



\section{Findings}
\DIFdelbegin \DIFdel{We discovered themes surrounding social VR’s reflection of (and divergence from) }\DIFdelend \DIFaddbegin \DIFadd{Social virtual reality spaces often reflect many of the norms and utilities of non-virtual social spaces. Participants shared more about their social VR uses and experiences, and how they were similar or even equivalent to their }\DIFaddend non-virtual social \DIFdelbegin \DIFdel{environments (4.1), VR avatars’ potential for multimodal self-expression (4.2}\DIFdelend \DIFaddbegin \DIFadd{interactions. 
}

\DIFadd{Participants used social VR for a variety of purposes, including entertainment (e.g., playing games), conversational (e.g., chatting with others}\DIFaddend ), and \DIFdelbegin \DIFdel{distinctions between public and private disability representations (4.3), as described below. We have also compiled suggestions participants had for increasing the accessibility of customization mechanisms (4.4)and summarized them alongside suggestions derived from the three themes (see Discussion) 
}\DIFdelend \DIFaddbegin \DIFadd{professional (e.g., for work). For example, P1 described attending support groups, celebrating birthdays, and watching movies in social VR, and P2 felt that }\textit{\DIFadd{“}[\DIFadd{engaging}] \DIFadd{with others while they’re doing something active in the same way you are is very similar to if I was gonna go fishing with somebody in real life. It’s the same, like being able to join a chat party with some of my friends and go fishing with them together in VR.”}} \DIFadd{Additionally, for some participants, virtual platforms provided them essential access to environments when their invisible disabilities prevented them from leaving home. 
}

\begin{quote}
\DIFadd{“What I’m getting out of VR is a little different than what most people get out of VR. They get in there, and they want to }[\DIFadd{play games}]\DIFadd{. I’m there so that the world doesn’t close in on me… to keep a tiny little porthole of the world open to me. Even though I cannot physically be in it, I can virtually be in it. I can visit a museum through VR. I went up }[\DIFadd{to}] \DIFadd{the space station through VR. I’ve gone scuba diving in VR. And the social aspects \textemdash{} I’ve met friends who have been my friends for years, but we live in different states. And we’ve come together.” (P7, 33F) 
}\end{quote}

\DIFadd{In this section, we present participants’ perceptions on the unique affordances of embodied VR avatars, detail current and imagined invisible disability representations for social VR avatars, and explore disclosure preferences across different social VR contexts}\DIFaddend .
\subsection{Embodied VR Avatars are Dynamic, Contextual, and Multimodal}
\DIFdelbegin %DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdelend Participants identified key differences in their perceptions of non-embodied and embodied avatars. In general, they viewed non-embodied avatars, such as Facebook profile pictures, Facebook avatars, and Snapchat Bitmojis, as a single snapshot of their identity. On the other hand, participants found embodied VR avatars to be more dynamic and authentic representations of themselves. Additionally, one key affordance of VR avatars is that they allow for multimodal self-expression, which greatly influenced participants’ current and imagined preferences for disability representations on social VR platforms. 

\subsubsection{Differences Between Embodied and Non-Embodied Avatars}
Though participants had experience using non-embodied avatars to represent themselves, they felt as though the static nature made it difficult for them to convey their true, current identity. For example, \DIFdelbegin \DIFdel{P14 referred to his Facebook profile picture as }\textit{\DIFdel{“just a representation, it’s not real,”}} %DIFAUXCMD
\DIFdel{whereas }\DIFdelend P1 said that her Facebook avatar \textit{“doesn’t look like me at all. I hate it.”} P3 also shared how her experiences with using Facebook and social VR for different purposes, and for different audiences, influenced her degree of comfort with representing herself in embodied and non-embodied contexts.

\begin{quote}
“With Facebook, of course my avatar is a photo of me. But it’s a photo of me 20 years ago. So my avatar doesn’t age there… and I have not changed it to be what I am now. Because the people that are on my Facebook, many of them are people that know me in this physical reality. They know what I look like. I don’t have to make it a picture from yesterday. But it’s also something that I’m not gonna change, you know. I cannot pretend in Facebook that I’m well or not well… I don’t represent a cause, I don’t represent a disease, I don’t represent anything by myself. … Whereas in VR, I do change those things. It doesn’t mean that I’m two-faced, or anything like that. … Virtual reality, there are people there that know and love me, but most people are acquaintances or strangers. So my interaction with them is going to be different [from] my interaction on Facebook.” (P3, 56F)
\end{quote}

\DIFaddbegin \DIFadd{Others also expressed that the embodied nature of social VR avatars encouraged them to be more authentic. P14 mentioned that the }\textit{\DIFadd{“immersive experience }[\DIFadd{of being}] \DIFadd{around a lot of people, seeing the avatar move around”}} \DIFadd{made him wish to represent himself in greater detail on a social VR avatar as opposed to a static avatar on Facebook. 
}

\DIFaddend Referring to the overall experience of using mainstream social media networks, P13 also mentioned that he actively chose to not engage with these platforms to avoid \textit{“engagement loops that keep you coming back to it… they’ll track you with their pixel tracker on other websites and start sending you advertisements.”} In contrast to text-only communication on social media, he found the different communication modes in social VR to be easier to process: \textit{“you can take in text easier… it’s basically reading text messages versus voice chat, digital avatar, [or] motion capture”} (P13). Additionally, he mentioned that the discomfort and fatigue associated with VR headsets was helpful for preventing him from spending excessively long on these platforms. 

When discussing the distinctions between social media and social VR, P9 summarized how his interactions differed between the two environments and emphasized that the immersive affordances of social VR avatars enabled him to not only better express himself, but understand others as well.

\begin{quote}
\textit{“I’d say [VR] is an order of magnitude above anything that you would see on Instagram \textemdash{} anything that you see on any other website \textemdash{} because those are just two-dimensional static images or videos. [You] can’t interact with photos, but when you’re there in virtual reality, you can see all the details on the avatar showing that this person is expressing themselves. [You can] see their facial expressions, their movements, and their body language. And it’s real time. No other kind of social platform comes even close to VR.”} (P9, 28M) 
\end{quote}

\subsubsection{Multimodal Affordances Can Represent Physical Human Expression}
Participants also discussed the multimodal expressiveness of embodied avatars, which manifested primarily through avatar visuals, voices, movements, body language, and facial expressions. For example, participants described more of the physicality of communicating in social VR spaces. P9 discussed the value of facial expressions: 

\begin{quote}
“I am quite expressive myself, but my invisible disability is nonverbal autism, so I wouldn’t actually say what I’m feeling. I would express it through my avatar’s facial expressions. Sometimes, the number of expressions on an avatar goes as high as 30 or 40 different options. So having many different options to express myself nonverbally is a way that I can get more synchronized and comfortable using an avatar.” (P9, 28M) 
\end{quote}

While P2 had not used the facial expression features of newer VR headsets, as someone with bipolar disorder, she was interested in using body language to represent changes in her mood. 

\begin{quote} 
“Let’s say I’m feeling excited or hyper. Your avatar can have a really upbeat energy to it if you’re going to apply an energy to an avatar. Or if you can put in there that you’re feeling slightly depressed, or that you have a low mood or that you’re tired, your avatar would be a little bit lower on the energy… That way my friends could see me and then go like, ‘Oh, that’s kind of the mood she’s in. Let’s cheer her up.’ Or, ‘Let’s just give her her space.’ And they see you come in in this perky mood, and then they can kind of match their energy to your mood without you having to be so vocal about it.” (P2, 32F) 
\end{quote}

Some participants focused on how the embodied movement of VR avatars could represent or support their disability identities. For example, P12 wanted to utilize either voice or movement: \textit{“if I am going to disclose my disability on the platform, it would be verbally or through using the VR controllers when I’m controlling the hands of the avatar.”} Conversely, though his experiences with arthritis sometimes impacted his mobility in the non-virtual world, P14 did not want to disclose his disability through this modality \DIFdelbegin \DIFdel{; }\DIFdelend \DIFaddbegin \DIFadd{\textemdash{} }\DIFaddend he preferred for his avatar to move in the same ways as others. \DIFdelbegin \DIFdel{Additionally, when speaking about her experiences in a disability support group in VR}\DIFdelend \DIFaddbegin \DIFadd{Regarding support of the disabled experience}\DIFaddend , P3 described how \DIFdelbegin \DIFdel{VR avatar movements }\DIFdelend \DIFaddbegin \DIFadd{embodied VR avatar interactions }\DIFaddend could facilitate community \DIFdelbegin \DIFdel{support with a physicality unique to embodied contexts}\DIFdelend \DIFaddbegin \DIFadd{empowerment and connection in a disability support group}\DIFaddend : \textit{“sometimes, our avatars will run over and give somebody a group avatar hug when they’re having a particularly bad time.”} P4 shared an anecdote about the inconvenience of embodying a cat and having your avatar’s eye line to the ground when engaging with human-sized avatars. 

Other extended reality technologies, such as augmented or mixed reality, were also of interest. P10 wanted to use her embodied social VR avatar in her content creation process to merge her representations in virtual and non-virtual domains:

\begin{quote}
“I just wish they had a lot more options for stuff. I’m hoping they grow in that area [mixed reality] when they come out with the next [headset], because I heard through the grapevine it’s supposed to be more for mixed reality. I would actually love using an avatar instead of my real body in my YouTube videos.” (P10, F, 52 years old) 
\end{quote}

\subsection{Current and Imagined Invisible Disability Representations}
\DIFdelbegin %DIFDELCMD < 

%DIFDELCMD < %%%
\subsubsection{\DIFdel{Current Uses of Social VR}}
%DIFAUXCMD
\addtocounter{subsubsection}{-1}%DIFAUXCMD
\DIFdel{Social virtual reality spaces often reflect many of the norms and utilities of non-virtual social spaces. Participants shared more about their social VR uses and experiences, and how they were similar or even equivalent to their non-virtual social interactions. For example, P1 described attending support groups, celebrating birthdays, and watching movies in social VR , and P2 felt that }\DIFdelend \DIFaddbegin \DIFadd{Throughout the interviews, participants shared the ways they currently represented or disclosed their invisible disability and brainstormed ways to improve avatar systems to make them more inclusive. Generally, social VR offers users unique affordances that shape avatar customization and self-expression. P11 described his avatar to be }\DIFaddend \textit{“\DIFaddbegin \DIFadd{an exaggeration of }\DIFaddend [\DIFdelbegin \DIFdel{engaging}\DIFdelend \DIFaddbegin \DIFadd{his}\DIFaddend ] \DIFdelbegin \DIFdel{with others while they’re doing something active in the same way you are is very similar }\DIFdelend \DIFaddbegin \DIFadd{physical identity \textemdash{} anonymous, but also close enough }\DIFaddend to \DIFaddbegin \DIFadd{be recognized }\DIFaddend if \DIFdelbegin \DIFdel{I was gonna go fishing with somebody in real life}\DIFdelend \DIFaddbegin \DIFadd{you know }[\DIFadd{him}] \DIFadd{personally}\DIFaddend .\DIFdelbegin \DIFdel{It’s the same, like being able to join a chat party with some of my friends and go fishing with them together in VR.}\DIFdelend ”} \DIFaddbegin \DIFadd{P12 had a similar description: }\textit{\DIFadd{“I try to represent myself as I am, of course, and for me, that involves maybe making an avatar that looks like me but is a little bit cooler if possible.”}}
\DIFaddend 

\DIFdelbegin \DIFdel{However, participants’ }\DIFdelend \DIFaddbegin \DIFadd{We found that }\DIFaddend desired methods of representing \DIFdelbegin \DIFdel{their disability }\DIFdelend \DIFaddbegin \DIFadd{invisible disabilities }\DIFaddend in social VR did not always align with \DIFdelbegin \DIFdel{their }\DIFdelend non-virtual disclosure practices. \DIFdelbegin %DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{VR affords such a breadth of social experiences that it can facilitate much of users’ daily social interactions. P7 shared, }\textit{\DIFdel{“VR is an interesting experience. Kinda really the majority of the socialization I do these days.”}} %DIFAUXCMD
\DIFdel{This transferral of social outlets from the non-virtual to the virtual world can occur for any number of reasons, but for some participants, virtual platforms provide essential access to environments when their invisible disabilities prevent them from leaving home. P7 shared: 
}%DIFDELCMD < 

%DIFDELCMD < \begin{quote}
%DIFDELCMD < %%%
\DIFdel{“What I’m getting out of VR is a little different than what most people get out of VR. They get in there, and they want to }%DIFDELCMD < [%%%
\DIFdel{play games}%DIFDELCMD < ]%%%
\DIFdel{. I’m there so that the world doesn’t close in on me. I’m there to keep a tiny little porthole of the world open to me. Even though I cannot physically be in it, I can virtually be in it. You know, I can visit a museum through VR. I went up on the space station through VR. I’ve gone scuba diving in VR. And the social aspects. I’ve met friends who have been my friends for years, but we live in different states. And we’ve come together.” (P7, 33F) 
}%DIFDELCMD < \end{quote}
%DIFDELCMD < 

%DIFDELCMD < %%%
\subsubsection{\DIFdel{Public and Private Representations of Disability}}
%DIFAUXCMD
\addtocounter{subsubsection}{-1}%DIFAUXCMD
\DIFdelend Participants desired options for both public (\DIFdelbegin \DIFdel{or }\DIFdelend \DIFaddbegin \DIFadd{i.e., }\DIFaddend explicit) and private (\DIFdelbegin \DIFdel{or }\DIFdelend \DIFaddbegin \DIFadd{i.e., }\DIFaddend implicit) identity expression. Suggestions \DIFdelbegin \DIFdel{included }\DIFdelend \DIFaddbegin \DIFadd{for both public and private representations encompassed }\DIFaddend clothing, accessories, icons, energy bars, or modifications to avatar bodies\DIFdelbegin \DIFdel{such as a tail, and some suggestion categories included both public and private meanings}\DIFdelend .

\DIFdelbegin \DIFdel{To start, }\DIFdelend \DIFaddbegin \subsubsection{\DIFadd{Public Representations and Expressions of Disability}}
\DIFadd{Some participants were interested in representing their disability identities in public and explicit ways, meaning that other social VR users could identify their specific disability or their symptoms from their avatar. 
}

\DIFadd{Ten }\DIFaddend participants suggested incorporating customizable clothing\DIFdelbegin \DIFdel{and patterns}\DIFdelend \DIFaddbegin \DIFadd{, patterns, or accessories }\DIFaddend that featured disability-related logos. \DIFaddbegin \DIFadd{These suggestions often supported participants’ goals of expressing their personal style and advocating or educating about their disability. }\DIFaddend For example, P1 wanted to have an avatar wearing a zebra-printed shirt and beret to advocate for Rare Disease Month. Similarly, \DIFdelbegin \DIFdel{P4 suggested }\DIFdelend \DIFaddbegin \DIFadd{P12 wished to express his personal style and disability status through a }\textit{\DIFadd{“little cool jacket }[\DIFadd{with}] \DIFadd{a label…to say my name and that I have Asperger’s and whatnot.”}} \DIFadd{Others suggested having accessories specific to their disability (e.g., a brooch saying “POTS” as suggested by P6, or a PTSD ribbon as suggested by P13). P4 wished to have }\DIFaddend an explicit representation for communicating the experience of dyslexia through apparel\DIFdelbegin \DIFdel{or logos}\DIFdelend : 

\begin{quote}
\DIFdelbegin \textit{\DIFdel{“}%DIFDELCMD < [%%%
\DIFdel{On clothing,}%DIFDELCMD < ] %%%
\DIFdel{have the word dyslexia, but then have it jumbled up so people can see what it looks like when we try to read. Then, they’ll be like, `Whoa, that’s not fun.’ And we’re like, `Well, welcome to my hell.’ Make it a joke, but also kind of be like, `Hey, this is really what it feels like.’ }} %DIFAUXCMD
\DIFdelend \DIFaddbegin \DIFadd{“}[\DIFadd{On clothing,}] \DIFadd{have the word dyslexia, but then have it jumbled up so people can see what it looks like when we try to read. Then, they’ll be like, ‘Whoa, that’s not fun.’ And we’re like, ‘Well, welcome to my hell.’ Make it a joke, but also kind of be like, ‘Hey, this is really what it feels like.’” }\DIFaddend (\DIFdelbegin \DIFdel{P4,F, 38 years old)
}\DIFdelend \DIFaddbegin \DIFadd{P4, 38F)
}\DIFaddend \end{quote}

\DIFdelbegin \DIFdel{Just as P4’s suggestion combined personality and humor to inspire avatar-based education and disability advocacy efforts, P12 wished to express his personal style and disability status through a }\textit{\DIFdel{“little cool jacket }%DIFDELCMD < [%%%
\DIFdel{with}%DIFDELCMD < ] %%%
\DIFdel{a label…to say my name and that I have Asperger’s and whatnot.”}}
%DIFAUXCMD
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdelend Other participants wanted customization libraries to include assistive technology (e.g., wheelchairs, canes, crutches, hearing aids), \DIFdelbegin \DIFdel{an assortment of chronic-illness specific items (e.g., a brooch that says }\textit{\DIFdel{“POTS”}}%DIFAUXCMD
\DIFdel{, P6), a }\DIFdelend \DIFaddbegin \DIFadd{a }\DIFaddend medical alert bracelet, and \textit{“spoonie”} gear \DIFdelbegin \DIFdel{like }\DIFdelend \DIFaddbegin \DIFadd{(e.g., }\DIFaddend a giant spoon, \DIFaddbegin \DIFadd{as suggested by }\DIFaddend P1) to disclose their disabilities. 

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{imgs/P1.png}
    \caption{Participant 1’s drawings and suggestions for invisible disability representation during the whiteboard component of the study, featuring a giant spoon to represent spoon theory and other assistive technologies to disclose their disability.} 
    \Description{Participant 1’s drawings and suggestions for invisible disability representation during the whiteboard component of the study. At the far left, there is a floating medication reminder inside a speech bubble that represents a floating emote. Below are examples of assistive technology such as a cane and hearing aids. Next is a person’s outline wearing a zebra print beret and shirt to represent rare disease month. The shirt also has a space for a custom disability graphic or a fact about the participant’s rare disease, both aimed at spreading invisible disability awareness. The person also wears a medical alert bracelet and carries a human-sized spoon to represent desired “spoonie” props that point to identification with spoon theory. Finally, there is a note where there would be a floating menu to enable and disable disability-related accessories.}
    \label{P1}
\end{figure*}

\DIFaddbegin \DIFadd{Icons and graphics around an avatar could also help with representing someone’s disability in a more subtle, but still public, way. Four participants were interested in disability representations that floated above their avatars, such as an awareness flag or a dynamic energy bar that correlated with their energy level or “social battery”. For example, P2 proposed }\textit{\DIFadd{“an energy bar, like in a video game where you have your life meter. If it’s full, you’re full of energy, and it’s all the way green… And if I’m really low on energy, I’ve got a red bar.”}} \DIFadd{Recognizable icons, such as the rainbow infinity symbol to represent neurodiversity, were also valued; however, participants specifically criticized harmful iconography, such as the light blue puzzle piece representing the Autism Speaks organization. Additionally, }\DIFaddend P11, a designer by trade, \DIFdelbegin \DIFdel{drew on his experience with video games to suggest ways to represent his disability through icons: 
}%DIFDELCMD < 

%DIFDELCMD < \begin{quote} 
%DIFDELCMD <     %%%
\textit{\DIFdel{“It’s probably influenced by video games and Internet culture…where there’s so much going on the screen in front of you, and you can’t really remember what every icon means. … So “I” is Information…You click that…and the general notice is also a symbol…because of the sensitivity of the types of people involved. This universal image for neurodiversity.”.”}} %DIFAUXCMD
\DIFdel{(P11, M, 28 years old)
}%DIFDELCMD < \end{quote} 
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{Notably, P11 }\DIFdelend \DIFaddbegin \DIFadd{proposed a specific idea for disclosing his disability through design patterns and iconography. Notably, he }\DIFaddend described the importance of the transient nature of this representation \DIFdelbegin \DIFdel{in facilitating social interactions:
}\DIFdelend \DIFaddbegin \DIFadd{so as not to greatly disrupt social interactions.
}\DIFaddend 

\begin{quote} 
\DIFdelbegin \textit{\DIFdel{“I would imagine that when the user clicks }%DIFDELCMD < [%%%
\DIFdel{the "I"}%DIFDELCMD < ] %%%
\DIFdel{the image pops up for only a few moments in time, right?...That way, you can continue your interactions and virtual space without necessarily having the label on you constantly.”}} %DIFAUXCMD
\DIFdelend \DIFaddbegin \DIFadd{“}[\DIFadd{This idea is}] \DIFadd{probably influenced by video games and internet culture… where there’s so much going on the screen in front of you, and you can’t really remember what every icon means. … So “i” is Information… You click that… }[\DIFadd{and it pops up}] \DIFadd{this universal image for neurodiversity. … I would imagine that when the user clicks }[\DIFadd{the “i”}]\DIFadd{, the image pops up for only a few moments… That way, you can continue your interactions and virtual space without necessarily having the label on you constantly.” }\DIFaddend (P11, \DIFdelbegin \DIFdel{M, 28 years old}\DIFdelend \DIFaddbegin \DIFadd{28M}\DIFaddend )
\end{quote} 

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{imgs/P11.png}
    \caption{Participant 11’s images, sticky notes, and suggestions for invisible disability representation during the whiteboard component of the study, featuring an information icon and the ADHD rainbow butterfly symbol above the avatar.} 
    \Description{Participant 11’s images, sticky notes, and suggestions for invisible disability representation during the whiteboard component of the study. There is an image of Toad, an anthropomorphized mushroom character from the Mario franchise, wearing an astronaut suit and helmet. On his cap, there is an information icon (a lowercase i in a circle) and above Toad is the ADHD rainbow butterfly symbol. To Toad’s right, there is a sticky note that reads, “General notice of invisible disability - other users can click to reveal more information. More information is presented as a specific symbol represen-”. To the right of the ADHD symbol, there is a sticky note reading “Symbol is animated and hovers on top the avatar for a few seconds after the (i) button is clicked.”}
    \label{P11}
\end{figure*}

\DIFdelbegin \DIFdel{Some participants (P2, P6) were interested in disability representations that floated above their avatars, such as an awareness flag or a dynamic energy bar that correlated with their energy level or “social battery. ” As an accommodation feature, this interfaces interestingly with P11}\DIFdelend \DIFaddbegin \DIFadd{Disability representations also included temporary adjustments to the avatar to indicate a user}\DIFaddend ’\DIFdelbegin \DIFdel{s proposal of }\DIFdelend \DIFaddbegin \DIFadd{s interest in engaging with others. Similar to the energy bar example, P11 proposed }\DIFaddend a feature that would allow an avatar to turn invisible when \DIFdelbegin \DIFdel{its user wants }\DIFdelend \DIFaddbegin \DIFadd{a user wanted }\DIFaddend to avoid social interactions\DIFdelbegin \DIFdel{. Turning invisible would convey nonverbally that a person does not want to be approached.
}%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdelend \DIFaddbegin \DIFadd{, which he dubbed as a }\textit{\DIFadd{“stealth mode.”}} \DIFaddend However, P11 \DIFdelbegin \DIFdel{quickly engaged critically with the potential }\DIFdelend \DIFaddbegin \DIFadd{assessed the potential privacy }\DIFaddend implications of implementing such a feature\DIFdelbegin \DIFdel{: 
}\DIFdelend \DIFaddbegin \DIFadd{, and concluded that turning an avatar translucent could convey a similar message of wishing to keep to themself while still alerting other users to the fact that there was another user within the space.
}\DIFaddend 

\begin{quote} 
\DIFdelbegin \textit{\DIFdel{“If you think about the other users of the space, do you really want an invisible person watching you? Because you can see them. … I guess if you are engaging in this space, you sort of have to descend. Maybe rather than being invisible, you can have a great observation of your avatar. So my }%DIFDELCMD < [%%%
\DIFdel{avatar}%DIFDELCMD < ]%%%
\DIFdel{, who’s red and blue, right? I can just make him more white }%DIFDELCMD < [%%%
\DIFdel{translucent}%DIFDELCMD < ] %%%
\DIFdel{instead, so he’s like one of them. ‘Just don’t come to me. }%DIFDELCMD < [%%%
\DIFdel{He’s}%DIFDELCMD < ] %%%
\DIFdel{not really colorful right now.’”}} %DIFAUXCMD
\DIFdelend \DIFaddbegin \DIFadd{“If I’m in }[\DIFadd{a}] \DIFadd{VR space and I just want to enjoy myself, and I don’t want anyone coming up to me, I should be able to say that. … }[\DIFadd{but}] \DIFadd{if you think about the other users of the space, do you really want an invisible person watching you? … Maybe rather than being invisible… I can just make him more white }[\DIFadd{translucent}] \DIFadd{instead… ‘Just don’t come to me. }[\DIFadd{My avatar’s}] \DIFadd{not really colorful right now.’” }\DIFaddend (P11, \DIFdelbegin \DIFdel{M, 28 years old}\DIFdelend \DIFaddbegin \DIFadd{28M}\DIFaddend ) 
\end{quote} 

\DIFdelbegin \DIFdel{This specific example speaks to the uniqueness of the embodied experience that social VR offers its users highlighting an affordance impossible in the physical world and offering humans an option to change colors like a chameleon, continuing the theme of avatars affording novel self-expression through non-humanoid embodiment. 
}\DIFdelend \DIFaddbegin \DIFadd{Participants’ public representations of their disability utilized unique affordances of the embodied avatar experience, such as wearing custom-designed clothes and accessories to advocate for invisible disabilities, having a visible “energy bar” to indicate mood and energy level, and changing colors to express one’s willingness to interact with others. 
}

\subsubsection{\DIFadd{Private Representations and Expressions of Disability}}
\DIFaddend Below, we describe how participants explored \DIFdelbegin \DIFdel{representations }\DIFdelend \DIFaddbegin \DIFadd{different expressions }\DIFaddend infused with personal meanings\DIFdelbegin \DIFdel{that are as invisible as their disabilities. 
}%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{For example, P8 gave his avatar earbuds during the creative exercise, explaining: }\textit{\DIFdel{“I’m not a big earbud guy, I’m a headphone wearer… }%DIFDELCMD < [%%%
\DIFdel{but}%DIFDELCMD < ] %%%
\DIFdel{I feel like maybe it would be an extension of you trying to conceal what invisible disabilities I would have, just pretending to be normal with stuff like that.”}} %DIFAUXCMD
\DIFdel{While this representation of his invisible disability was not explicit to others, he acknowledged that his avatar was }\textit{\DIFdel{“more of an expression of }%DIFDELCMD < [%%%
\DIFdel{him}%DIFDELCMD < ]%%%
\DIFdel{.”}} %DIFAUXCMD
\DIFdel{and preferred to keep this aspect abstract}\DIFdelend \DIFaddbegin \DIFadd{, such that they could still represent their invisible disability without necessarily disclosing a disability identity to other social VR users}\DIFaddend .

\DIFdelbegin \DIFdel{Similarly}\DIFdelend \DIFaddbegin \DIFadd{Participants primarily suggested representing their disability identities or experiences through accessories that matched those that they would wear in non-virtual settings. For example}\DIFaddend , P3 preferred more subtle accessories that would more closely resemble non-virtual affordances: \textit{“I would do it with accessories, [but] I don’t want a big sign saying, \DIFdelbegin \DIFdel{`}\DIFdelend \DIFaddbegin \DIFadd{‘}\DIFaddend disabled’ or a different color flashing over here that says \DIFdelbegin \DIFdel{`}\DIFdelend \DIFaddbegin \DIFadd{‘}\DIFaddend invisible illness is no longer invisible.’\DIFdelbegin \DIFdel{But I would do it with subtle accessories. Something a little more real.}\DIFdelend ”} \DIFdelbegin %DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{Speaking of “real” accessories, or those rooted in non-virtual environments, }\DIFdelend P12 \DIFaddbegin \DIFadd{also }\DIFaddend wanted to use clothing or accessories that blurred private and public significance: 

\begin{quote}
\DIFdelbegin \textit{\DIFdel{“For me, I utilized my interest in cars as both something to therapeutically do but also maybe relate to others that have that same interest. Which is why I also, in real life, like to collect diecast cars and books on cars and, sometimes, I also like to wear clothing with cars on it. This is more of a social preference. I don’t know how that would represent my disability entirely, but if }%DIFDELCMD < [%%%
\DIFdel{others}%DIFDELCMD < ] %%%
\DIFdel{at least understand my passions and interests and how knowledgeable I am about them, then maybe they have a better understanding of me, too. On a personal level, at least.”}} %DIFAUXCMD
\DIFdelend \DIFaddbegin \DIFadd{“For me, I utilized my interest in cars as both something to therapeutically do but also maybe relate to others that have that same interest. Which is why I also, in real life, like to collect diecast cars and books on cars and, sometimes, I also like to wear clothing with cars on it. This is more of a social preference. I don’t know how that would represent my disability entirely, but if }[\DIFadd{others}] \DIFadd{at least understand my passions and interests and how knowledgeable I am about them, then maybe they have a better understanding of me, too. On a personal level, at least.” }\DIFaddend (P12, \DIFdelbegin \DIFdel{M, 31 years old}\DIFdelend \DIFaddbegin \DIFadd{31M}\DIFaddend )
\end{quote} 

\DIFdelbegin \DIFdel{Two other participants (P5, }\DIFdelend \DIFaddbegin \DIFadd{Others used accessories that they didn’t wear in the physical world, but still carried meaning to the participant. During the creative exercise, P8 gave his avatar earbuds, explaining: }\textit{\DIFadd{“I’m not a big earbud guy, I’m a headphone wearer }[\DIFadd{in the physical world}]\DIFadd{… }[\DIFadd{but}] \DIFadd{I feel like maybe it would be an extension of you trying to conceal what invisible disabilities I would have, just pretending to be normal with stuff like that.”}} \DIFadd{While this representation of his invisible disability was not explicit to others, he acknowledged that the earbuds were }\textit{\DIFadd{“more of an expression of }[\DIFadd{him}]\DIFadd{”}} \DIFadd{and preferred to keep this aspect abstract. P14 also utilized headphones and a mask as symbolism for }\textit{\DIFadd{“blocking out all the noise”}} \DIFadd{in the environment. Similarly, }\DIFaddend P9 \DIFdelbegin \DIFdel{) were interested in representations of personal significance rather than using them to communicate with other users. For example, P9 used vibrant colors: }\textit{\DIFdel{“It’s a way that I can visually differentiate myself from a room full of other people. It’s my way of not just indicating to others that this person’s a little different, but it’s also indicating to myself that I’m a little different.”}}
%DIFAUXCMD
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{P9 also established his interest in using his social VR avatar to tell a complex and storied narrative through the deceptively commonplace selection of elbow and knee pads in }\DIFdelend \DIFaddbegin \DIFadd{also described how }\DIFaddend his ideal avatar representation \DIFdelbegin \DIFdel{: 
}\DIFdelend \DIFaddbegin \DIFadd{included elbow and knee pads: 
}

\DIFaddend \begin{quote}
\DIFdelbegin \textit{\DIFdel{“I really want to add knee and elbow pads. If you have ever gone roller skating, you need to put on knee and elbow pads, just in case you fall... The bipolar makes me swing really hard to the left and right. I get these mania phases and these depression phases that have a whiplash to them. And sometimes... I can get hurt or accidentally hurt others. So these pads on my knees and elbows would be a way to symbolize that if I do fall, I gotta make sure I’m protected. I don’t fall too hard, and I can stand up again.”}} %DIFAUXCMD
\DIFdelend \DIFaddbegin \DIFadd{“I really want to add knee and elbow pads. If you have ever gone roller skating, you need to put on knee and elbow pads, just in case you fall… The bipolar makes me swing really hard to the left and right. I get these mania phases and these depression phases that have a whiplash to them. And sometimes… I can get hurt or accidentally hurt others. So these pads on my knees and elbows would be a way to symbolize that if I do fall, I gotta make sure I’m protected. I don’t fall too hard, and I can stand up again.” }\DIFaddend (P9, 28M)
\end{quote}

\DIFdelbegin \DIFdel{Disability is one facet of a complex human experience that is filtered through intersecting lenses of other identities like gender and race. Participants identified connections between the experiences of people in distinct marginalized groups. P12 also compared disclosing invisible disabilities to disclosing sexuality and gender identity, citing LGBTQ award-winners at the Tony Awards as examples of ways that queer people expressed and disclosed their identity through clothing and other visual means. }%DIFDELCMD < 

%DIFDELCMD < \begin{figure*}[t]
%DIFDELCMD <     \centering
%DIFDELCMD <     \includegraphics[width=\linewidth]{imgs/P12.png}
%DIFDELCMD <     %%%
%DIFDELCMD < \caption{%
{%DIFAUXCMD
\DIFdelFL{Participant 12’s images, sticky notes, and suggestions for invisible disability representation during the whiteboard component of the study, featuring screenshots of two different avatars he uses. The images are blurred to preserve the participant’s anonymity.}} 
    %DIFAUXCMD
%DIFDELCMD < \Description{Participant 12’s images, sticky notes, and suggestions for invisible disability representation during the whiteboard component of the study. On the top there are four sticky notes, reading “Important notes for Autism and Aspergers with Avatars in VR: 1. Make sure facial expressions and non verbal expressions are accurate and can also include descriptions as needed.” / “For those who also may be LGBTQ or have a physical disability, have accurate representations of them.” / “Offer opportunity to have a community for those to share similar interests as a way of  improving socialization” / “Learn behavioural techniques in virtual environments and inhibit restrictions to help.” Below the sticky notes are three screenshots of P12’s avatar. On the left is a screenshot of his avatar’s head and torso with a box sketched to the right of his head. The avatar is 3D, light-skinned, has a beard, short hair, sunglasses, and a Unity sweatshirt. The middle screenshot shows a 2D avatar with glasses, a goatee, and wearing a blue shirt with a brown vest; the avatar’s hands are raised and it says “Happy New Year!” above his head. The screenshot on the right is a zoomed out version of the screenshot on the left, showing the 3D avatar’s whole body.}
%DIFDELCMD <     \label{P12}
%DIFDELCMD < \end{figure*}
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{On another note, }\DIFdelend \DIFaddbegin \DIFadd{Three participants were interested in alterations to their avatar itself, beyond accessories, that could indicate their difference from other users in an implicit way. For example, P9 used vibrant colors: }\textit{\DIFadd{“It’s a way that I can visually differentiate myself from a room full of other people. It’s my way of not just indicating to others that this person’s a little different, but it’s also indicating to myself that I’m a little different.”}} \DIFaddend P10 \DIFaddbegin \DIFadd{also }\DIFaddend expressed that her avatar\DIFaddbegin \DIFadd{’s large bushy tail }\DIFaddend represented her comfort zone and personal bubble\DIFdelbegin \DIFdel{, a current customization option she valued (and the only current yet implicit example of disability representation we found available on customization platforms at present): 
}%DIFDELCMD < 

%DIFDELCMD < \begin{quote} 
%DIFDELCMD <     %%%
\textit{\DIFdel{“Its tail wraps around it a lot as it’s moving, or if you stand still… but I like that one because, in some weird way, it gives me a comfort zone of hiding me in a bubble. I don’t know, I never found one that did that. So, when I came across that one, I just liked it. Even in real life, people have said I have a bubble, like a huge bubble around me. It’s like you get too close to me, and I’m kinda like… I just back away a little.”}} %DIFAUXCMD
\DIFdel{(P10, F, 52 years old)
}%DIFDELCMD < \end{quote}
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{P10 }\DIFdelend \DIFaddbegin \DIFadd{. She }\DIFaddend described using her humanoid and avatar-based self-expression as a metaphor for her non-virtual personality, further emphasizing the unique affordances of social VR in expanding the bounds of self-expression by allowing fantastical and metaphorical representations of the self. 

\DIFdelbegin \DIFdel{While }\DIFdelend \DIFaddbegin \begin{quote} 
\DIFadd{“Its tail wraps around it a lot as it’s moving, or if you stand still… but I like that one because, in some weird way, it gives me a comfort zone of hiding me in a bubble. … Even in real life, people have said I have a bubble, like a huge bubble around me. It’s like you get too close to me, and I’m kinda like… I just back away a little.” (P10, 52F)
}\end{quote}

\DIFadd{Though some participants brainstormed representations of disability were intended to be explicit, they realized that their ideas could still be implicit to other social VR users. For example, P9 emphasized how his embodied avatar reflected his mood, especially related to his experiences with Bipolar Type 1. He used VR avatar appearances to communicate his emotions nonverbally, strategically selecting avatars based on his goals for social interactions that day. He explained his use of colors and their social and psychological effects: 
}

\begin{quote}
\DIFadd{“The middle avatar is the avatar I use when I’m in a playful mood. It stands out, but it’s also really friendly looking. I got a lot of people that like to hang around with me in this one if I’m feeling energetic, a little bit extroverted. If we talk about bipolar phases a little bit more, like the manic phase, I’ll use the middle one. … If I’m in a really happy mood, but I pick an avatar with like no color, for few emotions, it wouldn’t really match. Same thing vice versa. It also adds some novelty to VR chat as well, because if I see myself in the same avatar for too long, I feel like I start to get fixed. I start to lock myself in the avatar. So, I like to mix it around, so I know there’s always flexibility to iterate and change.” (P9, 28M) 
}\end{quote}

\DIFadd{Similarly, while }\DIFaddend P5 wished to use glowing veins to represent chronic pain, he acknowledged that other users might not understand the disability-related symbolism: \textit{“\DIFdelbegin \DIFdel{That would show things more, but that }\DIFdelend \DIFaddbegin [\DIFadd{the glowing veins}] \DIFaddend still wouldn’t even show pain, because people are gonna look at that and just go like, ‘cool.’ They just see glowing things on your arm.”} \DIFdelbegin %DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{To P5’s point, these private and often implicit representations of disability were valuable to participants even }\DIFdelend \DIFaddbegin \DIFadd{Even }\DIFaddend though most other social VR users would not \DIFdelbegin \DIFdel{make the logical leap necessary to }\DIFdelend understand that a disability was being expressed\DIFaddbegin \DIFadd{, these private and often implicit representations of disability were still valuable to participants}\DIFaddend .

\subsection{Invisible Disability Disclosure Practices Differed Based on A User’s Context}
\DIFdelbegin \DIFdel{While many users opted to engage in social games, not all }\DIFdelend \DIFaddbegin \DIFadd{In this section, we explore participants’ varied motivations for disclosing or sharing their disability identity, informed by both different social VR environments and the dynamic nature of their disabilities. Then, we highlight participants’ suggested customization features and methods for making the customization process more accessible. 
}

\DIFadd{A variety of social factors influenced participants’ disclosure strategies: some were comfortable with disclosing their identity at all times, some preferred disclosing only some of the time, and others did not want to disclose in social VR at all. We found that participants generally belonged to one of three groups: }\textbf{\DIFadd{Activists}}\DIFadd{, }\textbf{\DIFadd{Non-Disclosers}}\DIFadd{, and }\textbf{\DIFadd{Situational Disclosers}}\DIFadd{. }\textbf{\DIFadd{Activists}} \DIFadd{were always open to disclosing to spread education and awareness, often tying into advocacy work that the participants did outside of }\DIFaddend social VR contexts\DIFdelbegin \DIFdel{were casual. For P6, who maintains an avatar for work purposes, there were distinctions between how she approached avatar customization in different environments. }\DIFdelend \DIFaddbegin \DIFadd{. }\textbf{\DIFadd{Non-Disclosers}} \DIFadd{did not want to disclose their invisible disability to others in any circumstances. Lastly, }\textbf{\DIFadd{Situational Disclosers}} \DIFadd{were sometimes open to disclosing their identity, and would rely on context cues to make their disclosure decisions. 
}\DIFaddend 

\DIFaddbegin \subsubsection{\DIFadd{Activists and Non-Disclosers}}
\DIFadd{One participant was part of the }\textbf{\DIFadd{Activist}} \DIFadd{group: P1 identified as an outspoken disability activist and felt comfortable openly sharing her disability identity in social VR. She felt that disclosing her chronic condition was helpful not only for raising awareness but also for indicating her access needs.
 }

\DIFaddend \begin{quote}
“I \DIFdelbegin \DIFdel{care a lot more about what my avatar looks like if I am engaging professionally for sure, because if I }\DIFdelend \DIFaddbegin \DIFadd{am an activist and an advocate for folks that have invisible disabilities… I}\DIFaddend ’\DIFdelbegin \DIFdel{m playing ping pong with my dad, I }\DIFdelend \DIFaddbegin \DIFadd{m an open book. So anything that can start a conversation or encourage people to ask questions is really valuable to me, and I feel like having that option is just really important in terms of raising awareness for things like that. And I like people to actually know. If I}\DIFaddend ’\DIFdelbegin \DIFdel{ll just use the default avatar or show up as a cat… Professionally, I manage it similarly to how I would dress if I were going to this event in-person professionally}\DIFdelend \DIFaddbegin \DIFadd{m going to start a friendship with somebody, I want them to be aware of the fact that I have a chronic illness, because that is a pretty large part of my life, and it does affect my ability to socialize sometimes. So you know, being open about that is important to me personally}\DIFaddend .” (\DIFdelbegin \DIFdel{P6, 24F}\DIFdelend \DIFaddbegin \DIFadd{P1, 32F}\DIFaddend )
\end{quote}

\DIFdelbegin \DIFdel{Just as social VR can host a number of social and professional engagements like those found in the non-virtual world, it is also home to diverse spaces thatcan offer experiences ranging from relatively safe communities to potentially harmful environments.P1 points out:  
}\DIFdelend \DIFaddbegin \DIFadd{On the other hand, one participant was not comfortable disclosing their disability identity in social VR at all. P8, a }\textbf{\DIFadd{Non-Discloser}}\DIFadd{, concealed his invisible disability in all non-virtual social situations and did not want to disclose in social VR either, as he felt that }\textit{\DIFadd{“}[\DIFadd{others}] \DIFadd{wouldn't be very receptive or kind to that”}} \DIFadd{and he did not want to be treated as }\textit{\DIFadd{“lesser than someone else.”}} \DIFadd{He emphasized that his invisible disability was not a core part of his identity, especially as it was }\textit{\DIFadd{“a condition that didn’t come until the last five years or so, so it’s not like I grew up with it”}} \DIFadd{(P5). Additionally, having observed others face negative stigmas strengthened his opinion of not disclosing his identity in any contexts, VR or otherwise: 
}

\DIFaddend \begin{quote}
\DIFdelbegin \textit{\DIFdel{“Personally, I’m totally fine with having }%DIFDELCMD < [%%%
\DIFdel{disability representations}%DIFDELCMD < ] %%%
\DIFdel{on all the time. But I really understand why somebody wouldn’t want to have that option to turn it off, especially if you’re going into more of a rough and rowdy crowd, like in VR Chat. You don’t want to make yourself a target for people that might look for things to hurt you with. A lot of the communities that I hang out in on all social VR platforms, typically, I know that the people that are hanging out there are going to be more kind, empathetic people. But if you’re going to a place that you don’t really know very well, I think it would be a good idea to be able to turn that off or on.”}} %DIFAUXCMD
\DIFdel{(P1, F, 32 years old}\DIFdelend \DIFaddbegin \DIFadd{“It comes from personal experience, because I've known people in the past… friends that have also had }[\DIFadd{my condition}]\DIFadd{, it's like you're treated differently. … It probably wouldn’t come up unless someone else brought it up… I’m trying to hide it so much that, outside of my family, I don’t think I ever opened up to anyone about it.” (P8, 20M}\DIFaddend )
\end{quote}

\DIFaddbegin \subsubsection{\DIFadd{Situational Disclosers: Disclosure Practices Informed by Perceptions of Stigma}}
\DIFadd{Participants’ different contexts, which encompassed both the VR environment and their day-to-day disability experience, had a strong impact on when and why they chose to disclose their invisible disability. While only a couple of participants identified as Activists or Non-Disclosers, the remaining 12 participants expressed varying degrees of excitement and hesitancy to represent their disability identity. Most did not want to disclose their disabilities in large group contexts because of their perceptions of the stigma they would face and due to prior negative experiences with disclosure. For example, }\DIFaddend P9 \DIFdelbegin \DIFdel{emphasized embodied avatars}\DIFdelend \DIFaddbegin \DIFadd{mentioned how he tried to mask or pass as nondisabled when interacting with others in social VR: }\textit{\DIFadd{“I don’t really represent my disability too much, but I also don’t conceal it.”}}

\DIFadd{For six Situational Disclosers, their intended audience significantly influenced their avatar design choices, and they often chose to disclose to support other disabled people in a safe space. For example, P3, P4, P6, and P9 stated that they were more likely to disclose in a disability-specific community rather than a large social situation. P9 also specifically mentioned that disclosing in this context allowed them to empathize and engage by sharing }\textit{\DIFadd{“something that I struggle with as well”}} \DIFadd{(P9). Similarly, P2 felt that sharing more about their experience through their bio could provide support to others who were having trouble navigating their invisible disability: }\textit{\DIFadd{“I very much enjoy }[\DIFadd{being}] \DIFadd{open with people, especially once I’ve made a connection with them. I don’t feel like it puts me at any risk or any danger… if anything, it adds to my support system.”}} \DIFadd{P4 also acknowledged that she did not want to disclose her disability to just any person in social VR: }\textit{\DIFadd{“we would mostly have to become friends outside of the virtual reality world for me to feel comfortable to disclose it.”}}

\DIFadd{Regardless of the scale of a social context, some felt as though certain disabilities carried more stigma compared to others. P4 was interested in disclosing two of her invisible disabilities but not a third \textemdash{} she felt comfortable representing dyslexia and chronic pain, but not epilepsy: }\textit{\DIFadd{“I’ve had more hatred for }[\DIFadd{having epilepsy}] \DIFadd{than dyslexia because most people understand dyslexia.”}} \DIFadd{Furthermore, P5 mentioned that the stigmas associated with Asperger}\DIFaddend ’\DIFdelbegin \DIFdel{connections to his mood, especially when expressing his experienceof Bipolar Type 1. He uses VR avatar appearances, and especially their colors, to communicate his emotions nonverbally, strategically selecting avatars based on his goals for social interactions that day. When sharing screenshots of his current avatars, he explained his use of visual affordances and their social and psychological effects: 
}\DIFdelend \DIFaddbegin \DIFadd{s and ADHD were }\textit{\DIFadd{“embarrassing”}} \DIFadd{and commonly }\textit{\DIFadd{“poked fun at a lot online,”}} \DIFadd{which furthered his concerns of being disrespected due to the }\textit{\DIFadd{“negative public perception”}} \DIFadd{of his disabilities. P12 also described their prior experiences of facing discrimination against neurodivergent people: 
}

\DIFaddend \begin{quote}
\DIFdelbegin \textit{\DIFdel{“The middle avatar is the avatar I use when I’m in a playful mood. It stands out, but it’s also really friendly looking. I got a lot of people that like to hang around with me in this one if I’m feeling energetic, a little bit extroverted. If we talk about bipolar phases a little bit more, like the maniac phase, I’ll use the middle one. … Yeah, I like to rotate between these 5. I kind of think of it as ‘How can I best express myself and kinda let others know how I’m feeling based on the avatar?’ If I’m in a really happy mood, but I pick an avatar with like no color, for few emotions, it wouldn’t really match. Same thing vice versa. It also adds some novelty to VR chat as well, because if I see myself in the same avatar for too long, I feel like I start to get fixed. I start to lock myself in the avatar. So, I like to mix it around, so I know there’s always flexibility to iterate and change.”}}  %DIFAUXCMD
\DIFdel{(P9, 28M}\DIFdelend \DIFaddbegin \DIFadd{“I don't go out of my way all the time in VR to disclose my disability. Some, if not many, people may not fully understand what the disability is about. Or, they'll jump to conclusions and assume… I don't want to get labeled that way. I don't want to be labeled as someone who's }[\DIFadd{r-word}]\DIFadd{. Unfortunately, which you know, that word has been thrown around a lot recently and with very negative connotations.” (P12, 31M}\DIFaddend )
\end{quote}

\DIFdelbegin \DIFdel{Though }\DIFdelend \DIFaddbegin \DIFadd{Given the dynamic and fluctuating nature of some invisible disabilities, some participants expressed that their disclosure preferences changed as needed. For example, }\DIFaddend P2\DIFdelbegin \DIFdel{expressed amazement at the current state of technology, she also shared some ideas for future development, including dynamic representations of energy: }\DIFdelend \DIFaddbegin \DIFadd{, P6, and P10 chose to disclose their disability based on their mood or flare-ups. P2 mentioned that she would sometimes disclose their disability to help others }\textit{\DIFadd{“understand what I’m going through… to avoid conflict,”}} \DIFadd{especially in a work setting. P6 also noted that }\textit{\DIFadd{“I really only disclose if I feel like I’m about to have a flare up.”}} \DIFadd{Similarly, P10 mentioned: }\textit{\DIFadd{“when my Hashimoto’s flares up, I lose lots of hair, I have no energy, and I am just tired… So people }[\DIFadd{can be like}]\DIFadd{, ‘Okay, she’s dealing with that today.’”}} \DIFadd{P3 elaborated on how having customizable avatars played a psychological role in grounding her VR experiences: }\textit{\DIFadd{“}[\DIFadd{having options}] \DIFadd{gives you virtual reality with just a little bit of more normalcy. … It gives you a little bit of an anchor to not overwhelm you”}} \DIFadd{(P3).
}

\DIFadd{Participants also shared how they wished to toggle specific avatar features on and off to support  their dynamic disclosure preferences. P9 shared that he felt comfortable and open to disclosing their disability in social VR, but that having a toggle for disclosure features could be crucial for avoiding ableism in unwelcoming settings. As someone with social anxiety, P10 also thought that having options to both (1) have her disability representation permanently fixed to their avatar and (2) select her disability representation on a daily basis would be most helpful: }\DIFaddend \textit{“\DIFdelbegin \DIFdel{An energy bar, like in a video game where }\DIFdelend \DIFaddbegin \DIFadd{if }\DIFaddend you have \DIFdelbegin \DIFdel{your life meter. If it}\DIFdelend \DIFaddbegin \DIFadd{social anxiety every single day, there}\DIFaddend ’s \DIFdelbegin \DIFdel{full, }\DIFdelend \DIFaddbegin \DIFadd{no reason to switch that on and off. That gives }\DIFaddend you \DIFdelbegin \DIFdel{’re full of energy}\DIFdelend \DIFaddbegin \DIFadd{anxiety}\DIFaddend , \DIFdelbegin \DIFdel{and it}\DIFdelend \DIFaddbegin \DIFadd{having to go do that every day.”}} \DIFadd{P3 explained how the toggles could be used for not only representing, but also managing her invisible disability: 
}

\begin{quote}
\DIFadd{“My VR Avatar is whatever I}\DIFaddend ’\DIFdelbegin \DIFdel{s all the way green…And if I}\DIFdelend \DIFaddbegin \DIFadd{m feeling at the moment. If I}\DIFaddend ’\DIFdelbegin \DIFdel{m really low on energy, }\DIFdelend \DIFaddbegin \DIFadd{m feeling immersed in my invisible illness, then I’m probably gonna want my avatar to be also. And if I’m feeling like, ‘okay, I’m escaping reality,’ I don’t want my avatar to be even close to what I am. }[\DIFadd{In our support group,}] \DIFadd{there will still be some days that I don’t want to manifest }[\DIFadd{my disability}]\DIFadd{. And then other days where it’s like, ‘Yeah, I’m feeling like crap and }\DIFaddend I’\DIFdelbegin \DIFdel{ve got a red bar.}\DIFdelend \DIFaddbegin \DIFadd{ll let you people know it in a non-verbal way,’ and I will come in there all crippled up with my avatar, altered to represent how I feel right now simply because I am trying to communicate it in a nonverbal way.}\DIFaddend ” \DIFdelbegin %DIFDELCMD < \MBLOCKRIGHTBRACE
%DIFDELCMD < %%%
\DIFdelend \DIFaddbegin \DIFadd{(P3, 56F)
}\end{quote}
\DIFaddend 

\DIFdelbegin \DIFdel{Despite some marked similarities between the virtual and non-virtual domains,several }\DIFdelend \DIFaddbegin \subsubsection{\DIFadd{Social VR vs. Non-Virtual Disclosure Preferences}}
\DIFadd{Some }\DIFaddend participants perceived social VR to be a relatively safe space where they could freely express their disability-related identities without worrying as much about the stigma they \DIFdelbegin \DIFdel{face }\DIFdelend \DIFaddbegin \DIFadd{faced }\DIFaddend in the non-virtual world. \DIFdelbegin \DIFdel{P9 }\DIFdelend \DIFaddbegin \DIFadd{For example, a few participants }\DIFaddend felt more open to disclosing \DIFdelbegin \DIFdel{his }\DIFdelend disabilities in social VR because \DIFdelbegin \DIFdel{, unlike in the non-virtual world, he felt }\DIFdelend a disability label would not persist beyond \DIFdelbegin \DIFdel{the current }\DIFdelend \DIFaddbegin \DIFadd{their }\DIFaddend VR experience. P9 explained: \textit{“I feel like once I label myself [with a disability] in real life, it becomes something that kind of follows you around.”} 

\DIFdelbegin \DIFdel{P12 expanded on how situational disclosure might be impacted by the VR context:  
}%DIFDELCMD < \begin{quote}
%DIFDELCMD <     %%%
\textit{\DIFdel{“I don’t mind disclosing, but it’s on a situational basis, especially based on the virtual environment in the case of VR versus a real-life environment. I mean, I’ll even give you a small example. There are times when I maybe wouldn’t necessarily disclose my disability in real life if, say, I’m stressed, but I would just tell the person I’m interacting with if I personally notice myself interacting that way. That’s something else with my disability, I noticed. Sometimes, I will be self-aware of how I’m feeling and how I’m interacting, but other times, it will just be impulsive, and it will feel like a blur.”}} %DIFAUXCMD
\DIFdel{(P12, M, 31 years old)
}%DIFDELCMD < \end{quote}
%DIFDELCMD < %%%
\DIFdelend \DIFaddbegin \DIFadd{However, others felt as though social VR experiences ranged from relatively safe communities to potentially harmful environments. For example, P13 recalled a news article reporting about a woman being assaulted in social VR spaces, and briefly mentioned his own experiences of being assaulted in VR. When speaking about specific VR platforms, P1 acknowledged how disability disclosure in social VR could potentially result in harassment:  
}\DIFaddend 

\DIFdelbegin \DIFdel{P3 unpacked more of the nuances behind transforming non-virtual representations into embodied VR environments, indicating the factors that contribute to her decision about the extent she wants to represent herself in VR: 
}\DIFdelend \begin{quote}
\DIFdelbegin \textit{\DIFdel{“My VR Avatar is whatever I’m feeling at the moment. If I’m feeling immersed in my invisible illness, then I’m probably gonna want my avatar to be also. And if I’m feeling like, ‘okay, I’m escaping reality,’ I don’t want my avatar to be even close to what I am. }%DIFDELCMD < [%%%
\DIFdel{In support group,}%DIFDELCMD < ] %%%
\DIFdel{there will still be some days that I don’t want to manifest that. And then other days where it’s like, ‘yeah, I’m feeling like crap and I’ll let you people know it in a non-verbal way,’ and I will come in there all crippled up with my avatar, altered to represent how I feel right now simply because I am trying to communicate it in a nonverbal way.”}} %DIFAUXCMD
\DIFdel{(P3, F, 56 years old)
}%DIFDELCMD < \end{quote}
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{Beyond the support group setting, she noted the importance of having the option to accurately reflect her non-virtual self, in a way normalizing the uncanny valley effect of embodied avatars that are: 
}%DIFDELCMD < \begin{quote}
%DIFDELCMD < %%%
\textit{\DIFdel{“A way I might have looked once upon a time. They keep me from aging…I’m not the type of person who changes }%DIFDELCMD < [%%%
\DIFdel{my avatar}%DIFDELCMD < ] %%%
\DIFdel{all the time, and it puts me in a little suspended animation where I haven’t aged in six years.”}} %DIFAUXCMD
\DIFdel{(P3, F, 56 years old}\DIFdelend \DIFaddbegin \DIFadd{“Personally, I’m totally fine with having }[\DIFadd{disability representations}] \DIFadd{on all the time. But I really understand why somebody wouldn’t want to have that option to turn it off, especially if you’re going into more of a rough and rowdy crowd, like in VR Chat. You don’t want to make yourself a target for people that might look for things to hurt you with. A lot of the communities that I hang out in on all social VR platforms, typically, I know that the people that are hanging out there are going to be more kind, empathetic people. But if you’re going to a place that you don’t really know very well, I think it would be a good idea to be able to turn that off or on.” (P1, 32F}\DIFaddend ) 
\end{quote}

\DIFdelbegin \DIFdel{She elaborated on customizable avatars’ psychological role in grounding her VR experiences : 
}\DIFdelend \DIFaddbegin \subsubsection{\DIFadd{Intersectional Identity Representation}}
\DIFadd{Disability is one facet of the complex human experience, filtered through intersecting lenses of other identities like gender and race. Participants identified connections between the experiences of people in multiple marginalized groups. Speaking to experiences of other identities, P6 acknowledged her intersectional identities of race and invisible disability but had varying perspectives on whether to represent them in her avatars. Her daily experiences in social and workplace settings also informed her avatar disclosure preferences:
}

\DIFaddend \begin{quote}
\DIFdelbegin \textit{\DIFdel{“}%DIFDELCMD < [%%%
\DIFdel{Having options}%DIFDELCMD < ] %%%
\DIFdel{gives you virtual reality with just a little bit of more normalcy. Just enough normalcy to make me go, ‘Okay, I’m not gonna run from this. It’s not so foreign that it’s freaking me out.’...It gives you a little bit of an anchor to not overwhelm you.}} %DIFAUXCMD
\DIFdelend \DIFaddbegin \DIFadd{“I feel like I’m seen as unreliable. Obviously, I’m also a Black woman, so that compounds things \textemdash{} that intersection of discrimination. But I do feel like I actively do not get treated well when I talk about it. I guess in social situations, I'm not concerned about it the way that I am in professional circumstances. … The intersection of disability and race has made me a lot less likely to disclose over the years. As I’ve seen, figures of authority are not necessarily empathetic or respectful about it.” }\DIFaddend (\DIFdelbegin \DIFdel{P3, F, 56 yearsold}\DIFdelend \DIFaddbegin \DIFadd{P6, 24F}\DIFaddend )
\end{quote}

\DIFdelbegin \subsection{\DIFdel{Suggested Features for Customizing Disability Representations}}
%DIFAUXCMD
\addtocounter{subsection}{-1}%DIFAUXCMD
\DIFdelend \DIFaddbegin \DIFadd{When speaking about the personal importance of disclosing his invisible disability identity, P12 drew parallels between LGBTQ and disability representation in media. He cited LGBTQ award-winners at the Tony Awards as examples of ways that queer people expressed and disclosed their identity through clothing and other visual means.
}\DIFaddend 

\DIFaddbegin \begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{imgs/P12.png}
    \caption{\DIFaddFL{Participant 12’s images, sticky notes, and suggestions for invisible disability representation during the whiteboard component of the study, featuring screenshots of two different avatars he uses. The images are blurred to preserve the participant’s anonymity.}} 
    \Description{Participant 12’s images, sticky notes, and suggestions for invisible disability representation during the whiteboard component of the study. On the top there are four sticky notes, reading “Important notes for Autism and Aspergers with Avatars in VR: 1. Make sure facial expressions and non verbal expressions are accurate and can also include descriptions as needed.” / “For those who also may be LGBTQ or have a physical disability, have accurate representations of them.” / “Offer opportunity to have a community for those to share similar interests as a way of  improving socialization” / “Learn behavioural techniques in virtual environments and inhibit restrictions to help.” Below the sticky notes are three screenshots of P12’s avatar. On the left is a screenshot of his avatar’s head and torso with a box sketched to the right of his head. The avatar is 3D, light-skinned, has a beard, short hair, sunglasses, and a Unity sweatshirt. The middle screenshot shows a 2D avatar with glasses, a goatee, and wearing a blue shirt with a brown vest; the avatar’s hands are raised and it says “Happy New Year!” above his head. The screenshot on the right is a zoomed out version of the screenshot on the left, showing the 3D avatar’s whole body.}
    \label{P12}
\end{figure*}

\subsection{\DIFadd{Accessible Methods for Customizing Avatars}}
\DIFaddend Five participants (P1, P2, P4, P5, P7) expressed interest in easier processes for importing and creating custom designs. P4 suggested \DIFdelbegin \DIFdel{: }\DIFdelend \DIFaddbegin \DIFadd{having }\DIFaddend \textit{“\DIFdelbegin \DIFdel{It’d be nice to have }\DIFdelend different options, like with different logos or different quotes that you want to put on shirts. It’d be nice to have a set-up so that you can do it pretty easily [because] I definitely don’t have the coding experience to be able to go any further.”} \DIFdelbegin %DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{Additionally, }\DIFdelend \DIFaddbegin \DIFadd{Another participant explained that current avatar customization processes were inaccessible due to the physical manifestations of their disability that impacted their mobility. }\DIFaddend P5 \DIFdelbegin \DIFdel{wanted }\DIFdelend \DIFaddbegin \DIFadd{wished }\DIFaddend to minimize arm movement requirements due to Repetitive Strain Injury\DIFaddbegin \DIFadd{, }\DIFaddend and shared ideas for optimizing user experiences through evolving technology: 

\begin{quote} 
\DIFdelbegin \textit{\DIFdel{“I could copy and paste it. That’s my ideal customization because I don’t like the menus. If you have the option of pressing a bunch of buttons or just being able to think it and it appears on the page, why would anyone want to have all the billion options when they could do the exact same thing? It has occurred to me, though, like with the recent AI developments, where you can produce pictures, it seems like it’s not too far away that they could just produce a 3D model using those systems. Like if there was a system where you could describe it, and it would generate one.”}} %DIFAUXCMD
\DIFdelend \DIFaddbegin \DIFadd{“I could copy and paste it. That’s my ideal customization because I don’t like the menus. If you have the option of pressing a bunch of buttons or just being able to think it and it appears on the page, why would anyone want to have all the billion options when they could do the exact same thing? It has occurred to me, though, with the recent AI developments, where you can produce pictures, it seems like it’s not too far away that they could just produce a 3D model using those systems. Like if there was a system where you could describe it, and it would generate one.” }\DIFaddend (P5\DIFdelbegin \DIFdel{, M, 31 years old) 
 }\DIFdelend \DIFaddbegin \DIFadd{, 31M) 
 }\DIFaddend \end{quote}

\DIFdelbegin \DIFdel{Even though invisible disabilities often have unrecognizable and misinterpreted features, some have physical manifestations that can impact mobility. For P5, his constrained arm movements shaped the way he approached avatar customization and ultimately his vision for an ideal customization process. }%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{P11 also had a wealth of ideas for ways to customize avatars, including }\textit{\DIFdel{“simple sliders and buttons…3D models you can customize…options to select what types of disabilities and neurodivergent conditions you identify as, and then you get a chance to customize the symbols or the icons.”}} %DIFAUXCMD
\DIFdel{He explained: }\textit{\DIFdel{“I think an ability for you to be able to type in what you’re saying or what you want through maybe image generation or text to 3D tools would be a great way to do that,”}} %DIFAUXCMD
\DIFdel{which would reduce the burden of users navigating complex customization systemswithin social VR systems themselves. }\DIFdelend Participants also mentioned that text-to-avatar pipelines could lower the barrier to avatar customization, which was perceived as intimidating for participants who did not know how to use Unity or other platforms that rely on user coding. \DIFaddbegin \DIFadd{P11 had multiple ideas for ways to customize avatars, including }\textit{\DIFadd{“simple sliders and buttons… 3D models you can customize… options to select what types of disabilities and neurodivergent conditions you identify as, and then you get a chance to customize the symbols or the icons.”}} \DIFadd{He felt that }\textit{\DIFadd{“}[\DIFadd{being}] \DIFadd{able to type in what you’re }[\DIFadd{thinking}]\DIFadd{, or what you want through maybe image generation or text to 3D tools, would be a great way to do that,”}} \DIFadd{as it would reduce the burden of users navigating complex customization systems within social VR systems themselves. 
}\DIFaddend 

\DIFdelbegin \DIFdel{As technology continues to evolve, it is no surprise that social VR users are eager to see emerging technologies implemented in the pursuit of improving the accessibility of social VR spaces. 
A key component of building an inclusive society is purposefully using resources, such as technology, to further our societal goals. Though our participants offer only a couple of examples here, designers should consider which features of emerging technologies could help shape a more inclusive tomorrow as they are being designed and implemented across the globe. 
}\DIFdelend \section{Discussion}

Avatar customization libraries decide who gets to express what identity, and current options do not enable the explicit expression of invisible disabilities. In our study, we found that people with invisible disabilities are interested in representing their disabilities through social VR platforms. Unlike people with visible disabilities who often depict disabilities through adding assistive technology to their avatars \cite{zhang_diarystudy}, representation of invisible disabilities tend to adopt more nuanced and symbolic approaches, including clothing-based designs (such as custom disability-related graphics) as well as accessory-based features (such as a floating energy bar). Additionally, a distinction emerged between public representations with explicit meaning and more private representations with personal significance and implicit meaning. Sometimes motivated by educational and awareness-raising goals, sometimes motivated by traumatic non-virtual disclosure experiences, we discovered that context informs virtual disclosure preferences.  It is important to note that social VR offers users access to a distinct set of verbal and non-verbal cues that can powerfully communicate shifting needs and preferences. Through the unique multimodal interactions afforded by social VR avatars (e.g., synchronous voice chat, motion tracking, facial expression), we found participants leveraged disability representation in more varied ways than on social media. 

\DIFaddbegin \subsection{\DIFadd{Taxonomy for Disability Disclosure}}
\DIFadd{We discovered themes surrounding disclosure, perceptions of stigma, and novel representations of invisible disabilities, as described below. We begin by highlighting the perceptions of stigma that impact disclosure decisions. Then, we examine three motivational groups that emerged from the data: }\textbf{\DIFadd{Activists}}\DIFadd{, }\textbf{\DIFadd{Situational Disclosers}}\DIFadd{, and }\textbf{\DIFadd{Non-Disclosers}}\DIFadd{. Throughout, we examine the unique affordances of social VR that facilitate novel disability expression and disclosure considerations.
}

\DIFadd{The data indicated that participant motivations for disclosure fell into three groups. The first group, Activists, were always open to disclosing to spread education and awareness. The second group, Situational Disclosers who were sometimes open to disclosing, would rely on context cues and environmental culture to make their disclosure decisions. The third group, Non-Disclosers, could not think of a situation where they would disclose their invisible disability to others. 
}

\DIFadd{As alluded to by the taxonomy above, 
}

\DIFaddend \subsection{Leveraging multimodality to represent disability in social VR.}
Disability disclosure preferences often vary by context and condition, a nuanced choice that becomes more pronounced with social VR embodiment and real-time immersion \cite{freeman_maloney_perception_of_self}. Mack et al. \cite{mack_towards} explored contextual differences across digital gaming and social platforms such as Roblox and Snapchat but did not explore embodied avatars, yet they found that non-digital experiences can inform expectations of digital spaces, just as we discovered non-virtual experiences inform virtual preferences. Despite this area of overlap, as acknowledged by P9, the engagement afforded by social VR, compared to digital social media platforms, can greatly influence avatar perceptions. Since avatars are the predominant form of self-expression in social VR, it is imperative to ensure that people have just as much, if not more, flexibility in representing their identities as they do in non-virtual spaces. We extend prior findings on invisible disability representation by examining social VR’s multimodal affordances for identity expression. While social media limits open disclosure to 2-D visual and text, social VR offers users multiple channels for sensory expression in addition to adding wearable disability representation through embodied avatars that might not be practical to carry around in still photos (e.g., a floating and dynamic energy bar to represent the user’s energy level during embodied social interactions). 

\subsection{Enabling adaptive disability representation for context-specific needs.}
Deciding whether to disclose is an ongoing negotiation across both digital (non-embodied) and virtual (embodied) platforms. In the context of embodied social VR, a recent study revealed that avatars with disability representations were more likely to experience ableism harassment during group social interactions \cite{zhang_diarystudy}. As such, it is important to offer an easy-to-use toggle on and off feature with disability representations so users can operate with the utmost autonomy in their avatar disclosure decisions. At present, avatar design processes are complex. Customization platforms such as Ready Player Me \cite{readyplayerme} offer “hundreds of options” but are often inaccessible to people from non-technical backgrounds. To streamline the customization process, we suggest that avatar design processes implement more options relevant to invisible disabilities so that self-representation is also accessible for users from non-technical backgrounds. Further, taking inspiration from participant suggestions like the dynamic energy bar, we suggest that future avatar designs incorporate intuitive and universally applicable design conventions (e.g., traffic light color guidelines \cite{traffic_light}), allowing users to effectively express themselves.

Our findings support preliminary discussions of invisible disability representation in non-virtual contexts, where there was interest in symbolically representing and disclosing invisible disabilities through toggling representations on and off. In a higher education context, Canadian university students expressed interest in a concealable invisible disability identity marker to generate greater understanding, such as a blue dot in place of the handicapped sign associated with visible disabilities \cite{mullins_invisible_uni}. The present study’s participants strengthened and expanded on this initial suggestion by offering more actionable implementations of disability expression across various modalities, which speaks to the creativity and self-exploration offered in VR affordances versus non-virtual settings. 

\DIFaddbegin [\DIFadd{copied from the last findings section}]
\DIFadd{As technology continues to evolve, social VR users hope that emerging technologies can improve the accessibility of social VR spaces and interactions. Though our participants offer only a couple of examples here, designers should consider which features of emerging technologies could help shape a more inclusive tomorrow as they are being designed and implemented across the globe. 
}\DIFaddend \subsection{VR Customization Design Recommendations} 

Based on our findings, we offer the following list of design recommendations. 

\begin{enumerate}
\item \textbf{Create more options for multimodal customization.} 
        \begin{itemize}
            \item For some users with invisible disabilities, certain forms of communication are more comfortable than others (e.g., verbal, visual, etc.). 
	\item By making it possible for users to dive further into fine-tuning their movements and facial expressions to represent physical communication of accommodations needs and dynamic thresholds for social interaction, social VR platforms can maximize a breadth of opportunities for making social VR a better experience for those with invisible disabilities.
        \end{itemize}
\item \textbf{Include explicit options for invisible disability representation on social VR customization platforms.} 
        \begin{itemize}
            \item Even though some participants suggested highly individualized representation ideas, \textbf{we recommend including awareness-building apparel and accessory options in customization libraries} (e.g., zebra print for rare disease month, dyslexia-oriented t-shirt design, giant spoon accessory for representing chronic illness). Navigating customization can be challenging for multiple reasons (see examples below), so offering a number of pre-set invisible disability representation features can help eliminate barriers to boosting awareness and facilitating self-expression. 
        \end{itemize}
\item \textbf{Make the avatar customization process more accessible.}
        \begin{itemize}
            \item Many social VR users \textbf{do not have the programming background} necessary to manually fine-tune more individualized customization features like those that might represent invisible disabilities.
            \item People with invisible disabilities want to be able to \textbf{upload custom apparel logos and t-shirt designs} that represent their disabilities. 
            \item Because of the \textbf{personal significance of many suggested disability representations}, a number of invisible disability-related customizations would need to be individually uploaded by social VR users.
            \item Consider ways to \textbf{minimize or remove the physical burden of swiping} through long lists of customization options to enhance accessibility, including customization by way of text or drawing. 
        \end{itemize}



\section{Limitations}

The recruitment process for this study was challenging in multiple ways.  Due to the invisible nature of the disabilities in our population of interest, participants had to feel comfortable disclosing they had an invisible disability to engage in the interview. We also considered that some people with chronic illnesses, neurodivergence, or other invisible disabilities might not identify as having an invisible disability. So, we altered our language in different rounds of recruitment, ensuring we included examples of invisible disabilities in every note. Additionally, because we only included consenting adults ages 18+ in the present study, we were unable to connect with the large population of youth and teen VR users and gamers. Despite these challenges, we recruited a strong sample of 12 participants who shared many overlapping experiences while also bringing to their interviews diverse suggestions and rich viewpoints. We halted recruitment once thematic saturation was achieved. 

Given that we recruited from primarily U.S. mailing lists, we recognize the geographic limitations of this study and acknowledge the importance of situating findings in diverse cultural and socioeconomic contexts. We understand that disability representation preferences, especially those linked to established symbolism, are culturally and geographically dependent. For example, while symbols  like spoon theory’s spoon are globally recognized for representations of invisible disability, others, like the Australian use of the sunflower on apparel and accessories, are less universal. Though we recruited from organizations, listservs, and social media threads globally (with some exceptions due to legal restrictions), our present demographics collection process did not include the participant country of origin.  We acknowledge that future projects would benefit from a more globally situated and culturally sensitive lens. 




\section{Conclusion}

Avatars mediate interpersonal interactions between social VR users, but at present, no built-in options exist for people to explicitly represent invisible disabilities. In this study, we explored the avatar customization preferences of people with invisible disabilities. Users wanted to tap into VR’s multimodal affordances (e.g., facial expressions, body language) to communicate their invisible disabilities. More broadly, users were interested in representing their invisible disabilities through various explicit avatar features (e.g., clothing, floating icons), and many expressed a need for an easily usable mechanism that could toggle disability representations on and off in different contexts. Interestingly, there emerged a distinction between public and private representations of disability, introducing a new level of nuance to our prior understanding of what it means to represent disability. We offer a new perspective that takes into consideration the importance of personal significance during self-expression, in addition to explicit and widely understood symbols for invisible disabilities. To our knowledge, this is the first study to capture the avatar representation wants and needs of social VR users with invisible disabilities. Broadly, our findings contribute to the ongoing conversation of designing with and for people with invisible disabilities. We hope this study inspires more researchers to offer future contributions to the valuable study of invisible disability representation and accessibility in VR. 

==> sections/new.tex <==
\section{Introduction}
Like anyone else, people with disabilities want to represent their unique identities through their avatars when interacting with others in social virtual reality (VR) spaces. Social VR platforms offer users a strong sense of embodiment and freedom from some forms of physical constraint, and as more people turn to VR for social connection, the importance of diverse mechanisms for self-expression grows \cite{maloney2020falling, yalon2008virtual}. However, given the varying identities of potential social VR users, the accessibility community has yet to understand how disabled social VR users wish to represent diverse disability identities through embodied avatars. 

Among other functions, avatars are vessels for self-expression in VR, and their characteristics provide cues that mediate interpersonal interactions \cite{freeman2021body, won2023your}. Previous research has investigated the avatar representation preferences of people with visible disabilities (i.e., disabilities that are apparent due to the presence of physical characteristics or assistive technologies \cite{cdcdefinition}) in social VR platforms. For example, Zhang et al. \cite{zhang2022s} found that d/Deaf and hard of hearing people and blind and low vision people wanted to disclose their disabilities, highlight their access needs, and raise awareness through their VR avatars and interactions. 

However, many disabled people do not have characteristics that are immediately visible, nor do they use commonly recognized assistive technologies \cite{invisibledisabilitydef}. For the 33 million people in the United States alone who have invisible disabilities (approximately 10\% of the U.S. population) \cite{disabledworld}, they may not use assistive technologies, or their assistive technologies may not be as recognizable or visible. As such, the findings from Zhang et al. do not readily apply to their experiences. 

More recently, Mack et al. \cite{mack2023towards} studied how people with both visible and invisible disabilities prefer to represent themselves on social media platforms (e.g., Snapchat, Animal Crossing, Facebook). The authors found that users with visible disabilities wished for their avatars to show their full bodies and assistive technologies, while users with invisible disabilities wanted to use disability-related symbols (e.g., words in the dyslexia-friendly font “Bionic”) to signify their disability. These distinct preferences underscore how representation needs differ between visible and invisible experiences. As their work focused primarily on digital social media platforms with non-embodied avatars, they only briefly discussed participants’ preferences for embodied avatars on social VR platforms.

Embodied avatars allow users to represent themselves, and their whole bodies, distinct from non-embodied avatars on platforms such as Snapchat and Facebook. On digital platforms, users are limited to 2D, static images of their avatars. Conversely, social VR users use embodied 3D avatars to represent themselves; VR avatars are capable of capturing more granular nuances, such as dynamic facial expressions, body language, and movement patterns as they socialize with others. Prior work has only briefly explored invisible disability representation in embodied avatars like those found in social VR spaces. At present, little is known about invisibly disabled users’ unique preferences for identity representation of multiple identities, including race, gender, and multiple invisible disabilities, in embodied avatars and social VR spaces. 

We address this gap by examining the embodied avatar preferences of people with invisible disabilities. We investigated how invisibly disabled people currently represent themselves, desired representation mechanisms, and how these preferences might differ across social VR contexts. Specifically, we posed the following research questions: 

\begin{itemize}
	\item \textbf{RQ1:} What are invisibly disabled people’s perceived differences between embodied vs. non-embodied avatars, and how do those differences impact identity representation?
	\item \textbf{RQ2:} How do people with invisible disabilities represent their disability in social virtual reality avatars today, and how do they wish to represent themselves in social VR avatars in the future?
	\item \textbf{RQ3:} In what social VR contexts (when and why) do people with invisible disabilities wish to disclose their disability identities and experiences?
\end{itemize}

We conducted semi-structured interviews with 14 participants with invisible disabilities, such as ADHD, dyslexia, and chronic conditions. We asked them about their current avatars, the similarities and differences between their embodied avatars and their non-virtual appearance, and the different contexts in which they engaged in social VR. During the interviews, we included an interactive brainstorming component where participants drew, typed, or otherwise visualized their \textit{ideal} avatar self-representation, going beyond what is currently available on customization platforms. 

We found that the embodied nature of social VR impacted invisibly disabled users’ disclosure preferences and methods. For example, some perceived social VR to be a safer space than non-virtual social spaces and felt comfortable disclosing their disability, while others preferred not to disclose due to prior uncomfortable experiences in social VR. Additionally, while some users with invisible disabilities already customized avatar appearances to indicate dynamic preferences for social engagement, many wished to lean further into customized facial expressions and body language to express their disabilities. 

We also identified two distinct methods by which invisibly disabled people represented their identity: public (i.e., explicit representations like disability-related shirt graphics) and private (i.e., implicit representations like knee pads that symbolize a need for self-protection from bipolar mood swings). Based on our findings, we conclude with design recommendations to guide more inclusive and accessible avatar customization experiences.

In summary, we contribute novel insights on how avatar customization can support the large and underserved population of people with invisible disabilities. We amplify the voices and experiences of this historically underrepresented group within a social VR context, taking another step toward making social settings more inclusive to all users. 

\section{Related Work}
Despite the invisible nature of some disabilities, identity representation is important. Broadly, social VR platforms lack diverse customization options (e.g., regarding body and racial diversity \cite{lee2014does, lee2011whose, morris2023don}). Invisible disability representation in social VR is also valuable, but even less present. Rendering invisible experiences visible opens doors for building awareness of underrepresented experiences. Further, social VR offers unique affordances for users to represent aspects of their identities in different ways compared to non-virtual contexts \cite{freeman2021body}. We build on prior literature regarding disability disclosure in various contexts, social VR experiences, and avatar customization and identity expression. To our knowledge, we are the first to explore the nuances of disability disclosure across a diverse set of invisible disabilities in embodied social environments. 

\subsection{Disability Disclosure in Employment, Academic, and Social Settings}
Many people with disabilities disabled people have varied perspectives on when and why to disclose their disability. Although discrimination against individuals with disabilities is legally prohibited\footnote{Both the Americans with Disabilities Act (ADA) of 1990 and Section 504 of the Rehabilitation Act of 1973 protect people from discrimination on the basis of a disability.}, discrimination and ableism are prevalent in society. As a result, disabled people with disabilities may have to carefully consider whether or not to disclose their disabilities. 

At school and the workplace, people with disabilities may require accommodations to perform their roles successfully; however, disclosure also heightens the risk of experiencing disability-related discrimination \cite{lindsay2018systematic, lindsay2019disability, wilton2006disability, von2014perspectives, dalgin2008invisible}. In addition to facing the potential of having favorable outcomes than their non-disabled peers in the job application process \cite{pearson2003to}, disabled people with disabilities may also be socially rejected by their peers and supervisors and fear being “reduced” to their disability or stereotypes thereof \cite{lindsay2019disability, lindsay2018systematic}. PDisabled people with disabilities may also fear that disclosure will indirectly impact their academic and professional success due to the damage to their social image \cite{rocco2004towards, toth2022disclosure, toth2014employee, mcgrath2023disclosure, gignac2022workplace}. Prior literature has found that people with invisible disabilities have more concealed their disability more easily than people with visible disabilities, especially if their condition is mild and they believe their conditions are “irrelevant” to their performance \cite{lindsay2019disability, von2014perspectives, dalgin2008invisible}. 

While there is substantial work investigating disabled peoples’ disclosure strategies in employment and academic environments, there is comparatively less research focusing on social settings. Some have explored the nuances of disability disclosure specifically for online dating \cite{porter2017filtered, saltes2013disability}, while others have focused on social media more broadly \cite{furr2016strategic, kaur2022social, heung2024vulnerable}. For example, through semi-structured interviews with people with physical disabilities, Furr et al. \cite{furr2016strategic} explored visibly disabled people’s disclosure strategies on social media. Notably, the privacy and curatorial nature of social media meant that the visible disabilities that participants had were not immediately apparent, mirroring the experiences of people with invisible disabilities. They identified three approaches to social media disability disclosure: open (full disability disclosure to a broad audience), secure (regular disability disclosure to a private audience), and limited (selective disclosure across all audiences). Participants who adopted an open disclosure approach likened disclosing their disability to “coming out” on social media, whereas those who were more hesitant generally avoided disclosure due to prior experiences with ableism and discrimination. Similarly, in a study of disabled content creators’ practices on social media, Heung et al. \cite{heung2024vulnerable} found that some content creators strategically censored or limited their online presence to mitigate disability-related hate and harassment.

Distinct from the experiences of people with visible disabilities, the non-apparent nature of invisible disabilities means that invisibly disabled people may not be taken as seriously when either seeking accommodations or outwardly expressing their disability. Regarding models of invisible disability disclosure, Evans et al. \cite{evans2019trial} found that a single individual often employed multiple disclosure strategies depending on their context, and disclosure decisions were often guided by a need to assert access needs in physical environments (e.g., reading small text, avoiding severe food allergens). Additionally, invisibly disabled people may specifically anticipate negative perceptions stemming from a lack of understanding of their disabilities, which may make them hesitant to disclose \cite{mullins2013lived}. For example, Moriña \cite{morina2022when} found that students with invisible disabilities were challenged by people who refused to believe they were “disabled,” which made them want to distance themselves from a disability identity and appear “normal” \cite{morina2022when}. While people with both visible and invisible disabilities anticipate and encounter stigma, invisibly disabled people may struggle more with validating their disability to themselves and others.

These studies provide necessary grounding for understanding disability disclosure in emerging social settings, such as social VR. Our empirical study provides additional insight into the experiences and challenges that invisibly disabled people face when deciding to represent or disclose their disability in the virtual world.

\subsection{Social Virtual Reality}
Recently, social VR has gained increasing popularity, enabling immersive 3D virtual experiences by allowing users to meet, interact, and socialize in the form of avatars \cite{freeman2021body}. Unlike 2D social media and virtual worlds, social VR affords users immersive embodied experiences through VR head-mounted displays, which allow real-time body movements and gestures to be tracked and rendered in virtual environments \cite{caserman2019real}. A person’s sense of embodiment (SoE) is characterized by their ability to control their body’s movements, experience the sensations their body does, and feel that they are within their body \cite{kilteni2012sense}. Although most commercial headsets do not track a user’s full body or subtler physical cues, like facial expressions and gaze, they still facilitate a greater SoE and social presence than other non-VR platforms \cite{maloney2020falling, tham2018understanding}. Additionally, users can no longer see their physical selves and environments, resulting in them being fully immersed in VR and their virtual bodies \cite{genay2022being}.

With these unique affordances, social VR platforms offer a variety of avatar-mediated activities and social interactions. To understand what people actually do in social VR, Maloney and Freeman \cite{maloney2020falling} interviewed 30 social VR users, finding that users enjoyed experiencing everyday practices (e.g., sleeping) in novel immersive ways and practicing self-improvement skills that they normally wouldn’t do in offline worlds (e.g., social skills and mental states). Users connected with others by hosting and attending parties and other gatherings, playing games together, and working remotely \cite{freeman2021body, abramczuk2023meet}. Furthermore, Won et al. \cite{won2023your} established a design space for understanding avatar representation in different social contexts and for different purposes, ranging from low anonymity and low immersion in professional contexts to high anonymity and high immersion for entertainment. However, while these provide a strong background for understanding some aspects of self-presentation in the virtual world, little is known about invisibly disabled people’s preferences.

Social VR platforms are particularly appealing to people with disabilities since they can address accommodations in ways that go beyond what is possible in the physical world. Virtual reality enables people with physical and intellectual disabilities to engage in active leisure activities, such as snowboarding, which are typically inaccessible to them in the physical world \cite{yalon2008virtual}. Virtual reality can also be leveraged to help people with invisible disabilities. For instance, in VR, neurodivergent users have greater control over their environment, so they may remove themselves from overwhelming situations or adjust settings to reduce their sensory load \cite{boyd2018leveling}. Given its increasing popularity and unique affordances, it is important to understand how invisibly disabled people want to engage and represent themselves within this social sphere.

\subsection{Traditional and Creative Avatar Expression}
Avatars enable users to develop a greater social presence in social VR. Langener et al. determined that avatar customization heightens the user’s sense of connection and ownership over their virtual body, thus intensifying SoE \cite{langener2022immersive}. Prior work has found that avatar realism through both appearance and behavior can heighten users’ sense of immersion and improve interpersonal understanding \cite{roth2016avatar, steed2015collaboration}. In studying selective self-presentation in social VR, Freeman et al. \cite{freeman2021body} identified that many social VR users strove to make their avatars as similar as possible to their non-virtual counterparts because they considered avatars an extension of themselves in virtual worlds. 

Despite some progress, current avatar representation options are generally inadequate at capturing the diverse range of human appearances and identities. Marginalized and stigmatized groups are especially under-represented. For example, Ready Player Me \cite{readyplayerme}, a popular avatar creation tool, presents gender as a binary, which neglects the diversity of gender identity and forces gender-nonconforming people to abide by societal standards. Furthermore, the middle-aged female participants in Morris et al.’s study noted that most avatars they encountered skewed towards youthful appearances, and existing avatar customization made them feel like a “caricature” of an older person \cite{morris2023don}. Researchers have explored identity and avatar representation preferences in social VR, including diverse user groups such as racial minorities \cite{blackwell2019harassment}, women \cite{sharvit2021virtual}, and LGBTQ users \cite{freeman2022acting, freeman2022re, povinelli2024springboard}. Another study explored the avatar choices of non-cisgender users, revealing that they changed their avatar’s gender expression frequently through outfits and accessories to indicate their flexible and gender-fluid identities \cite{freeman2022re}. 

In addition to capturing a person’s non-virtual appearance, avatars are often used to creatively express their users’ interests and identities, sometimes extending beyond what is possible in the physical world. Users may opt for fantastical, cartoonish, and non-human features, such as red or snake-like eyes offered in Ready Player Me \cite{readyplayerme}, or they can choose non-human avatars altogether. Furthermore, users can enable complete or partial invisibility of their avatars by manipulating the meshes that make up the 3D model \cite{youtube_invisibility_toolbox, youtube_PxINKY}. When exploring the contextual dynamics influencing users’ avatar choices, Ribeiro et al. \cite{ribeiro2024towards} found that people most often used avatars that closely resembled their actual appearance in work or academic meetings but preferred having a different representation when interacting or gaming with strangers. With the flexibility of presenting as they are or as they would want to be, users can communicate their uniqueness, explore life as their avatar, and hold greater control over how others perceive them. 

Avatar representation of disability is particularly understudied, with some recent exceptions. Zhang et al. \cite{zhang2022s} found that users disclosed disabilities by attaching assistive technology to their avatars (e.g., hearing aids) and generally wished to align their avatar representations with their non-virtual appearances. Additionally, Davis and Chansiri \cite{davis2019digital} found that online users with disabilities customized their avatars to foster a greater sense of empowerment and embodiment. For instance, one user depicted herself as younger because she felt that her disability removed years from her life. Regarding avatar presentation across multiple digital social media platforms, Mack et al. \cite{mack2023towards} investigated challenges facing individuals with intersectional identities, noting they often had to choose between using avatars to represent their disability or race-related identities.

Our study includes social VR users with all types of invisible disabilities, distinct from Zhang et al.’s study \cite{zhang2022s} focused on people with visible disabilities who use assistive technology. Though many participants with visible disabilities were interested in translating their non-virtual assistive technology into their virtual avatars, little is known about the preferences of invisibly disabled people for embodied representations. In addition, we build on Mack et al.’s study \cite{mack2023towards} on digital avatars. Though their work included participants with invisible disabilities and found they wanted to use symbolic representations of disability that would resonate with their more specific community (e.g., chronic conditions, ADHD), we extend our inquiry to study invisible disability representation preferences into virtual embodied contexts. By investigating the preferences of people with invisible disabilities, who often do not use apparent assistive technologies, we shift the focus from translating assistive technology into the virtual world and explore social VR affordances for illuminating experiences that are not necessarily visible in non-virtual spaces. In this study, we examine how users want to employ VR’s multimodal affordances for disability expression in spaces where avatars mediate all social interaction. 

\section{Methodology}
We conducted and analyzed data from semi-structured interviews with 14 participants who self-identified as having one or more invisible disabilities. We aimed to understand their perspectives on disability representation and disclosure in both non-virtual and VR social settings.

\subsection{Participants}
We recruited 15 participants by emailing disability-related organization mailing lists, posting in relevant subreddits, and partnering with our university’s undergraduate extra credit system. Our inclusion criteria indicated that participants had to be 18 years old or older and have an invisible disability, defined as a physical or psychological condition with no visible manifestation. Participants were also required to have experience using social VR platforms, such as Rec Room, VRChat, vTime XR, and AltspaceVR (recruitment began in January 2023, before AltspaceVR was shut down). Due to inconsistent identification (i.e., different names and spellings) during and after our study, we discarded data from one participant. 

The remaining 14 participants’ ages ranged 20 to 56 years old ($mean = 33.14, SD = 10.13$). Seven identified as female and seven identified as male. Regarding race, seven participants identified as White, three as Black or African American, two as mixed-race, one as Asian, and one as Alaskan Native. All participants disclosed that they had at least one invisible disability, such as dyslexia, chronic pain, ADHD, and autism. Two participants did not disclose their specific disabilities but did share the general type of disability (e.g., chronic condition, learning disability). In total, 22 unique invisible disabilities were represented among our participants. All participants had used at least one social VR platform, but many used multiple. Most used VR on a daily or weekly basis. We present a detailed demographic breakdown in Table \ref{table:participants}. 

Participants were compensated with a \$20 digital gift card upon completion of the interview. This study and all procedures were approved by our university’s Institutional Review Board (IRB).

\subsection{Procedure}
We conducted semi-structured interviews via video conferencing software (Zoom). As part of the interview, we engaged participants in a creative activity on a collaborative whiteboard application (Google Jamboard), which allowed participants to draw and paint in multiple colors, import or link images from a device or online, type thoughts and ideas on sticky notes, and create text boxes and shapes. All interviews were conducted in English and lasted approximately 60 minutes. We provide our full interview protocol in Supplementary Materials.

We began the interview by asking participants demographic questions. We then asked about their uses for social VR and existing avatar representations in social VR, followed by probing about their current use of avatars as vessels for disclosure (or not). For example, we asked: “Do you represent or conceal your invisible disability in social VR in any way? How similar is your avatar representation to your physical self?” After establishing the similarities and differences between participants’ virtual and non-virtual selves, we asked if participants were interested in representing their invisible disability / disabilities in social VR. Regardless of their responses, we followed up by discussing how context might impact their decisions to represent (or not represent) their invisible disabilities. We wrapped up the first section by broadly exploring participants’ granular customization preferences.

We then encouraged participants to generate avatar ideas through creative brainstorming. We invited participants to express their “ideal avatar representation” in social VR by adding ideas through images, drawing, or text on a virtual whiteboard. After completing their visualizations and describing the thought processes behind them, we asked participants to describe important features that were not currently available, as well as their ideal customization process. Understanding that verbal brainstorming often privileges people who are comfortable generating ideas and expressing themselves through voice, we designed this activity to offer an alternative opportunity for self-expression and accommodate a broader range of communication styles.

We then explored the importance of context in virtual and non-virtual disclosure. We asked questions such as, “In the non-virtual world, how do you navigate disability disclosure? Would you consider your avatar representation to be the same or different in different settings? How does this compare to other platforms with avatar options, such as Snapchat?” Finally, we discussed the practical implications of incorporating invisible disability representation features into avatars. 

\subsection{Analysis}
We audio recorded and transcribed all recordings, then used open coding to analyze the interviews, drawing on a grounded theory approach. Three researchers divided the first three transcripts so that each was double-coded. We discussed code discrepancies, created the preliminary codebook, and then split up the remaining transcripts for individual coding. Throughout the coding process, the coders iterated upon and refined the codebook. 

After coding, we conducted thematic analysis \cite{braun2012thematic} to identify overarching takeaways and patterns across participants. Our themes were grounded in the interview codes as well as the suggestions presented by participants during the whiteboard component, which included image, drawing, and text artifacts. We iterated on the codebook by reflecting on the proposed themes’ connections to our research questions, comparing areas of overlap and divergence, and reflexively confronting potential analytical assumptions. After multiple rounds of iteration, the two co-first authors determined the final thematic findings in consultation with the rest of the research team.

\subsection{Positionality}
One of the first authors lives with an invisible disability and has a background in feminist disability studies. The research team also includes social VR users, accessibility researchers, and people who have grappled with the complex issue of disability disclosure in their own lives. We believe avatar customization is an important step toward improving the inclusiveness of social VR spaces, and aim to include the voices of invisibly disabled VR users into ongoing conversations surrounding fostering positive representation and cultivating diverse spaces. 

\begin{table*}[h!]
  \footnotesize 
  \centering
  \caption{Participants’ demographics.} 
  \begin{tabular}{p{0.3cm}p{0.9cm}p{1.5cm}p{2.8cm}p{3.8cm}p{2.8cm}}
  \toprule
   \textbf{ID}& \textbf{Age/ Gender}& \textbf{Race}& \textbf{Disabilities}& \textbf{Social VR Use}&  \textbf{Frequency} \\
       \midrule 
  
  \textbf{P1}&  32/F&  White& Low vision; panhypopituitarism& Altspace VR; Spatial& several times/week \\ 
  
  \textbf{P2}&  32/F&  White& Bipolar; PTSD& synth Riders; VR fishing; VRChat; Walk about Mini Golf; & daily\\ 

   \textbf{P3} & 56/F & Mixed-race& Dyslexia; rheumatoid arthritis; congestive heart failure& Altspace VR; VR fishing; VR Chat; Spatial; Big Screen; Wander& weekly\\ 

   \textbf{P4}&  38/F&  White & Dyslexia; epilepsy; chronic pain& the limps, Les Mills, body cam, FedEx, Sabre, the mini golf&  two to four or five times a week\\ 
    
   \textbf{P5}&  31/M&  White&  RSI; ADHD; Asperger’s& two to four or five times a week& social: monthly
VR in general: weekly\\ 
  
  \textbf{P6}&  24/F&  Black &  POTS& vTime XR; Altspace VR; miscellaneous; Rec Room; Ping-pong& weekly\\ 
  
   \textbf{P7}&  33/F&  White&  Depression& VR Chat& daily\\ 
  
   \textbf{P8}&  20/M&  Asian&  Chronic condition (diagnosis undisclosed)& VR Chat& one to two times a month\\ 
  
   \textbf{P9}&  28/M&  White, Asian&  Autism (nonverbal); learning impairment with linguistics (text); bipolar type one& VR Chat& "extensive"; 5000-6000 hours\\ 
  
   \textbf{P10}&  52/F& White& Hashimoto’s disease; contextual social anxiety; osteoporosis& VR Chat, Synth Riders& "live on there" - work, sleep, "addiction"\\ 
  
   \textbf{P11}&  28/M& Black& ADHD (undiagnosed)& Altspace VR; Spatial; Rec Room; Horizon Worlds& multiple times a month\\ 
  
   \textbf{P12}&  31/M& White& Asperger’s; ADHD& Altspace VR; Oculus; Rec Room; Facebook Horizon& game and therapeutic tool since 2019 \\ 

   \bottomrule
  \end{tabular}
  \label{table:participants}
\end{table*}

\section{Findings}
Social VR spaces reflected many of the norms and utilities of non-virtual social spaces. Participants used social VR for a variety of purposes, similar or even equivalent to their non-virtual social interactions, including entertainment (e.g., playing games), conversational (e.g., chatting with others), and professional (e.g., for work). For example, multiple participants described attending support groups, celebrating birthdays, and watching movies in social VR. Additionally, for some, virtual platforms provided them essential access to environments when their invisible disabilities prevented them from leaving home. 

\begin{quote}
“What I’m getting out of VR is a little different than what most people get out of VR. They get in there, and they want to [play games]. I’m there so that the world doesn’t close in on me… to keep a tiny little porthole of the world open to me. Even though I cannot physically be in it, I can virtually be in it. I can visit a museum through VR. I went up [to] the space station through VR. I’ve gone scuba diving in VR. And the social aspects \textemdash{} I’ve met friends who have been my friends for years, but we live in different states. And we’ve come together.” (P3, 56F) 
\end{quote}

In this section, we present participants’ perceptions on the unique affordances of embodied avatars, detail current and imagined invisible disability representations for social VR avatars, and explore disclosure preferences across different social VR contexts.
\subsection{Embodied Avatars are Dynamic, Contextual, and Multimodal}
Participants identified key differences in their perceptions of non-embodied and embodied avatars. In general, they viewed non-embodied avatars, such as Facebook profile pictures, Facebook avatars, and Snapchat Bitmojis, as a snapshot of their identity. On the other hand, embodied avatars were perceived as dynamic and authentic representations of themselves. Additionally, participants appreciated that embodied avatars allowed for multimodal self-expression, as reflected in their current and imagined preferences for disability representations in social VR. 

\subsubsection{Differences Between Embodied and Non-Embodied Avatars}
Though participants had experience using non-embodied avatars to represent themselves, they felt as though the static nature made it difficult for them to convey their true, current identity. For example, P1 said that her Facebook avatar \textit{“doesn’t look like me at all. I hate it.”} P3 also shared how her experiences with using Facebook and social VR for different purposes, and for different audiences, influenced her degree of comfort with representing herself in embodied and non-embodied contexts.

\begin{quote}
“With Facebook, of course my avatar is a photo of me. But it’s a photo of me 20 years ago. So my avatar doesn’t age there… and I have not changed it to be what I am now. Because the people that are on my Facebook, many of them are people that know me in this physical reality. … But it’s also something that I’m not gonna change, you know. I cannot pretend in Facebook that I’m well or not well… I don’t represent a cause, I don’t represent a disease, I don’t represent anything but myself. … Whereas in VR, I do change those things. … [in] virtual reality, there are people there that know and love me, but most people are acquaintances or strangers. So my interaction with them is going to be different [from] my interaction on Facebook.” (P3, 56F)
\end{quote}

Others also felt that the embodied nature of social VR avatars encouraged them to go beyond what they would choose on digital platforms. For example, P14 mentioned that the \textit{“immersive experience [of being] around a lot of people, seeing the avatar move around”} made him wish to represent himself in greater detail on a social VR avatar as opposed to a static avatar on Facebook. On the other hand, P4 preferred having an embodied cat avatar but shared an anecdote about the inconvenience of having her avatar’s eye line towards the ground when engaging with human-sized avatars. 

Referring to the overall experience of using mainstream, non-embodied social media networks, P13 also mentioned that he actively chose to not engage with these platforms to avoid \textit{“engagement loops that keep you coming back to it… they’ll track you with their pixel tracker on other websites and start sending you advertisements.”} In contrast to text-only communication on social media, he found the different communication modes in social VR to be easier to process: \textit{“[digital is] basically reading text messages, [whereas in social VR you have] voice chat, digital avatar, [or] motion capture”} (P13). Additionally, he mentioned that the discomfort and fatigue associated with VR headsets was helpful for preventing him from spending excessively long on these platforms. 

Some participants highlighted the heightened interactivity and expressiveness of embodied avatars. For example, as a content creator, P10 wanted to use her social VR avatar in her videos to merge her representations in virtual and non-virtual domains, stating that she “would actually love using an avatar instead of my real body in my YouTube videos” to represent herself with features such as tails and wings. When discussing the distinctions between social media and social VR, P9 summarized how his interactions differed between the two environments and emphasized that the immersive affordances of social VR avatars enabled him to not only better express himself, but understand others as well.

\begin{quote}
“[VR] is an order of magnitude above anything that you would see on Instagram \textemdash{} [or] any other website \textemdash{} because those are just two-dimensional static images or videos. [You] can’t interact with photos, but when you’re there in virtual reality, you can see all the details on the avatar showing that this person is expressing themselves. [You can] see their facial expressions, their movements, and their body language. And it’s real time. No other kind of social platform comes even close to VR.” (P9, 28M) 
\end{quote}

\subsubsection{Multimodal Affordances Can Represent Physical Human Expression}
Participants also utilized the multimodal expressiveness of embodied avatars, which manifested primarily through avatar visuals, voices, movements, body language, and facial expressions. For example, participants valued the ability to show dynamic and nuanced facial expressions.

\begin{quote}
“I am quite expressive myself, but my invisible disability is nonverbal autism, so I wouldn’t actually say what I’m feeling. I would express it through my avatar’s facial expressions. Sometimes, the number of expressions on an avatar goes as high as 30 or 40 different options. So having many different options to express myself nonverbally is a way that I can get more synchronized and comfortable using an avatar.” (P9, 28M) 
\end{quote}

As someone with bipolar, P2 was interested in using body language to represent changes in her mood. 

\begin{quote} 
“Let’s say I’m feeling excited or hyper. Your avatar can have a really upbeat energy to it if you’re going to apply an energy to an avatar. Or if you can put in there that you’re feeling slightly depressed, or that you have a low mood or that you’re tired, your avatar would be a little bit lower on the energy… That way my friends could see me and then go like, ‘Oh, that’s kind of the mood she’s in. Let’s cheer her up.’ Or, ‘Let’s just give her her space.’ … They can kind of match their energy to your mood without you having to be so vocal about it.” (P2, 32F) 
\end{quote}

Some participants explained how the embodied movement of VR avatars could represent or support their disability in VR. For example, P12 wanted to utilize either voice or movement: \textit{“if I am going to disclose my disability on the platform, it would be verbally or through using the VR controllers when I’m controlling the hands of the avatar.”} Conversely, though his experiences with arthritis sometimes impacted his mobility in the non-virtual world, P14 did not want to disclose his disability through this modality \textemdash{} he preferred for his avatar to move in the same ways as others. Regarding support of the disabled experience, P3 described how embodied avatar interactions could facilitate community empowerment and connection in a disability support group: \textit{“sometimes, our avatars will run over and give somebody a group avatar hug when they’re having a particularly bad time.”} 

\subsection{Current and Imagined Invisible Disability Representations}
Throughout the interviews, participants shared how they currently represented or disclosed their invisible disability and brainstormed ways to make avatar customization systems more inclusive. For example, P11 described his avatar to be \textit{“an exaggeration of [his] physical identity \textemdash{} anonymous, but also close enough to be recognized if you know [him] personally.”} P12 had a similar description: \textit{“I try to represent myself as I am, of course, and for me, that involves maybe making an avatar that looks like me but is a little bit cooler if possible.”}

We found that desired methods of representing invisible disabilities in social VR did not always align with non-virtual disclosure practices. Participants desired options for both public (i.e., explicit) and private (i.e., implicit) identity expression. Suggestions for both public and private representations encompassed clothing, accessories, icons, energy bars, or modifications to avatar bodies.

\subsubsection{Public Representations and Expressions of Disability}
Some participants were interested in representing their disabilities in public and explicit ways, meaning that other social VR users could identify their specific disability or their symptoms from their avatar. 

Ten participants suggested incorporating customizable clothing, patterns, or accessories that featured disability-related logos. These suggestions often supported participants’ goals of expressing their personal style and educating others about their disability. For example, P1 wanted to have an avatar wearing a zebra-printed shirt and beret to advocate for Rare Disease Month. Similarly, P12 wished to express his personal style and disability status through a \textit{“jacket [with] a label… to say my name and that I have Asperger’s and whatnot.”} Others suggested having accessories specific to their disability (e.g., P6 suggested a brooch saying “POTS,” P13 suggested a PTSD ribbon). P4 wished to have an explicit representation for communicating the experience of dyslexia through apparel: 

\begin{quote}
“[On clothing,] have the word dyslexia, but then have it jumbled up so people can see what it looks like when we try to read. Then, they’ll be like, ‘Whoa, that’s not fun.’ And we’re like, ‘Well, welcome to my hell.’ Make it a joke, but also kind of be like, ‘Hey, this is really what it feels like.’” (P4, 38F)
\end{quote}

Other participants wanted customization libraries to include assistive technology (e.g., wheelchairs, canes, crutches, hearing aids), a medical alert bracelet, and \textit{“spoonie”} gear (e.g., a giant spoon, as suggested by P1) to disclose their disabilities. 

\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{imgs/P1.png}
  \caption{Participant 1’s drawings and suggestions for invisible disability representation during the whiteboard component of the study, featuring a giant spoon to represent spoon theory and other assistive technologies to disclose their disability.} 
  \Description{Participant 1’s drawings and suggestions for invisible disability representation during the whiteboard component of the study. At the far left, there is a floating medication reminder inside a speech bubble that represents a floating emote. Below are examples of assistive technology such as a cane and hearing aids. Next is a person’s outline wearing a zebra print beret and shirt to represent rare disease month. The shirt also has a space for a custom disability graphic or a fact about the participant’s rare disease, both aimed at spreading invisible disability awareness. The person also wears a medical alert bracelet and carries a human-sized spoon to represent desired “spoonie” props that point to identification with spoon theory. Finally, there is a note where there would be a floating menu to enable and disable disability-related accessories.}
  \label{P1}
\end{figure*}

Icons and graphics around an avatar could also help with representing someone’s disability in a more subtle, but still public, way. Four participants were interested in disability representations that floated above their avatars, such as an awareness flag or a dynamic energy bar that correlated with their energy level or “social battery”. For example, P2 proposed \textit{“an energy bar, like in a video game where you have your life meter. If it’s full, you’re full of energy, and it’s all the way green… And if I’m really low on energy, I’ve got a red bar.”} Recognizable icons, such as the rainbow infinity symbol to represent neurodiversity, were also valued; however, participants specifically criticized harmful iconography, such as the light blue puzzle piece representing the Autism Speaks organization. P11, a designer by trade, proposed disclosing his disability through design patterns and iconography inspired by video games and internet culture. He emphasized the transient nature of this representation so as not to greatly disrupt social interactions.

\begin{quote} 
“So “i” is “information” … You click that… [and it pops up] this universal image for neurodiversity. … The image pops up for only a few moments… That way, you can continue your interactions in virtual space without necessarily having the label on you constantly.” (P11, 28M)
\end{quote}

\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{imgs/P11.png}
  \caption{Participant 11’s images, sticky notes, and suggestions for invisible disability representation during the whiteboard component of the study, featuring an information icon and the ADHD rainbow butterfly symbol above the avatar.} 
  \Description{Participant 11’s images, sticky notes, and suggestions for invisible disability representation during the whiteboard component of the study. There is an image of Toad, an anthropomorphized mushroom character from the Mario franchise, wearing an astronaut suit and helmet. On his cap, there is an information icon (a lowercase i in a circle) and above Toad is the ADHD rainbow butterfly symbol. To Toad’s right, there is a sticky note that reads, “General notice of invisible disability - other users can click to reveal more information. More information is presented as a specific symbol represen-”. To the right of the ADHD symbol, there is a sticky note reading “Symbol is animated and hovers on top the avatar for a few seconds after the (i) button is clicked.”}
  \label{P11}
\end{figure*}

Disability representations also included temporary adjustments to the avatar to indicate a user’s interest in engaging with others. Similar to the energy bar example, P11 proposed a feature that would allow an avatar to turn invisible when a user wanted to avoid social interactions, which he dubbed as a \textit{“stealth mode.”} However, P11 assessed the potential privacy implications of implementing such a feature, and concluded that turning an avatar translucent could convey a similar message of wishing to keep to themself while still alerting other users to the fact that there was another user within the space.

\begin{quote} 
“If I’m in [a] VR space and I just want to enjoy myself, and I don’t want anyone coming up to me, I should be able to say that. … [but] if you think about the other users of the space, do you really want an invisible person watching you? … Maybe rather than being invisible… I can just make him more white [translucent] instead… ‘Just don’t come to me. [My avatar’s] not really colorful right now.’” (P11, 28M) 
\end{quote} 

Participants’ public representations of their disability leveraged affordances of the embodied avatar experience, such as wearing custom-designed clothes and accessories to advocate for invisible disabilities, having a visible “energy bar” to indicate mood and energy level, and changing colors to express one’s willingness to interact with others. 

\subsubsection{Private Representations and Expressions of Disability}
Below, we describe participants’ private avatar customizations, which carried personal meanings such that they could still represent their invisible disability without necessarily disclosing their disability identity to others.

Participants primarily suggested representing their disability or experiences through accessories that matched those that they would wear in non-virtual settings. For example, P3 preferred more subtle accessories that would more closely resemble non-virtual affordances: \textit{“I would do it with accessories, [but] I don’t want a big sign saying, ‘disabled’ or a different color flashing over here that says ‘invisible illness is no longer invisible.’”} P12 also wanted to use clothing or accessories that blurred private and public significance: 

\begin{quote}
“I utilized my interest in cars as both something to therapeutically do but also maybe relate to others that have that same interest. Which is why I also, in real life, like to collect diecast cars and books on cars and, sometimes, I also like to wear clothing with cars on it. This is more of a social preference. … If [others] at least understand my passions and interests and how knowledgeable I am about them, then maybe they have a better understanding of me, too.” (P12, 31M)
\end{quote} 

Others used accessories to represent themselves. During the creative exercise, P8 gave his avatar earbuds, explaining: \textit{“I’m not a big earbud guy, I’m a headphone wearer [in the physical world]… [but] I feel like maybe it would be an extension of you trying to conceal what invisible disabilities I would have, just pretending to be normal with stuff like that.”} While this representation of his invisible disability was not explicit to others, he acknowledged that the earbuds were \textit{“more of an expression of [him]”} and preferred to keep this aspect abstract. P14 also utilized headphones and a mask as symbolism for \textit{“blocking out all the noise”} in the environment. Similarly, P9 also described how his ideal avatar representation included elbow and knee pads: 

\begin{quote}
“I really want to add knee and elbow pads. If you have ever gone roller skating, you need to put on knee and elbow pads, just in case you fall… The bipolar makes me swing really hard to the left and right. I get these mania phases and these depression phases that have a whiplash to them. And sometimes… I can get hurt or accidentally hurt others. So these pads on my knees and elbows would be a way to symbolize that if I do fall, I gotta make sure I’m protected. I don’t fall too hard, and I can stand up again.” (P9, 28M)
\end{quote}

Three participants were interested in alterations to their avatar itself, beyond accessories, that could indicate their difference from other users in an implicit way. For example, P9 used vibrant colors: \textit{“It’s a way that I can visually differentiate myself from a room full of other people. It’s my way of not just indicating to others that this person’s a little different, but it’s also indicating to myself that I’m a little different.”} P10 also expressed that her avatar’s large bushy tail represented her comfort zone and personal bubble. She described using her humanoid and avatar-based self-expression as a metaphor for her non-virtual personality, further emphasizing the unique affordances of social VR in expanding the bounds of self-expression by allowing fantastical and metaphorical representations of the self. 

\begin{quote} 
“[My avatar’s] tail wraps around it a lot… but I like that one because, in some weird way, it gives me a comfort zone of hiding me in a bubble. … Even in real life, people have said I have a bubble, like a huge bubble around me. It’s like you get too close to me… [and] I just back away a little.” (P10, 52F)
\end{quote}

Though some participants brainstormed representations of disability were intended to be explicit, they realized that their ideas could still be implicit to other social VR users. For example, P9 emphasized how his embodied avatar reflected his mood, especially related to his experiences with Bipolar Type 1. He used VR avatar appearances to communicate his emotions nonverbally, strategically selecting avatars based on his goals for social interactions that day. He explained his use of colors and their social and psychological effects: 

\begin{quote}
“The middle avatar is the avatar I use when I’m in a playful mood. It stands out, but it’s also really friendly looking. I got a lot of people that like to hang around with me in this one if I’m feeling energetic, a little bit extroverted. If we talk about bipolar phases a little bit more, like the manic phase, I’ll use the middle one. … If I’m in a really happy mood, but I pick an avatar with like no color, for few emotions, it wouldn’t really match. Same thing vice versa. It also adds some novelty to VR chat as well… I like to mix it around, so I know there’s always flexibility to iterate and change.” (P9, 28M) 
\end{quote}

Similarly, while P5 wished to use glowing veins to represent chronic pain from repetitive strain injury, he acknowledged that other users might not understand the disability-related symbolism: \textit{“[the glowing veins] still wouldn’t even show pain, because people are gonna look at that and just go like, ‘cool.’ They just see glowing things on your arm.”} Even though most other social VR users would not understand that a disability was being expressed, these private and often implicit representations of disability were still valuable to participants.

\subsection{Invisible Disability Disclosure Practices Differ Based on Context}
In this section, we explore participants’ varied motivations for disclosing or sharing their disability identity, informed by both different social VR environments and the dynamic nature of their disabilities. Then, we highlight participants’ suggested customization features and methods for making the customization process more accessible. 

A variety of social factors influenced participants’ disclosure strategies: some were comfortable with disclosing their identity at all times, some preferred disclosing only some of the time, and others did not want to disclose in social VR at all. We found that participants generally belonged to one of three groups: \textbf{Activists}, \textbf{Non-Disclosers}, and \textbf{Situational Disclosers}. \textbf{Activists} were always open to disclosing to spread education and awareness, often tying into advocacy work that the participants did outside of social VR contexts. \textbf{Non-Disclosers} did not want to disclose their invisible disability to others in any circumstances. Lastly, \textbf{Situational Disclosers} were sometimes open to disclosing their identity, and would rely on context cues to make their disclosure decisions. 

\subsubsection{Activists and Non-Disclosers}
One participant was part of the \textbf{Activist} group. P1 identified as an outspoken disability activist and felt comfortable openly sharing her disability in social VR. She felt that disclosing her chronic condition was helpful not only for raising awareness but also for indicating her access needs.
 
\begin{quote}
“I am an activist and an advocate for folks that have invisible disabilities… I’m an open book. So anything that can start a conversation or encourage people to ask questions is really valuable to me, and I feel like having that option is just really important in terms of raising awareness for things like that. And I like people to actually know. If I’m going to start a friendship with somebody, I want them to be aware of the fact that I have a chronic illness, because that is a pretty large part of my life, and it does affect my ability to socialize sometimes. So you know, being open about that is important to me personally.” (P1, 32F)
\end{quote}

On the other hand, one participant was not comfortable disclosing their disability identity in social VR at all. P8, a \textbf{Non-Discloser}, concealed his invisible disability in all non-virtual social situations and did not want to disclose in social VR either, as he felt that \textit{“[others] wouldn't be very receptive or kind to that”} and he did not want to be treated as \textit{“lesser than someone else.”} He emphasized that his invisible disability was not a core part of his identity, especially as it was \textit{“a condition that didn’t come until the last five years or so, so it’s not like I grew up with it”} (P8). Additionally, having observed others face negative stigmas strengthened his opinion of not disclosing his identity in any contexts, VR or otherwise: 

\begin{quote}
“It comes from personal experience… friends that have also had [my condition], it's like you're treated differently. … I’m trying to hide it so much that, outside of my family, I don’t think I ever opened up to anyone about it.” (P8, 20M)
\end{quote}

\subsubsection{Situational Disclosers: Disclosure Practices Informed by Perceptions of Stigma}
Participants’ different contexts, within and outside of VR, had a strong impact on when and why they chose to disclose their invisible disability. While only a couple of participants identified as Activists or Non-Disclosers, the remaining 12 participants expressed varying degrees of excitement and hesitancy to represent their disability. Most did not want to disclose in large group contexts because of their perceptions of the stigma they would face and due to prior negative experiences with disclosure. For example, P9 mentioned how he tried to mask or pass as nondisabled when interacting with others in social VR: \textit{“I don’t really represent my disability too much, but I also don’t conceal it.”}

For six Situational Disclosers, their intended audience significantly influenced their avatar design choices, and they often chose to disclose to support other disabled people in a safe space. For example, P3, P4, P6, and P9 stated that they were more likely to disclose in a disability-specific community rather than a large social situation. P9 specifically mentioned that disclosing in this context allowed them to empathize and engage; similarly, P2 felt that describing her experience with bipolar disorder in her profile could provide support to others: \textit{“I very much enjoy [being] open with people, especially once I’ve made a connection with them. I don’t feel like it puts me at any risk or any danger… if anything, it adds to my support system.”} P4 also acknowledged that she did not want to disclose her disability to just anyone in social VR: \textit{“we would mostly have to become friends outside of the virtual reality world for me to feel comfortable to disclose it.”}

Regardless of the scale of a social context, some felt as though certain disabilities carried more stigma compared to others. P4 was interested in disclosing two of her invisible disabilities but not a third \textemdash{} she felt comfortable representing dyslexia and chronic pain, but not epilepsy: \textit{“I’ve had more hatred for [having epilepsy] than dyslexia because most people understand dyslexia.”} Furthermore, P5 mentioned that the stigmas associated with Asperger’s and ADHD were \textit{“embarrassing”} and commonly \textit{“poked fun at a lot online,”} which furthered his concerns of being disrespected due to the \textit{“negative public perception”} of his disabilities. P12 also described their prior experiences of facing discrimination against neurodivergent people: 

\begin{quote}
“I don't go out of my way all the time in VR to disclose my disability. Some, if not many, people may not fully understand what the disability is about. Or, they'll jump to conclusions and assume… I don't want to get labeled that way. I don't want to be labeled as someone who's [r-word]. … that word has been thrown around a lot recently.” (P12, 31M)
\end{quote}

Given the fluctuating nature of some invisible disabilities, some participants’ disclosure preferences were also dynamic. For example, P2, P6, and P10 chose to disclose based on their mood or flare-ups. P2 mentioned that she would sometimes disclose their disability to help others \textit{“understand what I’m going through… to avoid conflict,”} especially in a work setting. P6 also noted that \textit{“I really only disclose if I feel like I’m about to have a flare up.”} Similarly, P10 mentioned: \textit{“when my Hashimoto’s flares up, I lose lots of hair, I have no energy, and I am just tired… So people [can understand], ‘Okay, she’s dealing with that today.’”} P3 elaborated on how having customizable avatars played a psychological role in grounding her VR experiences: \textit{“[having options] gives you virtual reality with just a little bit of more normalcy. … It gives you a little bit of an anchor to not overwhelm you”} (P3).

Participants also shared how they wished to toggle specific avatar features on and off to support their dynamic disclosure preferences. P9 shared that he felt comfortable and open to disclosing their disability in social VR, but that having a toggle for disclosure features could be crucial for avoiding ableism in unwelcoming settings. As someone with social anxiety, P10 also thought that having options to both (1) have her disability representation permanently fixed to their avatar and (2) select her disability representation on a daily basis would be most helpful: \textit{“if you have social anxiety every single day, there’s no reason to switch that on and off. That gives you anxiety, having to go do that every day.”} P3 explained how the toggles could be used for not only representing, but also managing her invisible disability: 

\begin{quote}
“My VR avatar is whatever I’m feeling at the moment. If I’m feeling immersed in my invisible illness, then I’m probably gonna want my avatar to be also. If I’m feeling like, ‘okay, I’m escaping reality,’ I don’t want my avatar to be even close to what I am. [In our support group,] there will still be some days that I don’t want to manifest [my disability]. And then other days where it’s like, ‘Yeah, I’m feeling like crap and I’ll let you people know it in a non-verbal way,’ and I will come in there all crippled up with my avatar, altered to represent how I feel right now simply because I am trying to communicate it in a nonverbal way.” (P3, 56F)
\end{quote}

Disability is one facet of the complex human experience, filtered through intersecting lenses of other identities like gender and race. Participants identified connections between the experiences of people in multiple marginalized groups. P6 acknowledged her intersectional identities of race and invisible disability, and drew on her daily experiences in social and workplace settings to inform her avatar disclosure preferences:

\begin{quote}
“I feel like I’m seen as unreliable. Obviously, I’m also a Black woman, so that compounds things \textemdash{} that intersection of discrimination. But I do feel like I actively do not get treated well when I talk about it. In social situations, I'm not concerned about it the way that I am in professional circumstances. … The intersection of disability and race has made me a lot less likely to disclose over the years. As I’ve seen, figures of authority are not necessarily empathetic or respectful about it.” (P6, 24F)
\end{quote}

\subsubsection{Social VR vs. Non-Virtual Disclosure Preferences}
Some participants perceived social VR to be a relatively safe space where they could freely express their disability-related identities without worrying as much about the stigma they faced in the non-virtual world. For example, a few participants felt more open to disclosing disabilities in social VR because the “disability” label would not persist across contexts. P9 explained: \textit{“I feel like once I label myself [with a disability] in real life, it becomes something that kind of follows you around.”}

However, others felt as though social VR experiences ranged from relatively safe communities to potentially harmful environments. For example, P13 recalled a news article reporting about a woman being assaulted in social VR spaces, and briefly mentioned his own experiences of being assaulted in VR. When speaking about specific VR platforms, P1 acknowledged how disability disclosure in social VR could potentially result in harassment:

\begin{quote}
“If you’re going into more of a rough and rowdy crowd, like in VR Chat, you don’t want to make yourself a target for people that might look for things to hurt you with. … If you’re going to a place that you don’t really know very well, I think it would be a good idea to be able to turn [disability representations] off or on.” (P1, 32F) 
\end{quote}

When speaking about the personal importance of visibly representing his invisible disability identity, P12 drew parallels between LGBTQ and disability representation in the media. While he did not necessarily disclose his disability in non-virtual settings, he cited LGBTQ award-winners at the Tony Awards as examples of ways that queer people expressed and disclosed their identity through clothing and other visual means. 

\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{imgs/P12.png}
  \caption{Participant 12’s images, sticky notes, and suggestions for invisible disability representation during the whiteboard component of the study, featuring screenshots of two different avatars he uses. The images are blurred to preserve the participant’s anonymity.} 
  \Description{Participant 12’s images, sticky notes, and suggestions for invisible disability representation during the whiteboard component of the study. On the top there are four sticky notes, reading “Important notes for Autism and Aspergers with Avatars in VR: 1. Make sure facial expressions and non verbal expressions are accurate and can also include descriptions as needed.” / “For those who also may be LGBTQ or have a physical disability, have accurate representations of them.” / “Offer opportunity to have a community for those to share similar interests as a way of improving socialization” / “Learn behavioural techniques in virtual environments and inhibit restrictions to help.” Below the sticky notes are three screenshots of P12’s avatar. On the left is a screenshot of his avatar’s head and torso with a box sketched to the right of his head. The avatar is 3D, light-skinned, has a beard, short hair, sunglasses, and a Unity sweatshirt. The middle screenshot shows a 2D avatar with glasses, a goatee, and wearing a blue shirt with a brown vest; the avatar’s hands are raised and it says “Happy New Year!” above his head. The screenshot on the right is a zoomed out version of the screenshot on the left, showing the 3D avatar’s whole body.}
  \label{P12}
\end{figure*}

\subsection{Accessible Methods for Customizing Avatars}
Five participants expressed interest in easier processes for creating custom avatar designs. Participants also mentioned that text-to-avatar pipelines could lower the barrier to avatar customization, which was perceived as intimidating for participants who did not know how to use Unity or other platforms that rely on user coding. For example, P11 felt that \textit{“[being] able to type in what you’re [thinking], or what you want through maybe image generation or text to 3D tools, would be a great way”} to reduce the burden of users navigating complex customization systems within social VR systems themselves. Similarly, P5 also explained that current avatar customization processes were inaccessible; he wished to minimize arm movement requirements due to repetitive strain injury, and shared ideas for using AI to help with avatar customization: “WIf you have the option of pressing a bunch of buttons or just being able to think it and it appears on the page, why would anyone want to have all the billion options when they could do the exact same thing? It has occurred to me, though, with the recent AI developments, where you can produce pictures, it seems like it’s not too far away that they could just produce a 3D model using those systems. Like if there was a system where you could describe it, and it would generate one” (P5).

\section{Discussion}
Avatar customization libraries decide who gets to express what identity; however, current options do not enable the explicit expression of invisible disabilities. Unlike people with visible disabilities, who often depict disabilities through adding assistive technology to their avatars \cite{zhang2023diary}, we found that invisibly disabled people preferred to adopt more nuanced and symbolic approaches such as clothing-based designs (e.g., custom disability-related graphics) and accessory-based features (e.g., a floating energy bar). Additionally, a distinction emerged between public representations with explicit meaning and private representations with personal significance and implicit meaning. We discovered that context informs virtual disclosure preferences; participants’ strategies were also motivated by educational and awareness-raising goals or traumatic non-virtual disclosure experiences. Through the unique multimodal interactions afforded by social VR avatars (e.g., synchronous voice chat, motion tracking, facial expression), we also found participants leveraged the embodied nature of social VR to represent their disability identity in more varied ways than on social media. 

In this section, we discuss the distinctions between embodied and non-embodied social contexts, a taxonomy for disability disclosure, and design recommendations for future accessible and inclusive avatar customization systems.

\subsection{Preferences Across Embodied and Non-Embodied Social Contexts}
As shown in prior work, social VR establishes a context distinct from the non-virtual world \cite{}. The relative newness of this social setting brings significant potential \textemdash{} with some even referring to VR as “a technological ‘wild west’” \cite{harley2022would}. While social VR allows users to have greater degrees of self-expression and identity affirmation \cite{}, it also introduces new risks of hate and harassment \cite{}. As a result, users must navigate the newfound advantages of identity representation within VR spaces while also adopting new methods for protecting themselves and mitigating harm.

Our study uncovered explicit contrasts between disability representation preferences for embodied avatars compared to digital social media platforms such as Facebook or Snapchat. While Mack et al. \cite{mack2023towards} explored contextual differences across digital gaming and social platforms such as Roblox and Snapchat, we extend prior findings from on invisible disability representation by examining social VR’s multimodal affordances for identity expression. Social media limits open disclosure to 2D visual and text, whereas social VR offers users multiple channels for sensory expression (e.g., facial expressions) in addition to wearable disability representation through embodied avatars. However, to some degree, it is difficult to disentangle how these contrasts are influenced by the \textbf{audience} (e.g., primarily strangers in VR vs. primarily acquaintances and friends on social media), the \textbf{culture of a platform} (e.g., sharing synchronous experiences in social VR vs. sharing periodic life updates on social media), and the \textbf{sense of embodiment} (much higher in VR than on social media). Future work could examine the emerging and varied contexts in social VR to more explicitly identify the many ways in which avatar representation preferences differ between social VR and social media.

Furthermore, the embodied nature of VR avatars invokes a new degree of representation \textemdash{} avatar movements, also known as locomotion, can be another way in which invisibly disabled people align their virtual avatars with their non-virtual presentations. Prior work has examined how including diverse locomotion techniques can make video games more inclusive \cite{mason2022including}. For people with chronic conditions (including chronic pain), mobility or motor disabilities, or other disabilities which involve self-stimulating behaviors (i.e., stimming), their non-virtual behaviors and locomotion techniques are currently concealed by their VR avatars \cite{bozgeyikli2016locomotion}. Most work on virtual reality and disabilities takes a medicalized approach, focusing primarily on diagnosis, training, or rehabilitation (e.g., \cite{matamala2019immersive, ahmadpour2019virtual, harrison2002role, laufer2011virtual}), with some exceptions \cite{zhang2022s, zhang2023diary, mack2023towards}. We encourage future research to instead examine the rich potential for locomotion to serve as another method of disability disclosure and identity affirmation for people with both visible and invisible disabilities.

\subsection{Taxonomy of Disability Disclosure Strategies}
Disability disclosure preferences often vary by context and condition, a nuanced choice that becomes more pronounced with social VR embodiment and real-time immersion \cite{freeman2021body}. We discovered themes surrounding disclosure, perceptions of stigma, and novel representations of invisible disabilities. Similar to Furr et al. \cite{furr2016strategic}, we examine the three motivational groups that emerged from the data: \textbf{Activists}, \textbf{Situational Disclosers}, and \textbf{Non-Disclosers}. We now examine how the unique affordances of social VR facilitate novel disability expression and disclosure considerations.

The data indicated that participant motivations for disclosure fell into three groups. The first group, \textbf{Activists}, were always open to disclosing to spread education and awareness. The second group, \textbf{Situational Disclosers} who were sometimes open to disclosing, would rely on context cues and environmental culture to make their disclosure decisions. The third group, \textbf{Non-Disclosers}, could not think of a situation where they would disclose their invisible disability to others. 

As alluded to by the taxonomy above, 

Our taxonomy shows how, though disability disclosure can be dynamic, different people tend to adopt one of the three patterns. 


Deciding whether to disclose is an ongoing negotiation across both digital (non-embodied) and virtual (embodied) platforms. In the context of embodied social VR, a recent study revealed that avatars with disability representations were more likely to experience ableism harassment during group social interactions \cite{zhang2023diary}. As such, it is important to offer an easy-to-use toggle on and off feature with disability representations so users can operate with the utmost autonomy in their avatar disclosure decisions. At present, avatar design processes are complex. Customization platforms such as Ready Player Me \cite{readyplayerme} offer “hundreds of options” but are often inaccessible to people from non-technical backgrounds. To streamline the customization process, we suggest that avatar design processes implement more options relevant to invisible disabilities so that self-representation is also accessible for users from non-technical backgrounds. Further, taking inspiration from participant suggestions like the dynamic energy bar, we suggest that future avatar designs incorporate intuitive and universally applicable design conventions (e.g., traffic light color guidelines \cite{trafficlight}), allowing users to effectively express themselves.

Our findings support preliminary discussions of invisible disability representation in non-virtual contexts, where there was interest in symbolically representing and disclosing invisible disabilities through toggling representations on and off. In higher education, Canadian university students expressed interest in a concealable invisible disability marker to generate greater understanding, such as a blue dot in place of the handicapped sign associated with visible disabilities \cite{mullins2013lived}. The present study’s participants strengthened and expanded on this initial suggestion by offering more actionable implementations of disability expression across various modalities, which speaks to the creativity and self-exploration offered in VR affordances versus non-virtual settings. 

\subsection{Embodied Avatar Design Recommendations} 

Based on our findings, we offer the following list of design recommendations. 

\begin{enumerate}
\item \textbf{Create more options for multimodal customization.} 
    \begin{itemize}
      \item For some users with invisible disabilities, certain forms of communication are more comfortable than others (e.g., verbal, visual, etc.). 
	\item By making it possible for users to dive further into fine-tuning their movements and facial expressions to represent physical communication of accommodations needs and dynamic thresholds for social interaction, social VR platforms can maximize a breadth of opportunities for making social VR a better experience for those with invisible disabilities.
    \end{itemize}
\item \textbf{Include explicit options for invisible disability representation on social VR customization platforms.} 
    \begin{itemize}
      \item Even though some participants suggested highly individualized representation ideas, \textbf{we recommend including awareness-building apparel and accessory options in customization libraries} (e.g., zebra print for rare disease month, dyslexia-oriented t-shirt design, giant spoon accessory for representing chronic illness \cite{spoontheory}). Navigating customization can be challenging for multiple reasons (see examples below), so offering a number of pre-set invisible disability representation features can help eliminate barriers to boosting awareness and facilitating self-expression. 
    \end{itemize}
\item \textbf{Make the avatar customization process more accessible.}
    \begin{itemize}
      \item Many social VR users \textbf{do not have the programming background} necessary to manually fine-tune more individualized customization features like those that might represent invisible disabilities.
      \item People with invisible disabilities want to be able to \textbf{upload custom apparel logos and t-shirt designs} that represent their disabilities. 
      \item Because of the \textbf{personal significance of many suggested disability representations}, a number of invisible disability-related customizations would need to be individually uploaded by social VR users.
      \item Consider ways to \textbf{minimize or remove the physical burden of swiping} through long lists of customization options to enhance accessibility, including customization by way of text or drawing. 
    \end{itemize}
\end{enumerate}

\subsection{Limitations and Future Work}
For this study, we encountered some difficulties with recruitment. Participants needed to feel comfortable disclosing they had an invisible disability to participate in the interview; as such, we do not capture the perspectives of invisibly disabled people who do not wish to disclose their disabilities at all. We also considered that some people with chronic illnesses, neurodivergence, or other invisible disabilities might not identify as having an invisible disability. To reach a wider audience, we altered our language in different rounds of recruitment to include different examples of invisible disabilities. Additionally, due to recruiting adults aged 18 or older, we did not connect with the large population of youth and teen VR users and gamers. Despite these challenges, our participants shared diverse viewpoints while also having overlapping experiences. We halted recruitment once thematic saturation was achieved.

Given that we primarily recruited from U.S.-based organizations, we recognize the geographic limitations of this study and acknowledge the importance of situating findings in diverse cultural and socioeconomic contexts. We understand that disability representation preferences, especially those linked to established symbolism, are culturally and geographically dependent. For example, while symbols like a spoon \cite{spoontheory} are globally recognized as a representation of invisible disability, others, like the hidden disabilities sunflower, are more local \cite{sunflower}. Though we recruited from organizations, listservs, and social media threads globally, we did not collect participants’ country of origin and acknowledge that many of our participants were located in the United States. Future work could investigate invisible disability representation preferences across different cultural and geographic contexts.

\section{Conclusion}
Avatars mediate interpersonal interactions between social VR users, but at present, no built-in options exist for people to explicitly represent invisible disabilities. In this study, we explored the avatar customization preferences of invisibly disabled people. Users wished to tap into VR’s multimodal affordances (e.g., facial expressions, body language) to communicate their invisible disabilities. More broadly, users were interested in representing their invisible disabilities through various explicit avatar features (e.g., clothing, icons), and many desired an easily usable mechanism to toggle disability representations on and off in different contexts. We identify a distinction between public and private representations of disability and offer a new perspective that takes into consideration the importance of personal significance during self-expression, in addition to explicit and widely understood symbols for invisible disabilities. To our knowledge, this is the first study to specifically examine the embodied avatar representation preferences of social VR users with invisible disabilities. Our findings contribute to the ongoing conversation of designing with and for people with invisible disabilities. We hope this study inspires more researchers to offer future contributions to the valuable study of invisible disability representation and accessibility in technology-mediated social contexts.

